Exploring the substructure of nucleons and nuclei with machine learning

Perturbative quantum chromodynamics (QCD) ceases to be applicable at low interaction energies due to the rapid increase of the strong coupling. In that limit, the non-perturbative regime determines the properties of quarks and gluons (partons) in terms of parton distribution functions (PDFs) or nuclear PDFs, based on whether they are confined within nucleons or nuclei respectively. Related non-perturbative dynamics describe the hadronisation of partons into hadrons and are encoded by the fragmentation functions (FFs). This thesis focuses on the detailed study of PDFs in protons and nuclei as well as the charged pions FFs by means of a statistical framework based on machine learning algorithms. The key ingredients are the Monte Carlo method for error propagation as well as artificial neural networks that act as universal unbiased interpolators. The main topics addressed are the inference of proton PDFs with theoretical uncertainties and the impact on the gluon PDF from dijet cross-sections; a global determination of nuclear PDFs exploiting the constraints from proton-lead collisions at the LHC and using for the first time NNLO calculations; a new determination of FFs from single-inclusive annihilation and semi-inclusive deep-inelastic scattering data; and a quantitative assessment of the impact of future colliders such as the High-Luminosity LHC and the Electron-Ion Collider on the proton and nuclear PDFs.

==> _diagrams/compile <==
make clean
make realclean
make -j
rm feyngraph.*
latex $1
mf '\mode:=localfont; input fmftempl' 
mf '\mode:=localfont; input feyngraph'
latex $1
pdflatex $1

==> _diagrams/feynmf/Makefile <==
# Makefile -- install feynmf.
# Copyright (C) 1994,1995 Thorsten.Ohl@Physik.TH-Darmstadt.de
#
# Feynmf is free software; you can redistribute it and/or modify it
# under the terms of the GNU General Public License as published by 
# the Free Software Foundation; either version 2, or (at your option)
# any later version.
#
# Feynmf is distributed in the hope that it will be useful, but
# WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the 
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program; if not, write to the Free Software
# Foundation, Inc., 675 Mass Ave, Cambridge, MA 02139, USA.
#
# $Id: Makefile,v 1.27 1996/12/02 09:20:35 ohl Exp $
#
########################################################################

VERSION = 1
RELEASE = 08
STATUS  = 

########################################################################

# Directories
prefix = $(HOME)
bindir = $(prefix)/bin
mandir = $(prefix)/man/man1
texdir = $(prefix)/tex/inputs
mfdir = $(prefix)/mf/inputs
docdir = $(texdir)/doc

# Commands
INSTALL = install -c -m 755
INSTALL_DATA = install -c -m 644
# INSTALL = cp
# INSTALL_DATA = cp

# This has to be the new LaTeX
LATEX = latex
# This should be the old LaTeX
LATEX209 = tex '&latex209'
# This must not have the cmbase preloaded:
MF = mf
MP = mp
MAKEINDEX = makeindex

# Your local printer mode
MFMODE = laserjet

########################################################################
# No user serviceable parts below:
########################################################################

RESOLVE_XREF = \
  $(LATEX) $*.drv && \
  while grep 'Rerun to get cross-references right\.' $*.log; \
  do \
    $(LATEX) $*.drv; \
  done

RESOLVE_XREF209 = \
  $(LATEX209) $*.drv && \
  while grep 'Rerun to get cross-references right\.' $*.log; \
  do \
    $(LATEX209) $*.drv; \
  done

RUN_METAFONT = \
  $(MF) '\mode:=$(MFMODE); input fmfsamp1'; \
  $(MF) '\mode:=$(MFMODE); input fmfsamp2'; \
  $(MF) '\mode:=$(MFMODE); input fmfsamp3'; \
  $(MF) '\mode:=$(MFMODE); input fmfsamp4'

RUN_METAPOST = \
  $(MP) fmfsamp1; \
  $(MP) fmfsamp2; \
  $(MP) fmfsamp3; \
  $(MP) fmfsamp4;

RUN_MAKEINDEX = \
  $(MAKEINDEX) -s gind.ist -o $*.ind $*.idx && \
  $(MAKEINDEX) -s gglo.ist -o $*.gls $*.glo

MANPICS = manpics.1 manpics.2 manpics.3

all: feynmf.sty feynmf.mf feynmf.drv \
     feynmp.sty feynmp.mp feynmp.drv $(MANPICS) \
     feynmf.1

all209: feynmf209.sty feynmf.mf feynmf209.drv \
	feynmp209.sty feynmp.mp feynmp209.drv $(MANPICS)

man: fmfman.dvi

man209: fmfman209.dvi

quick-man:
	$(MAKE) man RUN_MAKEINDEX=: RESOLVE_XREF=:

dvi: feynmf.dvi

dvi209: feynmf209.dvi

quick-dvi:
	$(MAKE) dvi RUN_MAKEINDEX=: RESOLVE_XREF=:

bigtest: feynmf.dvi feynmp.dvi fmfman.dvi fmfmanps.dvi manual.ps

bigtest209: feynmf209.dvi feynmp209.dvi fmfman209.dvi \
	    fmfman209ps.dvi manual209.ps

install: all
	$(INSTALL_DATA) feynmf.mf $(mfdir)
	$(INSTALL_DATA) feynmp.mp $(mfdir)
	$(INSTALL_DATA) feynmf.sty $(texdir)
	$(INSTALL_DATA) feynmp.sty $(texdir)
	$(INSTALL_DATA) feynmf.1 $(mandir)
	$(INSTALL) feynmf.pl $(bindir)/feynmf

install.doc: all
	$(INSTALL_DATA) feynmf.dtx $(docdir)
	$(INSTALL_DATA) feynmf.drv $(docdir)
	$(INSTALL_DATA) fmfman.drv $(docdir)
	$(INSTALL_DATA) $(MANPICS)  $(docdir)

uninstall:
	rm -f $(mfdir)/feynmf.mf
	rm -f $(mfdir)/feynmp.mp
	rm -f $(texdir)/feynmf.sty
	rm -f $(texdir)/feynmp.sty
	rm -f $(bindir)/feynmf
	rm -f $(mandir)/feynmf.1

uninstall.doc:
	rm -f $(docdir)/feynmf.dtx
	rm -f $(docdir)/feynmf.drv
	rm -f $(docdir)/fmfman.drv

feynmf.sty: feynmf.dtx feynmf.ins
	$(LATEX) feynmf.ins

feynmf209.sty: feynmf.dtx feynmf209.ins
	$(LATEX209) feynmf209.ins

feynmf.mf feynmf.drv feynmp.sty feynmp.mp feynmp.drv \
  fmfman.drv fmfmanps.drv: feynmf.sty

feynmf209.drv feynmp209.sty feynmp209.drv \
  fmfman209.drv fmfman209ps.drv: feynmf209.sty

feynmf.dvi: feynmf.dtx feynmf.drv feynmf.sty feynmf.mf $(MANPICS)
	-$(LATEX) $*.drv
	$(RUN_METAFONT)
	-$(LATEX) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF)

feynmf209.dvi: feynmf.dtx feynmf209.drv feynmf209.sty feynmf.mf $(MANPICS)
	-$(LATEX209) $*.drv
	$(RUN_METAFONT)
	-$(LATEX209) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF209)

feynmp.dvi: feynmf.dtx feynmp.drv feynmp.sty feynmp.mp $(MANPICS)
	-$(LATEX) $*.drv
	$(RUN_METAPOST)
	-$(LATEX) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF)

feynmp209.dvi: feynmf.dtx feynmp209.drv feynmp209.sty feynmp.mp $(MANPICS)
	-$(LATEX209) $*.drv
	$(RUN_METAPOST)
	-$(LATEX209) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF209)

fmfman.dvi: feynmf.dtx fmfman.drv feynmf.sty feynmf.mf $(MANPICS)
	-$(LATEX) $*.drv
	$(RUN_METAFONT)
	-$(LATEX) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF)

fmfman209.dvi: feynmf.dtx fmfman209.drv feynmf209.sty feynmf.mf $(MANPICS)
	-$(LATEX209) $*.drv
	$(RUN_METAFONT)
	-$(LATEX209) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF209)

fmfmanps.dvi: feynmf.dtx fmfmanps.drv feynmp.sty feynmp.mp $(MANPICS)
	-$(LATEX) $*.drv
	$(RUN_METAPOST)
	-$(LATEX) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF)

fmfman209ps.dvi: feynmf.dtx fmfman209ps.drv feynmp209.sty feynmp.mp $(MANPICS)
	-$(LATEX209) $*.drv
	$(RUN_METAPOST)
	-$(LATEX209) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF209)

manual.ps.gz: manual.ps
	gzip < $< > $@

manual.ps: fmfmanps.dvi $(MANPICS)
	dvips -o $@ $<

manual209.ps: fmfman209ps.dvi $(MANPICS)
	dvips -o $@ $<

manpics.1: manpics.mp
	-mp $<

manpics.2 manpics.3: manpics.1

feynmf.1: feynmf.pl
	pod2man --section 1 \
	        --release "FeynMF Version $(VERSION).$(RELEASE)$(STATUS)" \
	        --center "Contributed LaTeX Utilities" $< > $@

clean:
	rm -f fmfsamp?.* \
	      *.tfm *.*gf *.*pk \
	      *.log *.t[1-9] *.t[1-9][0-9] *.t[12][0-9][0-9] \
	      *.dvi *.aux *.toc *.ilg *.glo *.gls *.idx *.ind \
	      *.ps *.mpx '#*#' *~ .*~

realclean: clean
	rm -f feynmf.mf feynmf.sty feynmf.drv feynmp.* fmfman* \
	      feynmf209.sty feynmf209.drv feynmp209.*

distclean: realclean

########################################################################
# Maintenance:

DISTFILES = /usr/local/etc/COPYING README Makefile feynmf.dtx \
	    feynmf.ins feynmf209.ins manpics.mp $(MANPICS) \
	    feynmf.pl template.tex

distdir = feynmf-$(VERSION).$(RELEASE)$(STATUS)
CVSTAG = FEYNMF_$(VERSION)_$(RELEASE)$(STATUS)
TEXTAG = v$(VERSION).$(RELEASE)
M = 

fileversion:
	perl -pe \
	  's/^\\def\\fileversion\{.*\}/\\def\\fileversion{$(TEXTAG)}/;' \
	  feynmf.dtx > feynmf.vtmp
	if cmp -s feynmf.dtx feynmf.vtmp; then \
	  rm -f feynmf.vtmp; \
	else \
	  mv feynmf.vtmp feynmf.dtx; \
	fi
	
commit: fileversion
	@if test -n "$(M)"; then \
	  echo "cvs commit -m '$(M)'"; cvs commit -m '$(M)'; \
	  echo "cvs tag $(CVSTAG)"; cvs tag $(CVSTAG); \
	  echo "cvs tag -b $(CVSTAG)_"; cvs tag -b $(CVSTAG)_; \
	else \
	  echo "usage: make commit M='<message>'" 1>&2; \
	fi

dist: $(distdir).tar.gz
snap: feynmf-current.tar.gz

$(distdir).tar.gz:
	rm -fr $(distdir) $(distdir).tmp
	cvs export -r $(CVSTAG) -d $(distdir).tmp feynmf
	mkdir $(distdir)
	(cd ./$(distdir).tmp && \
         make $(DISTFILES) && \
         cp $(DISTFILES) ../$(distdir))
	tar cf - $(distdir) | gzip > $@
	rm -fr $(distdir) $(distdir).tmp

feynmf-current.tar.gz: $(DISTFILES) fileversion
	rm -fr feynmf-current
	mkdir feynmf-current
	touch feynmf-current/1_THIS_IS_A_SNAPSHOT_OF_
	touch feynmf-current/2_WORK_IN_PROGRESS_AND__
	touch feynmf-current/3_NOT_YET_RELEASED_CODE_
	cp $(DISTFILES) feynmf-current
#	perl -pe \
#	  's/\[\\filedate/[(UNRELEASED and UNSUPPORTED snapshot)/;' \
	  feynmf.dtx > feynmf-current/feynmf.dtx
	tar cf - feynmf-current | gzip > $@
	rm -fr feynmf-current

########################################################################
# Local Variables:
# mode:text
# End:


==> _diagrams/feynmf/README <==
# $Id: README,v 1.30 1996/12/02 01:38:45 ohl Exp $
########################################################################

    This is feynmf, a combined LaTeX/Metafont package for easy drawing
    of professional quality Feynman diagrams.  feynmf lays out most
    diagrams satisfactorily from the structure of the graph without
    any need for manual intervention.  Nevertheless all the power of
    Metafont is available for more obscure cases.  See the
    documentation for appetizers, examples and more details.

    A preformatted manual (`manual.ps.gz') is provided to wet your
    appetite with numerous examples.

    Anyway, you are invited to share, use, abuse, and improve it, see
    the file COPYING for details.

    Enjoy,
    -Thorsten

########################################################################

   Installation:

   You need a recent LaTeX (LaTeX2e, as of December 1994 is
   sufficient) to use feynmf,  docstrip.tex to install it and doc.sty
   to typeset the documentation.  If it is not already on your system,
   you can get all this (and much more) from your nearest CTAN host.

   To install, either use the Makefile or use the installation file
   feynmf.ins:

     $ latex feynmf.ins

   then you can typeset the documentation by

     $ latex fmfman.drv
     $ mf '\mode:=laserjet; input fmfsamp1'
     $ mf '\mode:=laserjet; input fmfsamp2'
     $ mf '\mode:=laserjet; input fmfsamp3'
     $ mf '\mode:=laserjet; input fmfsamp4'
     $ latex fmfman.drv
     $ makeindex -s gind.ist -o fmfman.ind fmfman.idx
     $ makeindex -s gglo.ist -o fmfman.gls fmfman.glo
     $ latex fmfman.drv

   or by using the Makefile (`make man').  That's it.

   There is also a simple example `template.tex' that you can use as
   a template for your own creations.  To typeset, either use the
   feynmf script

     $ feynmf template

   or run Metafont manually

     $ latex template
     $ mf '\mode:=localfont; input fmftempl'
     $ latex template

   Finally, there is another installation file for LaTeX 2.09 compatible
   versions: feynmf209.ins.  This file has to be processed _in addition_
   to feynmf.ins!

########################################################################

WARNING:

    If LaTeX fails with `Unknown graphics extension: 3', you have a
    slightly out-of-date graphics.sty file (LaTeX will have issued a
    warning in this case).  There has been a change to the user
    interface, which makes it very hard to support both versions.
    Sorry.  I have chosen to support the current one, which will
    hopefully be stable.

    You can work around this by either getting a more recent graphics
    package from CTAN (macros/latex/packages/graphics) or by using
    epsf.sty instead (`\let\includegraphics\epsffile\input epsf.sty').
    [You can also ignore it and get the preformatted manual.  But you
    will not be able to use the MetaPost version in this case.]

########################################################################

    Comments, bug reports and improvements are welcome at:

        Thorsten.Ohl@Physik.TH-Darmstadt.de
        (aka: ohl@crunch.ikp.physik.th-darmstadt.de)

    New versions can be found in:

        crunch.ikp.physik.th-darmstadt.de:/pub/ohl/feynmf

    or at CTAN:

        {ftp.shsu.edu,ftp.tex.ac.uk,ftp.dante.de}:
          ... macros/latex/contrib/supported/feynmf

    There are two mailing lists

        feynmf-announce@crunch.ikp.physik.th-darmstadt.de
        feynmf-bugs@crunch.ikp.physik.th-darmstadt.de

    both are open for subscription.  The former should be very low
    volume and carry only important announcements.  The latter can
    serve as a more general discussion forum.

    To subscribe, send mail to

        majordomo@crunch.ikp.physik.th-darmstadt.de

    and NOT to the lists itself.  The following commands (on a line in
    the body of the mail, not in the subject) are useful: `subscribe
    feynmf-announce', `unsubscribe feynmf-bugs', `help', etc.

########################################################################

NEWS for Version 1.08

    *  Improved very short gluon and photon propagators by relaxing
    overly aggressive rounding.

    *  New (still experimental) `feynmf' script automating the
    invocation of Metafont (requires perl(1)).

NEWS for Version 1.07

    *  Switch off I/O during the first pass in AMS-LaTeX equation
    environments.  This avoids a nasty race condition (thanks to Axel
    Thimm for reporting this bug).  A beneficial side effect is that
    it saves us 50% processing time in these cases.

NEWS for Version 1.06

    *  New abstraction: polygons.  Useful for complex vertices in
    non-perturbative diagrams.

    *  New commands: \fmfpoly, \fmfpolyn and \fmfrpolyn, implementing
    polygons.

    *  New option `rubout' for crossing propagators.

    *  Some common typos are detected are appropriate warning messages
    are issued.

    *  New options `errorstop', `scroll', `nonstop' and `batch' for
    specifying the desired interactionmode.

    *  Work around an obscure babel/german/feynmf three way
    destructive interference.

NEWS for Version 1.05

    *  FeynMF now coexists with french.sty and other packages that
    change the \catcode of ``:''.

    *  Fixed a bug introduced in version 1.03, which could cause
    problems with font loading.  Unfortunately, the fix has to give up
    some compatibility with earlier versions.  Sources for version
    1.02 and earlier which used \noexpand in labels have to upgraded
    or the option `pre-1.03' has to be used.  Sorry.

NEWS for Version 1.04

    *  Finally, \fmffixed{(dx,whatever)}{v1,v2} and
    \fmffixed{(whatever,dy)}{v1,v2} do what you would expect them
    to.  \fmffixedx and \fmffixedy are new synonyms for those.

NEWS for Version 1.03

    *  It is no longer necessary to protect TeX command sequences with
    \noexpand.  Old files using \noexpand will continue to work.

NEWS for Version 1.02

    *  Read the .tfm file before writing the .mf file destructively.
    This should allow a transparent two pass processing if MakeTeXTFM
    is enabled.  Thanks to Thomas Esser <te@informatik.uni-hannover.de> 
    for the suggestion.

NEWS for Version 1.01

    * new decoration shapes for vertices by popular demand: `cross'
    (also `triacross', `pentacross' and `hexacross').

    * fixed a rounding bug in cut-off ends (noticeable as a spurious
    thin diagonal line at the left end of double lines).

    * The maximum size for shaded and hatched areas has been doubled
    by removing an obsolete speedup hack that was not used anymore.

    * In an unrelated move, shading and hatching has been
    reimplemented in a much more general fashion.  Now arbitray
    tilings can be specified as argument to `decoration.filled='.  The
    old style numerical arguments continue to work, but should be
    replaced by `empty', `full', `shaded', and `hatched' in new
    documents.

########################################################################
# Local Variables:
# mode:indented-text
# End:


==> _diagrams/feynmf/compile <==
#make clean
#latex $1
##mf '\mode:=localfont; input fmftempl' 
#mf '\mode:=localfont; input feyngraph'
#latex $1
#pdflatex $1
#latex $1
#pdflatex $1

#pdflatex $1
#sh $1.out
#pdflatex $1
#open template.pdf

rm template.aux  
rm template.fdb_latexmk  
rm template.log  
rm template.pdf*
rm template.dvi  
rm template.fls
rm template.out
rm feyngraph.t1
rm feyngraph.1 
pdflatex -shell-escape $1
pdflatex -shell-escape $1

==> _diagrams/feynmf/feynmf.1 <==
.\" Automatically generated by Pod::Man 4.10 (Pod::Simple 3.35)
.\"
.\" Standard preamble:
.\" ========================================================================
.de Sp \" Vertical space (when we can't use .PP)
.if t .sp .5v
.if n .sp
..
.de Vb \" Begin verbatim text
.ft CW
.nf
.ne \\$1
..
.de Ve \" End verbatim text
.ft R
.fi
..
.\" Set up some character translations and predefined strings.  \*(-- will
.\" give an unbreakable dash, \*(PI will give pi, \*(L" will give a left
.\" double quote, and \*(R" will give a right double quote.  \*(C+ will
.\" give a nicer C++.  Capital omega is used to do unbreakable dashes and
.\" therefore won't be available.  \*(C` and \*(C' expand to `' in nroff,
.\" nothing in troff, for use with C<>.
.tr \(*W-
.ds C+ C\v'-.1v'\h'-1p'\s-2+\h'-1p'+\s0\v'.1v'\h'-1p'
.ie n \{\
.    ds -- \(*W-
.    ds PI pi
.    if (\n(.H=4u)&(1m=24u) .ds -- \(*W\h'-12u'\(*W\h'-12u'-\" diablo 10 pitch
.    if (\n(.H=4u)&(1m=20u) .ds -- \(*W\h'-12u'\(*W\h'-8u'-\"  diablo 12 pitch
.    ds L" ""
.    ds R" ""
.    ds C` ""
.    ds C' ""
'br\}
.el\{\
.    ds -- \|\(em\|
.    ds PI \(*p
.    ds L" ``
.    ds R" ''
.    ds C`
.    ds C'
'br\}
.\"
.\" Escape single quotes in literal strings from groff's Unicode transform.
.ie \n(.g .ds Aq \(aq
.el       .ds Aq '
.\"
.\" If the F register is >0, we'll generate index entries on stderr for
.\" titles (.TH), headers (.SH), subsections (.SS), items (.Ip), and index
.\" entries marked with X<> in POD.  Of course, you'll have to process the
.\" output yourself in some meaningful fashion.
.\"
.\" Avoid warning from groff about undefined register 'F'.
.de IX
..
.nr rF 0
.if \n(.g .if rF .nr rF 1
.if (\n(rF:(\n(.g==0)) \{\
.    if \nF \{\
.        de IX
.        tm Index:\\$1\t\\n%\t"\\$2"
..
.        if !\nF==2 \{\
.            nr % 0
.            nr F 2
.        \}
.    \}
.\}
.rr rF
.\"
.\" Accent mark definitions (@(#)ms.acc 1.5 88/02/08 SMI; from UCB 4.2).
.\" Fear.  Run.  Save yourself.  No user-serviceable parts.
.    \" fudge factors for nroff and troff
.if n \{\
.    ds #H 0
.    ds #V .8m
.    ds #F .3m
.    ds #[ \f1
.    ds #] \fP
.\}
.if t \{\
.    ds #H ((1u-(\\\\n(.fu%2u))*.13m)
.    ds #V .6m
.    ds #F 0
.    ds #[ \&
.    ds #] \&
.\}
.    \" simple accents for nroff and troff
.if n \{\
.    ds ' \&
.    ds ` \&
.    ds ^ \&
.    ds , \&
.    ds ~ ~
.    ds /
.\}
.if t \{\
.    ds ' \\k:\h'-(\\n(.wu*8/10-\*(#H)'\'\h"|\\n:u"
.    ds ` \\k:\h'-(\\n(.wu*8/10-\*(#H)'\`\h'|\\n:u'
.    ds ^ \\k:\h'-(\\n(.wu*10/11-\*(#H)'^\h'|\\n:u'
.    ds , \\k:\h'-(\\n(.wu*8/10)',\h'|\\n:u'
.    ds ~ \\k:\h'-(\\n(.wu-\*(#H-.1m)'~\h'|\\n:u'
.    ds / \\k:\h'-(\\n(.wu*8/10-\*(#H)'\z\(sl\h'|\\n:u'
.\}
.    \" troff and (daisy-wheel) nroff accents
.ds : \\k:\h'-(\\n(.wu*8/10-\*(#H+.1m+\*(#F)'\v'-\*(#V'\z.\h'.2m+\*(#F'.\h'|\\n:u'\v'\*(#V'
.ds 8 \h'\*(#H'\(*b\h'-\*(#H'
.ds o \\k:\h'-(\\n(.wu+\w'\(de'u-\*(#H)/2u'\v'-.3n'\*(#[\z\(de\v'.3n'\h'|\\n:u'\*(#]
.ds d- \h'\*(#H'\(pd\h'-\w'~'u'\v'-.25m'\f2\(hy\fP\v'.25m'\h'-\*(#H'
.ds D- D\\k:\h'-\w'D'u'\v'-.11m'\z\(hy\v'.11m'\h'|\\n:u'
.ds th \*(#[\v'.3m'\s+1I\s-1\v'-.3m'\h'-(\w'I'u*2/3)'\s-1o\s+1\*(#]
.ds Th \*(#[\s+2I\s-2\h'-\w'I'u*3/5'\v'-.3m'o\v'.3m'\*(#]
.ds ae a\h'-(\w'a'u*4/10)'e
.ds Ae A\h'-(\w'A'u*4/10)'E
.    \" corrections for vroff
.if v .ds ~ \\k:\h'-(\\n(.wu*9/10-\*(#H)'\s-2\u~\d\s+2\h'|\\n:u'
.if v .ds ^ \\k:\h'-(\\n(.wu*10/11-\*(#H)'\v'-.4m'^\v'.4m'\h'|\\n:u'
.    \" for low resolution devices (crt and lpr)
.if \n(.H>23 .if \n(.V>19 \
\{\
.    ds : e
.    ds 8 ss
.    ds o a
.    ds d- d\h'-1'\(ga
.    ds D- D\h'-1'\(hy
.    ds th \o'bp'
.    ds Th \o'LP'
.    ds ae ae
.    ds Ae AE
.\}
.rm #[ #] #H #V #F C
.\" ========================================================================
.\"
.IX Title "FEYNMF 1"
.TH FEYNMF 1 "2008-02-21" "FeynMF Version 1.08" "Contributed LaTeX Utilities"
.\" For nroff, turn off justification.  Always turn off hyphenation; it makes
.\" way too many mistakes in technical documents.
.if n .ad l
.nh
.SH "NAME"
feynmf \- Process LaTeX files using FeynMF
.SH "SYNOPSIS"
.IX Header "SYNOPSIS"
\&\fBfeynmf\fR [\fB\-hvqncfT\fR] [\fB\-t\fR \fItfm\fR [\fB\-t\fR \fItfm\fR ...]] [\fB\-m\fR \fImode\fR]
       \fIfile\fR [\fIfile\fR ...]
.PP
\&\fBfeynmf\fR [\fB\-\-help\fR] [\fB\-\-version\fR] [\fB\-\-quiet\fR] [\fB\-\-noexec\fR] [\fB\-\-clean\fR]
       [\fB\-\-force\fR] [\fB\-\-notfm\fR] [\fB\-\-tfm\fR \fItfm\fR [\fB\-\-tfm\fR \fItfm\fR ...]]
       [\fB\-\-mode\fR \fImode\fR] \fIfile\fR [\fIfile\fR ...]
.SH "DESCRIPTION"
.IX Header "DESCRIPTION"
The most complicated part of using the \fBFeynMF\fR style appears to be the
proper invocation of \fBMetafont\fR.  The \fBfeynmf\fR script provides a
convenient front end and will automagically invoke \fBMetafont\fR with the
proper mode and magnifincation.  It will also avoid cluttering system font
directories and offers an option to clean them.
.SH "OPTIONS"
.IX Header "OPTIONS"
.IP "\fB\-h\fR, \fB\-\-help\fR" 4
.IX Item "-h, --help"
Print a short help text.
.IP "\fB\-v\fR, \fB\-\-version\fR" 4
.IX Item "-v, --version"
Print the version of \fBfeynmf\fR.
.IP "\fB\-q\fR, \fB\-\-quiet\fR" 4
.IX Item "-q, --quiet"
Don't echo the commands being executed.
.IP "\fB\-n\fR, \fB\-\-noexec\fR" 4
.IX Item "-n, --noexec"
Don't execute \fBLaTeX\fR or \fBMetafont\fR.
.IP "\fB\-c\fR, \fB\-\-clean\fR" 4
.IX Item "-c, --clean"
Offer to delete font files that have accidentally been placed in a
system directory by the \fBMakeTeXTFM\fR and \fBMakeTeXPK\fR scripts (these
scripts are run by \fBtex\fR (and \fBlatex\fR) in the background).  This
option has only been tested with recent versions of \s-1UNIX\s0 TeX.
.IP "\fB\-f\fR, \fB\-\-force\fR" 4
.IX Item "-f, --force"
Don't ask any questions.
.IP "\fB\-T\fR, \fB\-\-notfm\fR" 4
.IX Item "-T, --notfm"
Don't try to prepare fake \f(CW\*(C`.tfm\*(C'\fR files for the first run.
.IP "\fB\-t\fR, \fB\-\-tfm\fR \fItfm\fR" 4
.IX Item "-t, --tfm tfm"
Don't try guess the names of the \f(CW\*(C`.tfm\*(C'\fR files to fake for
the first run and use the given name(s) instead.  This option
can be useful if our incomplete parsing of the LaTeX input
files fails.
.IP "\-\fBm\fR \fImode\fR, \fB\-\-mode\fR \fImode\fR" 4
.IX Item "-m mode, --mode mode"
Select the \s-1METAFONT\s0 mode \fImode\fR.  The default is guessed or
\&\f(CW\*(C`localfont\*(C'\fR if the guess fails.
.IP "\fIfile\fR" 4
.IX Item "file"
Main \fBLaTeX\fR input files.
.IP "\fIfile\fR ..." 4
.IX Item "file ..."
Other LaTeX input files that are included by the main file.
.SH "AUTHOR"
.IX Header "AUTHOR"
Thorsten Ohl <Thorsten.Ohl@Physik.TH\-Darmstadt.de>
.SH "BUGS"
.IX Header "BUGS"
The preparation of \f(CW\*(C`.tfm\*(C'\fR files is not foolproof yet, because we can
parse \fBTeX\fR files only superficially.
.PP
This script has only been tested for recent \fBteTeX\fR distributions
of \s-1UNIX\s0 \fBTeX\fR, though it will probably work with other versions of
\&\s-1UNIX\s0 \fBTeX\fR.  The author will be grateful for portability suggestions,
even concerning \fBBorg\fR operating systems, for the benefit of those users
that are forced to live with \s-1DOS\s0 or Windows.


==> _diagrams/feynmf/graphs/DIS.tex <==
\large
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(160,140)
    \fmfleft{i1,ip,i2,il,i3}
    \fmfright{o1,x1,x2,x3,x4,o3,o3,o4,o5,ol,o5}
    \fmfset{arrow_len}{10}
    \fmf{phantom,tension=0.29}{vl,vp}
    % lepton
    \fmflabel{\textcolor{blue}{$\ell^-$}$\hspace{5pt}$
            \textcolor{red}{$\nu$}$\hspace{5pt}$
            \textcolor{forestgreen}{$\bar{\nu}$}}{il}
    \fmflabel{\textcolor{blue}{$\ell^-$}$\hspace{5pt}$
    \textcolor{red}{$\ell^-$}$\hspace{5pt}$
    \textcolor{forestgreen}{$\ell^+$}}{ol}
    \fmf{fermion,label=\textcolor{gray}{$k$}, label.side=left}{il,vl}
    \fmf{fermion,label=\textcolor{gray}{$k'$},label.side=left}{vl,ol}
    % proton
    \fmfv{l=$A$,l.a=180,l.d=10}{ip}
    \fmf{phantom}{ip,vp,x1}
    \fmffreeze
    \fmf{phantom}{ip,vp}
    \fmfi{fermion,label=\textcolor{gray}{$p$},label.side=left}
                  {vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 6)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 0)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4,-6)}
    % X
    \fmfv{l=\mybrace{80}$X$,l.d=20,l.a=-5}{x2}
    \fmfshift{12 left}{x1,x2,x3,x4}
    \fmf{phantom}{vp,x1} % to help \fmfi
    \fmf{phantom}{vp,x2} % to help \fmfi
    \fmf{phantom}{vp,x3} % to help \fmfi
    \fmf{phantom}{vp,x4} % to help \fmfi
    \fmfi{fermion}{vpath (__vp,__x1) scaled 1.08 shifted ( 0.0,-8.0)}
    \fmfi{fermion}{vpath (__vp,__x2) scaled 1.06 shifted ( 0.0,-2.0)}
    \fmfi{fermion}{vpath (__vp,__x3) scaled 1.04 shifted ( 0.0, 4.0)}
    \fmfv{decor.shape=circle,decor.filled=0,label.dist=0,label=$f^{A}_q$,background=white,decor.size=25}{vp}
    % photon & parton
    \fmf{photon,tension=1,label=\vspace{15pt}\hspace{5pt}\textcolor{blue}{$\text{Z}/\gamma^*$},label.side=right}{vl,v}
    \fmf{photon,tension=1,label=\vspace{-4pt}\textcolor{red}{$\text{W}^+$}$/$\textcolor{forestgreen}{$\text{W}^-$},label.side=left}{vl,v}
    \fmf{fermion,label=\textcolor{gray}{$xp$},label.side=right}{vp,v}
    \fmf{fermion}{v,o3}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/DIS_bulk.tex <==
%%---- DIS bulk
\large
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(160,100)
    \fmfleft{ip,il}
    \fmfright{x1,x2,x3,o1,o2,o3,o4,ol}
    \fmfset{arrow_len}{10}
    % lepton
    \fmflabel{$\text{e}^-$}{il}
    \fmflabel{$\text{e}^-$}{ol}
    \fmf{fermion,label=\textcolor{gray}{$k$}, label.side=left}{il,vl}
    \fmf{fermion,label=\textcolor{gray}{$k'$},label.side=left}{vl,ol}
    \fmf{phantom,tension=0.6}{vl,vp}
    % proton
    \fmfv{l=$\text{A}$,l.a=-160}{ip} % l.a = label.angle
    \fmf{phantom,tension=1}{ip,vp,x1}
    \fmffreeze
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01}
    \fmfi{fermion,label=\textcolor{gray}{$p$},label.side=left}
                  {vpath (__ip,__vp) scaled 1.01 shifted (-1.4, 6)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted ( 1.4,-6)}
    \fmfblob{25}{vp}
    % X
    \fmfv{l=\mybrace{40} $X$,l.a=10}{x2}
    \fmf{fermion}{vp,x1}
    \fmf{phantom}{vp,x2} % to help \fmfi
    \fmf{phantom}{vp,x3} % to help \fmfi
    \fmfi{fermion}{vpath (__vp,__x2) scaled 0.98 shifted (0,2.2)}
    \fmfi{fermion}{vpath (__vp,__x3) scaled 0.92 shifted (0,4.5)}
    \fmffreeze
    % photon
    \fmf{photon,label=\vspace{-4pt}\hspace{5pt}{\textcolor{gray}{$q$}},label.side=left}{vl,vp}
    % parton
    %\fmf{fermion,label=\textcolor{gray}{$x$},label.side=left}{vp,v}
    %\fmf{fermion}{v,o2}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/DIS_parton.tex <==
%---- DIS_parton
\large
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(160,100)
    \fmfleft{ip,il}
    \fmfright{x1,x2,x3,o1,o2,o3,o4,ol}
    \fmfset{arrow_len}{10}
    % lepton
    \fmflabel{$\text{e}^-$}{il}
    \fmflabel{$\text{e}^-$}{ol}
    \fmf{fermion,label=\textcolor{gray}{$k$}, label.side=left}{il,vl}
    \fmf{fermion,label=\textcolor{gray}{$k'$},label.side=left}{vl,ol}
    \fmf{phantom,tension=0.6}{vl,vp}
    % proton
    \fmfv{l=$\text{A}$,l.a=-160}{ip} % l.a = label.angle
    \fmf{phantom,tension=1}{ip,vp,x1}
    \fmffreeze
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01}
    \fmfi{fermion,label=\textcolor{gray}{$p$},label.side=left}
                  {vpath (__ip,__vp) scaled 1.01 shifted (-1.4, 6)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted ( 1.4,-6)}
    \fmfblob{25}{vp}
    % X
    \fmfv{l=\mybrace{75} $X$,l.a=10}{x2}
    \fmf{fermion}{vp,x1}
    \fmf{phantom}{vp,x2} % to help \fmfi
    \fmf{phantom}{vp,x3} % to help \fmfi
    \fmfi{fermion}{vpath (__vp,__x2) scaled 0.98 shifted (0,2.2)}
    \fmfi{fermion}{vpath (__vp,__x3) scaled 0.92 shifted (0,4.5)}
    \fmffreeze
    % photon
    \fmf{photon,label=\vspace{-4pt}\hspace{5pt}{\textcolor{gray}{$q$}},label.side=left}{vl,v}
    % parton
    \fmf{fermion,label=\textcolor{gray}{$\xi p$},label.side=left}{vp,v}
    \fmf{fermion}{v,o2}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/DIS_parton_nolabels.tex <==
%---- DIS_parton
\large
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(160,100)
    \fmfleft{ip,il}
    \fmfright{x1,x2,x3,o1,o2,o3,o4,ol}
    \fmfset{arrow_len}{10}
    % lepton
    %\fmflabel{$\text{e}^-$}{il}
    %\fmflabel{$\text{e}^-$}{ol}
    \fmf{fermion}{il,vl}
    \fmf{fermion}{vl,ol}
    \fmf{phantom,tension=0.6}{vl,vp}
    % proton
    %\fmfv{l=$\text{A}$,l.a=-160}{ip} % l.a = label.angle
    \fmf{phantom,tension=1}{ip,vp,x1}
    \fmffreeze
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-1.4, 6)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted ( 1.4,-6)}
    \fmfv{decor.shape=circle,decor.filled=0,background=white,decor.size=25}{vp}
    % X
    %\fmfv{l=\mybrace{75} $X$,l.a=10}{x2}
    \fmf{fermion}{vp,x1}
    \fmf{phantom}{vp,x2} % to help \fmfi
    \fmf{phantom}{vp,x3} % to help \fmfi
    \fmfi{fermion}{vpath (__vp,__x2) scaled 0.98 shifted (0,2.2)}
    \fmfi{fermion}{vpath (__vp,__x3) scaled 0.92 shifted (0,4.5)}
    \fmffreeze
    % photon
    \fmf{photon}{vl,v}
    % parton
    \fmf{fermion}{vp,v}
    \fmf{fermion}{v,o2}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/DY.tex <==
\large
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(160,160)
    \fmfleft{i1,iq,i2,ip,i3}
    \fmfright{y1,y2,y3,o1,f1,o2,o3,o4,f2,o5,x3,x2,x1}
    \fmfset{arrow_len}{10}
    % skeleton
    \fmf{phantom,tension=0.48}{vq,vp}
    \fmf{phantom}{ip,vp,x1}
    \fmf{phantom}{iq,vq,y1}
    \fmffreeze
    % parton
    \fmfv{l=$x_1p_1$,l.a=-90,l.d=22}{vp} % cheat: actually a line label
    \fmfv{l=$x_2p_2$,l.a=90,l.d=22}{vq} % cheat: actually a line label
    \fmf{fermion,tension=1.6}{vp,v}
    \fmf{fermion,tension=1.6}{v,vq}
    % hard process
    \fmfshift{20 right}{f1,f2}
    \fmfv{l=\textcolor{blue}{$\ell^-$}$\hspace{5pt}$
    \textcolor{red}{$\nu$}$\hspace{5pt}$
    \textcolor{forestgreen}{$\ell^-$}}{f2}

    \fmfv{l=\textcolor{blue}{$\ell^+$}$\hspace{5pt}$
            \textcolor{red}{$\ell^+$}$\hspace{5pt}$
            \textcolor{forestgreen}{$\bar{\nu}$}}{f1}
    \fmf{boson,tension=2,label=\textcolor{blue}{$\text{Z}/\gamma^*$},label.side=left}{v,vf}
    \fmf{boson,tension=2,label=\textcolor{red}{$\text{W}^+$}$/$\textcolor{forestgreen}{$\text{W}^-$},label.side=right}{v,vf} %$\text{W}$\textcolor{red}{$^+$}$^/$\textcolor{forestgreen}{$^-$}
    \fmf{fermion,tension=2}{f1,vf,f2}
    % proton 1
    \fmfv{l=$A_1$,l.a=180,l.d=10}{ip}
    \fmf{phantom}{ip,vp}
    \fmfi{fermion,l=\textcolor{gray}{$p_1$},l.s=left,l.d=8}
                  {vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 6)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 0)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4,-6)}
    % proton 2
    \fmfv{l=$A_2$,l.a=180,l.d=10}{iq}
    \fmf{phantom}{iq,vq}
    \fmfi{fermion}{vpath (__iq,__vq) scaled 1.01 shifted (-2.4, 6)}
    \fmfi{fermion}{vpath (__iq,__vq) scaled 1.01 shifted (-2.4, 0)}
    \fmfi{fermion,l=\textcolor{gray}{$p_2$},l.s=right,l.d=8}
                  {vpath (__iq,__vq) scaled 1.01 shifted (-2.4,-6)}
    % X 2
    \fmfshift{25 left}{x1}
    \fmfshift{20 left}{x2,x3}
    \fmf{phantom}{vp,x1} % to help \fmfi
    \fmf{phantom}{vp,x2} % to help \fmfi
    \fmf{phantom}{vp,x3} % to help \fmfi
    \fmfi{fermion}{vpath (__vp,__x1) scaled 1.0 shifted ( 0.0, 2.0)}
    \fmfi{fermion}{vpath (__vp,__x2) scaled 1.0 shifted ( 0.0, 0.0)}
    \fmfi{fermion}{vpath (__vp,__x3) scaled 1.0 shifted ( 0.0,-2.0)}
    \fmfv{decor.shape=circle,decor.filled=0,label.dist=0,label=$f^{A_1}_q$,background=white,decor.size=25}{vp}
    % X 2
    \fmfshift{25 left}{y1}
    \fmfshift{20 left}{y2,y3}
    \fmf{phantom}{vq,y1} % to help \fmfi
    \fmf{phantom}{vq,y2} % to help \fmfi
    \fmf{phantom}{vq,y3} % to help \fmfi
    \fmfi{fermion}{vpath (__vq,__y1) scaled 1.0 shifted ( 0.0,-2.0)}
    \fmfi{fermion}{vpath (__vq,__y2) scaled 1.0 shifted ( 0.0, 0.0)}
    \fmfi{fermion}{vpath (__vq,__y3) scaled 1.0 shifted ( 0.0, 2.0)}
    \fmfv{decor.shape=circle,decor.filled=0,label.dist=0,label=$f^{A_2}_q$,background=white,decor.size=25}{vq}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/DY_nolabels.tex <==
\large
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(160,160)
    \fmfleft{i1,iq,i2,ip,i3}
    \fmfright{y1,y2,y3,o1,f1,o2,o3,o4,f2,o5,x3,x2,x1}
    \fmfset{arrow_len}{10}
    % skeleton
    \fmf{phantom,tension=0.48}{vq,vp}
    \fmf{phantom}{ip,vp,x1}
    \fmf{phantom}{iq,vq,y1}
    \fmffreeze
    % parton
    %\fmfv{l=$x_1p_1$,l.a=-90,l.d=22}{vp} % cheat: actually a line label
    %\fmfv{l=$x_2p_2$,l.a=90,l.d=22}{vq} % cheat: actually a line label
    \fmf{fermion,tension=1.6}{vp,v}
    \fmf{fermion,tension=1.6}{v,vq}
    % hard process
    \fmfshift{20 right}{f1,f2}
    %\fmfv{l=\textcolor{blue}{$\ell^-$}$\hspace{5pt}$
    %\textcolor{red}{$\nu$}$\hspace{5pt}$
    %\textcolor{forestgreen}{$\ell^-$}}{f2}

    %\fmfv{l=\textcolor{blue}{$\ell^+$}$\hspace{5pt}$
    %        \textcolor{red}{$\ell^+$}$\hspace{5pt}$
    %        \textcolor{forestgreen}{$\bar{\nu}$}}{f1}
    \fmf{boson,tension=2}{v,vf}
    \fmf{boson,tension=2}{v,vf} %$\text{W}$\textcolor{red}{$^+$}$^/$\textcolor{forestgreen}{$^-$}
    \fmf{fermion,tension=2}{f1,vf,f2}
    % proton 1
    %\fmfv{l=$A_1$,l.a=180,l.d=10}{ip}
    \fmf{phantom}{ip,vp}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 6)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 0)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4,-6)}
    % proton 2
    %\fmfv{l=$A_2$,l.a=180,l.d=10}{iq}
    \fmf{phantom}{iq,vq}
    \fmfi{fermion}{vpath (__iq,__vq) scaled 1.01 shifted (-2.4, 6)}
    \fmfi{fermion}{vpath (__iq,__vq) scaled 1.01 shifted (-2.4, 0)}
    \fmfi{fermion}{vpath (__iq,__vq) scaled 1.01 shifted (-2.4,-6)}
    % X 2
    \fmfshift{25 left}{x1}
    \fmfshift{20 left}{x2,x3}
    \fmf{phantom}{vp,x1} % to help \fmfi
    \fmf{phantom}{vp,x2} % to help \fmfi
    \fmf{phantom}{vp,x3} % to help \fmfi
    \fmfi{fermion}{vpath (__vp,__x1) scaled 1.0 shifted ( 0.0, 2.0)}
    \fmfi{fermion}{vpath (__vp,__x2) scaled 1.0 shifted ( 0.0, 0.0)}
    \fmfi{fermion}{vpath (__vp,__x3) scaled 1.0 shifted ( 0.0,-2.0)}
    \fmfv{decor.shape=circle,decor.filled=0,background=white,decor.size=25}{vp}
    % X 2
    \fmfshift{25 left}{y1}
    \fmfshift{20 left}{y2,y3}
    \fmf{phantom}{vq,y1} % to help \fmfi
    \fmf{phantom}{vq,y2} % to help \fmfi
    \fmf{phantom}{vq,y3} % to help \fmfi
    \fmfi{fermion}{vpath (__vq,__y1) scaled 1.0 shifted ( 0.0,-2.0)}
    \fmfi{fermion}{vpath (__vq,__y2) scaled 1.0 shifted ( 0.0, 0.0)}
    \fmfi{fermion}{vpath (__vq,__y3) scaled 1.0 shifted ( 0.0, 2.0)}
    \fmfv{decor.shape=circle,decor.filled=0,background=white,decor.size=25}{vq}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/SIA.tex <==
\large
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(120,105)
    %\fmfset{arrow_len}{10}
    \fmfleft{i2,i1}
    \fmfright{o2,o1}
    \fmf{fermion,label=\textcolor{gray}{$k$}}{i1,v1}
    \fmf{fermion,label=\textcolor{gray}{$k'$}}{v1,i2}
    \fmf{fermion}{o2,v2,vf}
    \fmf{boson,label=\textcolor{black}{$\text{Z}/\gamma^*$},label.side=right}{v1,v2}
    \fmflabel{$\ell^-$}{i1}
    \fmflabel{$\ell^+$}{i2}
    \fmflabel{$\bar{q}$}{o2}
    \fmflabel{$q$}{o1}
    \fmfv{decor.shape=circle,decor.filled=0,label.dist=0,label=$D^h_q$,background=white,decor.size=25}{vf}
    \fmfv{l=$\pi^\pm$}{o1}
    \fmf{fermion,label=\textcolor{gray}{$p_h$},label.side=left}{vf,o1}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/SIA_NLO.tex <==
\large
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(160,140)
    \fmfleft{i0,i1,i2,i3}
    \fmfright{o1,x1,x2,x3,x4,o3,o3,o4,o5,ol,o5}
    \fmfset{arrow_len}{10}
    % lepton
    \fmflabel{\textcolor{blue}{$\ell^\mp$}}{i1}
    \fmflabel{\textcolor{blue}{$\ell^\pm$}}{i2}
    \fmf{fermion, label.side=right}{i1,ip}
    \fmf{phantom, label.side=right}{i2,ip}
    \fmf{fermion,label.side=right}{ip,i2}
    %\fmf{photon,label=\vspace{-5pt}\textcolor{blue}{$\text{Z}^0/\gamma^*$},label.side=right}{vph,vp}
   % \fmf{photon,tension=0.2}{vph,vp}
    % proton
    \fmf{phantom}{ip,vp,x2}
    \fmffreeze
    \fmf{photon,label=\vspace{-5pt}\textcolor{blue}{$\text{Z}^0/\gamma^*$},label.side=right}{ip,vp}
    %\fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 6)}
    %\fmfi{photon}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 0)}
    %\fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4,-6)}
    % X
    \fmfv{l=\mybrace{50}$X$,l.d=20,l.a=-2}{x2}
    % X
    \fmfshift{15 left}{x1,x2,x3,x4}
    \fmf{phantom}{vp,x1} % to help \fmfi
    \fmf{phantom}{vp,x2} % to help \fmfi
    \fmf{phantom}{vp,x3} % to help \fmfi
    \fmf{phantom}{vp,x4} % to help \fmfi
    \fmfi{fermion}{vpath (__vp,__x1) scaled 1.08 shifted ( 0.0,-10.0)}
    \fmfi{fermion}{vpath (__vp,__x2) scaled 1.06 shifted ( 0.0,-5.0)}
    \fmfi{fermion}{vpath (__vp,__x3) scaled 1.04 shifted ( 0.0, 0.0)}
    \fmfi{phantom}{vpath (__vp,__x4) scaled 1.02 shifted ( 0.0, 5.0)}
    \fmfblob{25}{vp}
    % photon & parton
    \fmf{fermion,label.side=left}{vp,vf}
    %https://tex.stackexchange.com/questions/163535/how-do-i-put-a-label-inside-a-feynman-diagram-circle
    \fmf{plain, left=1, tension=0.1}{vf,vf2}
    \fmf{plain, right=1, tension=0.1}{vf,vf2}
    \fmf{phantom,label.dist=0,label=$D^h_z$}{vf,vf2}
    \fmfv{l=$\text{h}$}{o3}
    \fmf{fermion}{vf2,o3}
    %\fmfblob{25}{vf}
    %\fmf{fermion}{o3,vf}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/SIDIS.tex <==
\large
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(160,140)
    \fmfleft{i1,ip,i2,il,i3}
    \fmfright{o1,x1,x2,x3,x4,o3,o3,o4,o5,ol,o5}
    \fmfset{arrow_len}{10}
    \fmf{phantom,tension=0.29}{vl,vp}
    % lepton
    \fmflabel{\textcolor{black}{$\ell$}}{il}
    \fmflabel{\textcolor{black}{$\ell$}}{ol}
    \fmf{fermion,label=\textcolor{gray}{$k$},label.side=left}{il,vl}
    \fmf{fermion,label=\textcolor{gray}{$k'$},label.side=left}{vl,ol}
    % proton
    \fmfv{l=$\text{p}$,l.a=180,l.d=10}{ip}
    \fmf{phantom}{ip,vp,x1}
    \fmffreeze
    \fmf{phantom}{ip,vp}
    \fmfi{fermion,label.side=left,label=\textcolor{gray}{$p$}}
                  {vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 6)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 0)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4,-6)}
    % X
    \fmfv{l=\mybrace{70}$X$,l.d=30,l.a=-15}{x3}
    \fmfshift{12 left}{x1,x2,x3,x4}
    \fmf{phantom}{vp,x1} % to help \fmfi
    \fmf{phantom}{vp,x2} % to help \fmfi
    \fmf{phantom}{vp,x3} % to help \fmfi
    \fmf{phantom}{vp,x4} % to help \fmfi
    \fmfi{fermion}{vpath (__vp,__x1) scaled 1.08 shifted ( 0.0,-8.0)}
    \fmfi{fermion}{vpath (__vp,__x2) scaled 1.06 shifted ( 0.0,-2.0)}
    \fmfi{fermion}{vpath (__vp,__x3) scaled 1.04 shifted ( 0.0, 4.0)}
    \fmfv{decor.shape=circle,decor.filled=0,label.dist=0,label=$f^p_q$,background=white,decor.size=25}{vp}
    % photon & parton
    \fmf{photon,tension=1,label=\textcolor{black}{$\text{Z}/\gamma^*$},label.side=right}{vl,v}
    \fmf{photon,tension=1}{vl,v}
    \fmf{fermion,label.side=right}{vp,v}
    \fmf{fermion}{v,vf}
    \fmfv{decor.shape=circle,decor.filled=0,label.dist=0,label=$D^h_q$,background=white,decor.size=25}{vf}
    \fmfv{l=$\pi^\pm$}{o3}
    \fmf{fermion,label=\textcolor{gray}{$p_h$},label.side=left}{vf,o3}
    %\fmfblob{25}{vf}
    %\fmf{fermion}{o3,vf}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/ep_scattering_ff.tex <==
%---- ep scattering + ff
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(100,80)
    \fmfleft{i1,i2}
    \fmfright{o1,o2}
    \fmflabel{$A$}{i1}
    \fmflabel{$e^-$}{i2}
    \fmflabel{$A$}{o1}
    \fmflabel{$e^-$}{o2}
    %\fmfblob{25}{v1}
    \fmf{fermion,label=\textcolor{gray}{$p$},label.side=right}{i1,v1}
    \fmf{fermion,label=\textcolor{gray}{$p'$},label.side=right}{v1,o1}
    \fmf{fermion,label=\textcolor{gray}{$k$},label.side=left}{i2,v2}
    \fmf{fermion,label=\textcolor{gray}{$k'$},label.side=left}{v2,o2}
    \fmf{photon,label=$\gamma$,label.side=left}{v1,v2}
    \fmf{photon,label=\textcolor{gray}{$q$},tension=0.1,label.side=right}{v1,v2}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/gamma_ff_vertex_LO.tex <==
%---- gamma ff vertex LO
\begin{fmffile}{feyngraph}
    \begin{fmfgraph*}(100,80)
      \fmfleft{i1,i2}
      \fmfright{o1,o2}
      \fmflabel{$f$}{i1}
      %\fmflabel{$e^-$}{i2}
      \fmflabel{$f$}{o1}
      %\fmflabel{$e^-$}{o2}
      \fmfblob{25}{v1}
      \fmf{fermion,label=\textcolor{gray}{$p$},label.side=right}{i1,v1}
      \fmf{fermion,label=\textcolor{gray}{$p'$},label.side=right}{v1,o1}
      \fmf{phantom,label.side=left}{i2,v2}
      \fmf{phantom,label.side=left}{v2,o2}
      \fmf{photon,label=$\gamma$,label.side=left}{v1,v2}
      \fmf{photon,label=\textcolor{gray}{$q$},tension=0.1,label.side=right}{v1,v2}
      \fmfv{d.sh=circle,d.f=1,d.si=5pt,l.s=left,l.a=60}{v2}
    \end{fmfgraph*}
  \end{fmffile}

==> _diagrams/feynmf/graphs/gamma_ff_vertex_LO_nolabels.tex <==
%---- gammaf vertex
\begin{fmffile}{feyngraph}
    \begin{fmfgraph*}(100,80)
      \fmfleft{i1,i2}
      \fmfright{o1,o2}
      %\fmflabel{$f$}{i1}
      %\fmflabel{$e^-$}{i2}
      %\fmflabel{$f$}{o1}
      %\fmflabel{$e^-$}{o2}
      \fmf{fermion,label.side=right}{i1,v1}
      %\fmf{fermion}{v1,v3}
      \fmf{fermion,label.side=right}{v1,o1}
      %\fmf{photon,tension=0.1,label.side=right}{v1,v3}
      \fmf{phantom,label.side=left}{i2,v4}
      \fmf{phantom,label.side=left}{v4,o2}
      \fmf{photon,label.side=left}{v1,v4}
      \fmf{photon,tension=0.1,label.side=right}{v1,v4}
      \fmfv{d.sh=circle,d.f=1,d.si=5pt,l.s=left,l.a=60}{v4}
    \end{fmfgraph*}
  \end{fmffile}

==> _diagrams/feynmf/graphs/gamma_ff_vertex_NLO.tex <==
%---- gammaf vertex correction (one loop)
\begin{fmffile}{feyngraph}
    \begin{fmfgraph*}(100,80)
      \fmfleft{i1,i2}
      \fmfright{o1,o2}
      %\fmflabel{$f$}{i1}
      %\fmflabel{$e^-$}{i2}
      %\fmflabel{$f$}{o1}
      %\fmflabel{$e^-$}{o2}
      \fmf{fermion,label.side=right}{i1,v1}
      \fmf{fermion}{v1,v2}
      \fmf{fermion}{v2,v3}
      \fmf{fermion,label.side=right}{v3,o1}
      \fmf{photon,tension=0.1,label.side=right}{v1,v3}
      \fmf{phantom,label.side=left}{i2,v4}
      \fmf{phantom,label.side=left}{v4,o2}
      \fmf{photon,label.side=left}{v2,v4}
      \fmf{photon,tension=0.1,label.side=right}{v2,v4}
      \fmfv{d.sh=circle,d.f=1,d.si=5pt,l.s=left,l.a=60}{v4}
    \end{fmfgraph*}
  \end{fmffile}

==> _diagrams/feynmf/graphs/gamma_ff_vertex_NLO_nolabels.tex <==
%---- gammaf vertex correction (one loop)
\begin{fmffile}{feyngraph}
    \begin{fmfgraph*}(100,80)
      \fmfleft{i1,i2}
      \fmfright{o1,o2}
      %\fmflabel{$f$}{i1}
      %\fmflabel{$e^-$}{i2}
      %\fmflabel{$f$}{o1}
      %\fmflabel{$e^-$}{o2}
      \fmf{fermion,label.side=right}{i1,v1}
      \fmf{fermion}{v1,v2}
      \fmf{fermion}{v2,v3}
      \fmf{fermion,label.side=right}{v3,o1}
      \fmf{photon,tension=0.1,label.side=right}{v1,v3}
      \fmf{phantom,label.side=left}{i2,v4}
      \fmf{phantom,label.side=left}{v4,o2}
      \fmf{photon,label.side=left}{v2,v4}
      \fmf{photon,tension=0.1,label.side=right}{v2,v4}
      \fmfv{d.sh=circle,d.f=1,d.si=5pt,l.s=left,l.a=60}{v4}
    \end{fmfgraph*}
  \end{fmffile}

==> _diagrams/feynmf/graphs/gamma_ff_vertex_blob.tex <==
%---- ep scattering + ff
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(100,80)
    \fmfleft{i1,i2}
    \fmfright{o1,o2}
    \fmflabel{$f$}{i1}
    %\fmflabel{$f$}{i2}
    \fmflabel{$f$}{o1}
    %\fmflabel{$f$}{o2}
    \fmfblob{25}{v1}
    \fmf{fermion,label=\textcolor{gray}{$p$},label.side=right}{i1,v1}
    \fmf{fermion,label=\textcolor{gray}{$p'$},label.side=right}{v1,o1}
    \fmf{phantom,label.side=left}{i2,v2}
    \fmf{phantom,label.side=left}{v2,o2}
    \fmf{photon,label=$\gamma$,label.side=left}{v1,v2}
    \fmf{photon,label=\textcolor{gray}{$q$},tension=0.1,label.side=right}{v1,v2}
    \fmfv{d.sh=circle,d.f=1,d.si=5pt,l.s=left,l.a=60}{v2}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/gamma_ff_vertex_self_energy_f_nolabels.tex <==
%---- gammaf vertex
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(100,80)
    \fmfleft{i1,i2}
    \fmfright{o1,o2}
    %\fmflabel{$f$}{i1}
    %\fmflabel{$e^-$}{i2}
    %\fmflabel{$f$}{o1}
    %\fmflabel{$e^-$}{o2}
    \fmf{fermion,label.side=right,tension=0.4}{i1,v1}
    \fmf{fermion}{v1,v2}
    \fmf{fermion}{v2,v3}
    \fmf{fermion,label.side=right}{v3,o1}
    \fmf{photon,right=1.0,tension=0.2,label.side=right}{v2,v3}
    \fmf{phantom,label.side=left}{i2,v4}
    \fmf{phantom,label.side=left}{v4,o2}
    \fmf{photon,label.side=left}{v1,v4}
    \fmf{photon,tension=0.1,label.side=right}{v1,v4}
    \fmfv{d.sh=circle,d.f=1,d.si=5pt,l.s=left,l.a=60}{v4}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/gamma_ff_vertex_self_energy_i_nolabels.tex <==
%---- gammaf vertex
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(100,80)
    \fmfleft{i1,i2}
    \fmfright{o1,o2}
    %\fmflabel{$f$}{i1}
    %\fmflabel{$e^-$}{i2}
    %\fmflabel{$f$}{o1}
    %\fmflabel{$e^-$}{o2}
    \fmf{fermion,label.side=right}{i1,v1}
    \fmf{fermion}{v1,v2}
    \fmf{fermion}{v2,v3}
    \fmf{fermion,label.side=right,tension=0.4}{v3,o1}
    \fmf{photon,right=1.0,tension=0.2,label.side=right}{v1,v2}
    \fmf{phantom,label.side=left}{i2,v4}
    \fmf{phantom,label.side=left}{v4,o2}
    \fmf{photon,label.side=left}{v3,v4}
    \fmf{photon,tension=0.1,label.side=right}{v3,v4}
    \fmfv{d.sh=circle,d.f=1,d.si=5pt,l.s=left,l.a=60}{v4}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/gamma_ff_vertex_vacuum_polarization_nolabels.tex <==
% vertex + vacuum polarization 
\begin{fmffile}{feyngraph}
      \begin{fmfgraph*}(100,80)
        \fmfleft{i1,i2}
        \fmfright{o1,o2}
        %\fmflabel{$f$}{i1}
        %\fmflabel{$e^-$}{i2}
        %\fmflabel{$f$}{o1}
        %\fmflabel{$e^-$}{o2}
        %\fmfblob{25}{v1}
        \fmf{fermion,label.side=right}{i1,v1}
        \fmf{fermion,label.side=right}{v1,o1}
        \fmf{phantom,label.side=left}{i2,v4}
        \fmf{phantom,label.side=left}{v4,o2}
        \fmf{photon,tension=1,label.side=right}{v1,v2}
        \fmf{photon,tension=1,label.side=right}{v3,v4}
        \fmf{fermion,left,tension=0.4}{v2,v3}
        \fmf{fermion,left,tension=0.4}{v3,v2}
        \fmfv{d.sh=circle,d.f=1,d.si=5pt,l.s=left,l.a=60}{v4}
      \end{fmfgraph*}
    \end{fmffile}

==> _diagrams/feynmf/graphs/jet0.tex <==
\large
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(160,160)
    \fmfleft{i1,iq,i2,ip,i3}
    \fmfright{y1,y2,y3,o1,f1,o2,o3,o4,f2,o5,x3,x2,x1}
    \fmfset{arrow_len}{10}
    % skeleton
    \fmf{phantom,tension=0.48}{vq,vp}
    \fmf{phantom}{ip,vp,x1}
    \fmf{phantom}{iq,vq,y1}
    \fmffreeze
    % parton
    \fmfv{l=$x_1p_1$,l.a=-90,l.d=22}{vp} % cheat: actually a line label
    \fmfv{l=$x_2p_2$,l.a=90,l.d=22}{vq} % cheat: actually a line label
    \fmf{dashes,tension=1.6}{vp,v}
    \fmf{dashes,tension=1.6}{v,vq}
    % hard process
    \fmfshift{20 right}{f1,f2}
    %\fmfv{l=\textcolor{blue}{$\ell^-$}$\hspace{5pt}$
    %\textcolor{red}{$\nu$}$\hspace{5pt}$
    %\textcolor{forestgreen}{$\ell^-$}}{f2}
%
    %\fmfv{l=\textcolor{blue}{$\ell^+$}$\hspace{5pt}$
    %        \textcolor{red}{$\ell^+$}$\hspace{5pt}$
    %        \textcolor{forestgreen}{$\bar{\nu}$}}{f1}
    \fmf{dashes,tension=2}{v,vf}
    \fmf{dashes,tension=2}{f1,vf,f2}
    % proton 1
    \fmfv{l=$A_1$,l.a=180,l.d=10}{ip}
    \fmf{phantom}{ip,vp}
    \fmfi{fermion,l=\textcolor{gray}{$p_1$},l.s=left,l.d=8}
                  {vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 6)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 0)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4,-6)}
    % proton 2
    \fmfv{l=$A_2$,l.a=180,l.d=10}{iq}
    \fmf{phantom}{iq,vq}
    \fmfi{fermion}{vpath (__iq,__vq) scaled 1.01 shifted (-2.4, 6)}
    \fmfi{fermion}{vpath (__iq,__vq) scaled 1.01 shifted (-2.4, 0)}
    \fmfi{fermion,l=\textcolor{gray}{$p_2$},l.s=right,l.d=8}
                  {vpath (__iq,__vq) scaled 1.01 shifted (-2.4,-6)}
    % X 2
    \fmfshift{25 left}{x1}
    \fmfshift{20 left}{x2,x3}
    \fmf{phantom}{vp,x1} % to help \fmfi
    \fmf{phantom}{vp,x2} % to help \fmfi
    \fmf{phantom}{vp,x3} % to help \fmfi
    \fmfi{fermion}{vpath (__vp,__x1) scaled 1.0 shifted ( 0.0, 2.0)}
    \fmfi{fermion}{vpath (__vp,__x2) scaled 1.0 shifted ( 0.0, 0.0)}
    \fmfi{fermion}{vpath (__vp,__x3) scaled 1.0 shifted ( 0.0,-2.0)}
    \fmfv{decor.shape=circle,decor.filled=0,label.dist=0,label=$f^{A_1}_q$,background=white,decor.size=25}{vp}
    % X 2
    \fmfshift{25 left}{y1}
    \fmfshift{20 left}{y2,y3}
    \fmf{phantom}{vq,y1} % to help \fmfi
    \fmf{phantom}{vq,y2} % to help \fmfi
    \fmf{phantom}{vq,y3} % to help \fmfi
    \fmfi{fermion}{vpath (__vq,__y1) scaled 1.0 shifted ( 0.0,-2.0)}
    \fmfi{fermion}{vpath (__vq,__y2) scaled 1.0 shifted ( 0.0, 0.0)}
    \fmfi{fermion}{vpath (__vq,__y3) scaled 1.0 shifted ( 0.0, 2.0)}
    \fmfv{decor.shape=circle,decor.filled=0,label.dist=0,label=$f^{A_2}_q$,background=white,decor.size=25}{vq}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/jet1.tex <==
\large
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(160,160)
    \fmfleft{i1,iq,i2,ip,i3}
    \fmfright{y1,y2,y3,o1,f1,o2,o3,o4,f2,o5,x3,x2,x1}
    \fmfset{arrow_len}{10}
    % skeleton
    \fmf{phantom,tension=0.48}{vq,vp}
    \fmf{phantom}{ip,vp,x1}
    \fmf{phantom}{iq,vq,y1}
    \fmffreeze
    % parton
    \fmfv{l=$x_1p_1$,l.a=-90,l.d=22}{vp} % cheat: actually a line label
    \fmfv{l=$x_2p_2$,l.a=90,l.d=22}{vq} % cheat: actually a line label
    \fmf{fermion,tension=1.6}{vp,v}
    \fmf{fermion,tension=1.6}{v,vq}
    % hard process
    \fmfshift{20 right}{f1,f2}
    %\fmfv{l=\textcolor{blue}{$\ell^-$}$\hspace{5pt}$
    %\textcolor{red}{$\nu$}$\hspace{5pt}$
    %\textcolor{forestgreen}{$\ell^-$}}{f2}
%
    %\fmfv{l=\textcolor{blue}{$\ell^+$}$\hspace{5pt}$
    %        \textcolor{red}{$\ell^+$}$\hspace{5pt}$
    %        \textcolor{forestgreen}{$\bar{\nu}$}}{f1}
    \fmf{gluon,tension=2}{v,vf}
    \fmf{gluon,tension=2}{f1,vf,f2}
    % proton 1
    \fmfv{l=$A_1$,l.a=180,l.d=10}{ip}
    \fmf{phantom}{ip,vp}
    \fmfi{fermion,l=\textcolor{gray}{$p_1$},l.s=left,l.d=8}
                  {vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 6)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4, 0)}
    \fmfi{fermion}{vpath (__ip,__vp) scaled 1.01 shifted (-2.4,-6)}
    % proton 2
    \fmfv{l=$A_2$,l.a=180,l.d=10}{iq}
    \fmf{phantom}{iq,vq}
    \fmfi{fermion}{vpath (__iq,__vq) scaled 1.01 shifted (-2.4, 6)}
    \fmfi{fermion}{vpath (__iq,__vq) scaled 1.01 shifted (-2.4, 0)}
    \fmfi{fermion,l=\textcolor{gray}{$p_2$},l.s=right,l.d=8}
                  {vpath (__iq,__vq) scaled 1.01 shifted (-2.4,-6)}
    % X 2
    \fmfshift{25 left}{x1}
    \fmfshift{20 left}{x2,x3}
    \fmf{phantom}{vp,x1} % to help \fmfi
    \fmf{phantom}{vp,x2} % to help \fmfi
    \fmf{phantom}{vp,x3} % to help \fmfi
    \fmfi{fermion}{vpath (__vp,__x1) scaled 1.0 shifted ( 0.0, 2.0)}
    \fmfi{fermion}{vpath (__vp,__x2) scaled 1.0 shifted ( 0.0, 0.0)}
    \fmfi{fermion}{vpath (__vp,__x3) scaled 1.0 shifted ( 0.0,-2.0)}
    \fmfv{decor.shape=circle,decor.filled=0,label.dist=0,label=$f^{A_1}_q$,background=white,decor.size=25}{vp}
    % X 2
    \fmfshift{25 left}{y1}
    \fmfshift{20 left}{y2,y3}
    \fmf{phantom}{vq,y1} % to help \fmfi
    \fmf{phantom}{vq,y2} % to help \fmfi
    \fmf{phantom}{vq,y3} % to help \fmfi
    \fmfi{fermion}{vpath (__vq,__y1) scaled 1.0 shifted ( 0.0,-2.0)}
    \fmfi{fermion}{vpath (__vq,__y2) scaled 1.0 shifted ( 0.0, 0.0)}
    \fmfi{fermion}{vpath (__vq,__y3) scaled 1.0 shifted ( 0.0, 2.0)}
    \fmfv{decor.shape=circle,decor.filled=0,label.dist=0,label=$f^{A_2}_q$,background=white,decor.size=25}{vq}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/jet_gg_gg.tex <==
%---- ep scattering + ff
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(100,100)
    \fmfleft{i1,i2}
    \fmfright{o1,o2}
    \fmf{gluon}{i1,v1,i2}
    \fmf{gluon}{o1,v2,o2}
    \fmf{gluon}{v1,v2}
    %\fmf{gluon,tension=0.1}{v1,v2}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/jet_gq_gq.tex <==
%---- ep scattering + ff
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(100,100)
    \fmfleft{i1,i2}
    \fmfright{o1,o2}
    \fmf{fermion}{i1,v1}
    \fmf{gluon}{v1,i2}
    \fmf{gluon}{o1,v2}
    \fmf{fermion}{v2,o2}
    \fmf{fermion}{v1,v2}
    %\fmf{gluon,tension=0.1}{v1,v2}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/jet_gq_qgamma.tex <==
%---- ep scattering + ff
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(100,100)
    \fmfleft{i1,i2}
    \fmfright{o1,o2}
    \fmf{fermion}{i1,v1}
    \fmf{gluon}{v1,i2}
    \fmf{photon}{o1,v2}
    \fmf{fermion}{v2,o2}
    \fmf{fermion}{v1,v2}
    %\fmf{gluon,tension=0.1}{v1,v2}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/jet_qq_g_qq.tex <==
%---- ep scattering + ff
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(100,100)
    \fmfleft{i1,i2}
    \fmfright{o1,o2}
    \fmf{fermion}{i1,v1,i2}
    \fmf{fermion}{o1,v2,o2}
    \fmf{photon}{v1,v2}
    %\fmf{gluon,tension=0.1}{v1,v2}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/jet_qq_gg.tex <==
%---- ep scattering + ff
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(100,100)
    \fmfleft{i1,i2}
    \fmfright{o1,o2}
    \fmf{fermion}{i1,v1,i2}
    \fmf{gluon}{o1,v2,o2}
    \fmf{gluon}{v1,v2}
    %\fmf{gluon,tension=0.1}{v1,v2}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/jet_qq_qq.tex <==
%---- ep scattering + ff
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(100,100)
    \fmfleft{i1,i2}
    \fmfright{o1,o2}
    \fmf{fermion}{i1,v1,i2}
    \fmf{fermion}{o1,v2,o2}
    \fmf{gluon}{v1,v2}
    %\fmf{gluon,tension=0.1}{v1,v2}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/self_energy.tex <==
%---- gammaf vertex
\begin{fmffile}{feyngraph}
  \begin{fmfgraph*}(100,80)
    \fmfleft{i1,i2}
    \fmfright{o1,o2}
    %\fmflabel{$f$}{i1}
    %\fmflabel{$e^-$}{i2}
    %\fmflabel{$f$}{o1}
    %\fmflabel{$e^-$}{o2}
    \fmf{fermion,label=\textcolor{gray}{$k$},label.side=right}{i1,v1}
    \fmf{fermion,label=\textcolor{gray}{$k-q$},label.side=left}{v1,v2}
    \fmf{fermion}{v2,o1}
    \fmf{photon,label=\textcolor{gray}{$q$},right=1.0,tension=0.2,label.side=right}{v1,v2}
  \end{fmfgraph*}
\end{fmffile}

==> _diagrams/feynmf/graphs/vacuum_pol.tex <==
% vacuum polarization 
\begin{fmffile}{feyngraph}
    \quad\parbox{100pt}{
      \begin{fmfgraph*}(100,80)
         \fmfleft{i}
         \fmfright{o}
         \fmfv{d.sh=circle,d.f=1,d.si=5pt,l.s=left,l=$\mu$,l.a=60}{i}
         \fmfv{d.sh=circle,d.f=1,d.si=5pt,l.s=right,l=$\nu$,l.a=120}{o}
         \fmf{photon,label=\textcolor{gray}{$q$}, tension=1}{i,v1} % ,label=H,label.side=left
         \fmf{photon,tension=1}{v2,o}
         \fmf{fermion,left,tension=0.4,label=\textcolor{gray}{$k+q$}}{v1,v2}
         \fmf{fermion,left,tension=0.4,label=\textcolor{gray}{$k$}}{v2,v1}
      \end{fmfgraph*}}
    \end{fmffile}

==> _inputs/MAPFF10/acknowledgements.tex <==
\section*{Acknowledgments}
We thank W. Vogelsang for confirming that the misprint in the
$C_{L,qg}^{(1),nm}$ expression reported in Ref.~\cite{Stratmann:2001pb}
was corrected in Ref.~\cite{Anderle:2012rq}, and
Rodolfo Sassot for helping us debug the {\tt APFEL++}
implementation and for providing us with the predictions of
Ref.~\cite{deFlorian:2014xna}. We are grateful to Gunar Schnell
for support with the interpretation of the HERMES data and to Nobuo Sato and
the JAM collaboration for providing us with their theoretical predictions,
PDF and FF sets. We thank J. Rojo for a critical reading of the paper. The work of R.~A.~K.
is partially supported by the Netherlands Organization for Scientific
Research (NWO). V.~B. is supported by the European Union's Horizon
2020 research and innovation programme under grant agreement
\textnumero~824093. E.~R.~N. is supported by the UK STFC grant
ST/T000600/1 and was also supported by the European Commission through
the Marie Sk\l odowska-Curie Action ParDHonSFFs.TMDs (grant number
752748).


==> _inputs/MAPFF10/sec-introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Unpolarised collinear fragmentation functions
(FFs)~\cite{Metz:2016swz} encode the non-perturbative mechanism,
called hadronisation, that leads a fast on-shell parton (a
quark or a gluon) to inclusively turn into a fast hadron moving along
the same direction. In the framework of quantum chromodynamics (QCD),
FFs are a fundamental ingredient to compute the cross section for any
process that involves the measurement of a hadron in the final
state. Among these processes are single-hadron production in
electron-positron annihilation (SIA), semi-inclusive deep-inelastic
scattering (SIDIS), and proton-proton collisions.

An analysis of the measurements for one or more of these processes allows for a
phenomenological determination of FFs. Measurements are compared to the
predictions obtained with a suitable parametrisation of the FFs, which is then
optimised to achieve the best global description possible. The determination
of the FFs has witnessed a remarkable progress in the last years, in particular
of the FFs of the pion, which is the most copiously produced hadron.
Three aspects have been investigated separately:
the variety of measurements analysed, the accuracy of the theoretical settings
used to compute the predictions, and the sophistication of the methodology
used to optimise FFs. In the first respect, global determinations of
FFs including recent measurements for all of the three processes
mentioned above have become available~\cite{deFlorian:2014xna};
in the second respect, determinations of FFs accurate to
next-to-next-to-leading order
(NNLO)~\cite{Anderle:2015lqa,Bertone:2017tyb} or including all-order
resummation~\cite{Anderle:2016czy} have been presented, albeit based
on SIA data only; in the third respect, determinations of FFs using
modern optimisation techniques that minimise parametrisation
bias~\cite{Bertone:2017tyb}, or attempting a simultaneous
determination of the parton distribution functions
(PDFs)~\cite{Moffat:2021dji}, have been performed. These three aspects
have also been investigated for the FFs of the
kaon~\cite{Sato:2016wqj, deFlorian:2017lwf,Bertone:2017tyb,Ethier:2017zbq,
  Sato:2019yez,Moffat:2021dji}.

This paper presents a determination of the FFs of charged pions,
called {\tt MAPFF1.0}, in which the most updated SIA and SIDIS
measurements are analysed to next-to-leading order (NLO) accuracy in
perturbative QCD. Our focus is on a proper statistical treatment of
experimental uncertainties and of their correlations in the
representation of FF uncertainties, and on the efficient minimisation
of model bias in the optimisation of the FF parametrisation. These
goals are achieved by means of a fitting methodology that is inspired
by the framework developed by the NNPDF Collaboration for the
determination of the proton
PDFs~\cite{Ball:2008by,Ball:2012cx,Ball:2014uwa,Ball:2017nwa,Nocera:2014gqa,
  Ball:2013lla}, nuclear
PDFs~\cite{AbdulKhalek:2019mzd,AbdulKhalek:2020yuc}, and
FFs~\cite{Bertone:2017tyb,Bertone:2018ecm}.  The framework combines
the Monte Carlo sampling method to map the probability density
distribution from the space of data to the space of FFs and neural
networks to parametrise the FFs with minimal bias.  In comparison to
previous work~\cite{Bertone:2017tyb,Bertone:2018ecm}, in this paper
the input data set is extended to SIDIS and the neural network is
optimised by means of a gradient descent algorithm that makes use of
the knowledge of the analytic derivatives of the neural network
itself~\cite{AbdulKhalek:2020uza}.

The structure of the paper is as follows. In Sect.~\ref{sec:data}, I
introduce the data sets used in this analysis, their features, and the
criteria applied to select the data points. In Sect.~\ref{sec:theory}, I discuss the setup used to compute the theoretical
predictions, focusing on the description of SIDIS multiplicities. In
Sect.~\ref{sec:methodology} I illustrate the methodological framework
adopted in our analysis, specifically the treatment of the
experimental uncertainties and the details of the neural network
parametrisation. In Sect.~\ref{sec:results}, I present the results of
our analysis where we assess the interplay between SIA and SIDIS data sets
and the stability of FFs upon variation of the kinematic
cuts. Finally, in Sect.~\ref{sec:conclusion}, I provide a summary of
our results and outline possible future developments.


==> _inputs/definitions.tex <==
\chapter*{Definitions and conventions}
\label{chap:Definitions}
\addcontentsline{toc}{chapter}{Definitions and conventions [To remove]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Troughout the plots in this thesis, Base colors are adopted for proton parton distribution functions (PDFs), their variant (as in modified) colors for nuclear PDFs (nPDFs), and different colors for Fragmentation functions (FFs) as displayed in the following figure:
%\begin{figure}[!h]
%    \begin{center}
%      \makebox[\textwidth]{\includegraphics[width=0.75\textwidth]{_plots/colors.pdf}%}
%  \end{center}
%\end{figure}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%All of which are generated by means of the following code:
%\begin{center}
%  \texttt{https://github.com/rabah-khalek/Compare\_LHAPDFsets}
%\end{center}

%\paragraph{Chapter.~\ref{chap:1}}
\begin{itemize}
    \item Restricting the $\bm{x}$ notation to a three-vector
    in space, we will use $x^\mu$ to designate the
    four-vector in space-time, where $x^\mu = (ct, \bm{x})$.
    \item $g_{\mu\nu} = \text{diag}(1, -1, -1, -1)$ is the
    Minkowski metric. Such that $x^\mu = (t,\bm{x})$ and $x_\mu = g_{\mu\nu} x^\nu = (t,-\bm{x})$
    \item $ds^2 = g_{\mu\nu} dx^\mu dx^\nu$ is the \textit{interval}\footnote{Interval: in special relativity,
an interval in Minkowski space is the equivalent of a
distance in Euclidean space.}
    interval for infinitesimal separations.
    \item $\epsilon_{ijk}$ is the Levi-Civita tensor equal
    to $1$ if $(i, j, k)$ is an even permutation of $(1, 2,
    3)$, $−1$ if it is an odd permutation, and $0$ if any
    index is repeated.
    \item $\gamma_E$ is the Euler-Mascheroni constant.
    \item $\alpha = \frac{e^2}{4\pi}$ is the Fine-structure constant.
%\paragraph{Chapter.~\ref{chap:2}}
    \item $\bm{D} \equiv \{D_1,D_2,...D_n\}$: set of correlated random variables of dimension $n$.
    \item $\bm{x} \equiv \{x_1,x_2,...x_n\}$: set of constants of dimension $n$ associated with $\bm{D}$ that could be seen as input of a function $x \mapsto D(x)$ such that $D(x_1) = D_1$ for instance. $x_i$ can be mutli-dimensional without loss of generality.
    \item $\bm{d} \equiv E(\bm{D}) \equiv \{d_1, d_2, ..., d_n\}$ is the associated set of expected values designating the data of dimension $n$.
    \item $\bm{\Sigma} \equiv cov(\bm{D})$ is the covariance matrix of dimension $n\times n$.
    \item $\bm{\theta} \equiv \{\theta_1, \theta_2, ..., \theta_m\}$: set of parameters of dimension $m$.
    \item $\bm{m(\theta)} \equiv \{m_1,m_2,...m_n\}$: set of values designating the model, a function that folds the parameters and maps the inputs $\bm{x}$ to data-space of dimension $n$. the model can be seen as well as $(x;\bm{\theta}) \mapsto m(x;\bm{\theta})$.
  \end{itemize}

==> _inputs/nNNPDF10/tables/tab-APFELvsFK.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}%[ht]
  \centering
  \small
     \renewcommand{\arraystretch}{1.65}
  \begin{tabular}{ccc|ccc|ccc} 
  \multirow{2.5}{*}{$A$} & \multirow{2.5}{*}{$x$} & \multirow{2.5}{*}{$Q^2$ (GeV$^2$)} &  \multicolumn{3}{c|}{FONLL-B (NLO)} &  \multicolumn{3}{c}{FONLL-C (NNLO)}\\ 
  & & & {\tt APFEL} & {\tt FK} & $\Delta_{\rm rel}~(\%)$  & {\tt APFEL} & {\tt FK} & $\Delta_{\rm rel}~(\%)$\\ [0.5ex] \toprule
  \multirow{5}{*}{12} 
  & 0.009 & 1.7  & 0.2895 & 0.2893 &  0.0694   &  0.2534 & 0.2534    &0.027\\ 
  & 0.013 & 2.3   & 0.3057 & 0.3052 & 0.1521  &     0.2837 & 0.283   & 0.228   \\ 
  & 0.13 & 14 &  0.27 & 0.2715 & 0.5642    &     0.2655 & 0.2647  &0.277       \\ 
  & 0.35 & 26 &  0.1292 & 0.1274 & 1.3683     &     0.1217 & 0.1213  &  0.308       \\ 
  & 0.65 & 42  & 0.0165 & 0.0168 & 1.8437  &      0.016 & 0.0163  & 2.347       \\
  \midrule
  \multirow{4}{*}{208} & 0.012 & 2.42 &  0.2795 & 0.279 & 0.1553       & 0.2581 & 0.2573  & 0.293      \\ 
  & 0.02 & 4.45 &   0.309 & 0.3103 & 0.3885     & 0.3041 & 0.3043      &0.084\\ 
  & 0.04 & 7.91 &   0.32 & 0.3214 & 0.3253     &  0.3181 & 0.3177     &0.104\\ 
  & 0.31 & 22.5 &   0.1467 & 0.1445 & 1.4583      &  0.1388 & 0.1382     &0.401 \\
 \bottomrule
  \end{tabular}
  \vspace{0.3cm}
  \caption{\small Comparison between the deep-inelastic structure function $F_2(x,Q^2,A)$
    computed with the {\tt APFEL} program and with the corresponding
    {\tt FK} interpolation tables.
    %
    The predictions are given for two different
    perturbative orders, FONLL-B and FONLL-C, and are computed 
    using the \texttt{EPPS16} nPDF set with theoretical settings described in the text.
    %
    The values of $x$ and $Q^2$ correspond to representative measurements
     for carbon ($A=12$) and lead ($A=208$) nuclei.
    %
    Also given are the relative differences between the two calculations, $\Delta_{\rm rel}\equiv
    |{\tt APFEL}-{\tt FK}|/{\tt APFEL}$.
  }
 \label{table:APFELvsFK} 
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> _inputs/nNNPDF10/tables/tab-chi2-L1CT.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}%[ht]
  \centering
  \small
   \renewcommand{\arraystretch}{1.55}
   \begin{tabular}{c c c | c | c }
     \multirow{2}{*}{Experiment} &
     \multirow{2}{*}{$~~~{\rm A}_1/{\rm A}_2~~~$} &
     \multirow{2}{*}{${N}_{\rm dat}$} & \multirow{2}{*}{$\chi^2/N_{\rm dat}$ (L1CT)} &
     \multirow{2}{*}{$\chi^2/N_{\rm dat}$ (prior)} \\
     & & & & \\
 \toprule
  SLAC E-139 & $^4$He/$^2$D & 3     &  0.94       &   2.61      \\
  NMC 95, re. & $^4$He/$^2$D & 13 &    1.83       &   1.17      \\
\midrule
  NMC 95 & $^6$Li/$^2$D & 12 &    0.97        &   0.87      \\
\midrule
  SLAC E-139 & $^9$Be/$^2$D & 3 &  0.66     &   0.09    \\
  NMC 96 & $^9$Be/$^{12}$C & 14 &     1.04    &  0.99       \\
\midrule
  EMC 88, EMC 90 & $^{12}$C/$^2$D & 12 &   0.45        &    0.47     \\
  SLAC E-139 & $^{12}$C/$^2$D & 2 &   0.52        &   0.80      \\
  NMC 95, NMC 95, re.   & $^{12}$C/$^2$D & 26 &   1.79       &  1.79       \\
  FNAL E665 & $^{12}$C/$^2$D & 3 &  1.07        &   0.84      \\
  NMC 95, re. & $^{12}$C/$^6$Li & 9 &  0.71        &    0.54     \\
\midrule
  BCDMS 85 & $^{14}$N/$^2$D & 9 &   0.81     &    0.77     \\
\midrule
  SLAC E-139  & $^{27}$Al/$^2$D & 3 &   2.42        &   3.14      \\
  NMC 96 & $^{27}$Al/$^{12}$C & 14 &  1.18     &   1.26      \\
\midrule
  SLAC E-139 & $^{40}$Ca/$^2$D & 2 &   1.24       &  1.36        \\
  NMC 95, re. & $^{40}$Ca/$^2$D & 12 &   2.07       &   1.87      \\
  EMC 90 & $^{40}$Ca/$^2$D & 3 &   3.18      &  3.23       \\
  FNAL E665 & $^{40}$Ca/$^2$D & 3 &   0.23      &   0.23      \\
  NMC 95, re. & $^{40}$Ca/$^6$Li & 9 &   0.46       &   0.41      \\
  NMC 96 & $^{40}$Ca/$^{12}$C & 23 &    1.22       &  1.20       \\
\midrule
  EMC 87 & $^{56}$Fe/$^2$D & 58 &     0.60      &   0.59     \\
  SLAC E-139 & $^{56}$Fe/$^2$D & 8 &   0.66        &   0.57      \\
  NMC 96 & $^{56}$Fe/$^{12}$C & 14 &   1.35        &   1.05      \\
  BCDMS 85, BCDMS 87 & $^{56}$Fe/$^2$D & 16 &   0.82       &   0.70      \\
\midrule
  EMC 88, EMC 93 & $^{64}$Cu/$^2$D & 27 &   1.32       &   1.38      \\
\midrule
  SLAC E-139 & $^{108}$Ag/$^2$D & 2 &   0.33        &    0.28     \\
\midrule
 EMC 88 & $^{119}$Sn/$^2$D & 8 &   0.12       &   0.13     \\
 NMC 96, $Q^2$ dependence & $^{119}$Sn/$^{12}$C & 119 &  0.95     &  0.98      \\
\midrule
 FNAL E665 & $^{131}$Xe/$^2$D & 4 &    0.99       &    0.84    \\
\midrule
  SLAC E-139 & $^{197}$Au/$^2$D & 3 &  0.21      &   0.31      \\
\midrule
 FNAL E665 & $^{208}$Pb/$^2$D & 3 &    1.29      &  1.31      \\
 NMC 96 & $^{208}$Pb/$^{12}$C & 14 &   0.98      &  0.90       \\
 \midrule
 \midrule
 {\bf Total} & & {\bf 451} &   1.03        &   1.00     \\
\bottomrule
\end{tabular}
\vspace{4mm}
\caption{\small The averaged values for $\chi^2/N_{\rm dat}$
  for each experiment in a Level 1 closure test compared with
  values obtained using the nCTEQ15 distributions.
  %
}
\label{tab:chi2table-L1CT}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> _inputs/nNNPDF10/tables/tab-eic.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}%[ht]
   \centering
   \renewcommand{\arraystretch}{1.75}
   \begin{tabular}{l|c|cc|cc|c}
     Scenario  & $A$   & $E_e$ &   $E_A/A$  &  $Q_{\rm max}^2$  &  $x_{\rm min}$ &$ N_{\rm dat}$ \\
 \toprule
     {\tt eRHIC\_5x50C} & 12  &   5 GeV &    50 GeV  &      440 GeV$^2$ &  0.003
     & 50 \\
     {\tt eRHIC\_5x75C} & 12  &   5 GeV &    75 GeV  &      440 GeV$^2$ &  0.002
     & 57 \\
        {\tt eRHIC\_5x100C} & 12  &   5 GeV &    100 GeV  &      780 GeV$^2$ &  0.001
        & 64 \\
    {\tt eRHIC\_5x50Au} & 197  &   5 GeV &    50 GeV  &      440 GeV$^2$ &  0.003
    & 50 \\
     {\tt eRHIC\_5x75Au} & 197  &   5 GeV &    75 GeV  &      440 GeV$^2$ &  0.002
     & 57 \\
       {\tt eRHIC\_5x100Au} & 197  &   5 GeV &    100 GeV  &    780  GeV$^2$ &  0.001
       & 64 \\
       \midrule
         {\tt eRHIC\_20x50C} & 12  &   20 GeV &    50 GeV  &    780 GeV$^2$ &  0.0008
     & 75 \\
     {\tt eRHIC\_20x75C} & 12  &   20 GeV &    75 GeV  &    780 GeV$^2$ &  0.0005
     & 79 \\
        {\tt eRHIC\_20x100C} & 12  &   20 GeV &    100 GeV  &   780 GeV$^2$ &  0.0003
        & 82 \\
             {\tt eRHIC\_20x50Au} & 197  &   20 GeV &    50 GeV  &    780 GeV$^2$ &  0.0008
     & 75 \\
     {\tt eRHIC\_20x75Au} & 197  &   20 GeV &    75 GeV  &   780 GeV$^2$ &  0.0005
     & 79 \\
        {\tt eRHIC\_20x100Au} & 197  &   20 GeV &    100 GeV  &    780 GeV$^2$ &  0.0003
        & 82 \\
     \bottomrule
   \end{tabular}
   \vspace{0.3cm}
   \caption{\label{tab:eicpseudodata}
  The different scenarios for the EIC pseudodata considered here.
     %
  For each scenario, we indicate the atomic mass number $A$, the electron energy
  $E_e$, the nucleus (per nucleon) energy $E_A/A$, the maximum value of $Q^2$ and
  the minimum value of $x$ reached, and the number of pseudodata points $N_{\rm dat}$.
  %
  The upper part of the table corresponds to the ``low energy'' scenario (with $E_e=5$ GeV)
  while the lower one to the ``high energy'' scenario (with $E_e=20$ GeV).
   }
 \end{table}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> _inputs/nNNPDF20/tables/tab-inputdata.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}%[ht]
  \centering
  \small
   \renewcommand{\arraystretch}{1.09}
\begin{tabular}{c c c c}
Experiment & ${\rm A}_1/{\rm A}_2$ & ${\rm N}_{\rm dat}$ & Reference\\
\toprule
  SLAC E-139 & $^4$He/$^2$D & 3 & \cite{Gomez:1993ri} \\
  NMC 95, re. & $^4$He/$^2$D & 13 & \cite{Amaudruz:1995tq}\\
\midrule
  NMC 95 & $^6$Li/$^2$D & 12 & \cite{Arneodo:1995cs}\\
\midrule
  SLAC E-139 & $^9$Be/$^2$D & 3 & \cite{Gomez:1993ri}\\
  NMC 96 & $^9$Be/$^{12}$C & 14 & \cite{Arneodo:1996rv}\\
\midrule
  EMC 88, EMC 90 & $^{12}$C/$^2$D & 12 & \cite{Ashman:1988bf,Arneodo:1989sy}\\
  SLAC E-139 & $^{12}$C/$^2$D & 2 & \cite{Gomez:1993ri}\\
  NMC 95, NMC 95, re.  & $^{12}$C/$^2$D & 26 & \cite{Arneodo:1995cs,Amaudruz:1995tq}\\
  FNAL E665 & $^{12}$C/$^2$D & 3 & \cite{Adams:1995is}\\
  NMC 95, re. & $^{12}$C/$^6$Li & 9 & \cite{Amaudruz:1995tq}\\
\midrule
  BCDMS 85 & $^{14}$N/$^2$D & 9 & \cite{Alde:1990im}\\
\midrule
  SLAC E-139 & $^{27}$Al/$^2$D & 3 & \cite{Gomez:1993ri}\\
  NMC 96 & $^{27}$Al/$^{12}$C & 14 & \cite{Arneodo:1996rv}\\
\midrule
  SLAC E-139 & $^{40}$Ca/$^2$D & 2 & \cite{Gomez:1993ri}\\
  NMC 95, re. & $^{40}$Ca/$^2$D & 12 & \cite{Amaudruz:1995tq}\\
  EMC 90 & $^{40}$Ca/$^2$D & 3 & \cite{Arneodo:1989sy}\\
  FNAL E665 & $^{40}$Ca/$^2$D & 3 & \cite{Adams:1995is}\\
  NMC 95, re. & $^{40}$Ca/$^6$Li & 9 & \cite{Amaudruz:1995tq}\\
  NMC 96 & $^{40}$Ca/$^{12}$C & 23 & \cite{Arneodo:1996rv}\\
\midrule
  EMC 87 & $^{56}$Fe/$^2$D & 58 & \cite{Aubert:1987da}\\
  SLAC E-139 & $^{56}$Fe/$^2$D & 8 & \cite{Gomez:1993ri}\\
  NMC 96 & $^{56}$Fe/$^{12}$C & 14 & \cite{Arneodo:1996rv}\\
  BCDMS 85, BCDMS 87 & $^{56}$Fe/$^2$D & 16 & \cite{Alde:1990im,Benvenuti:1987az}\\
\midrule
  EMC 88, EMC 93 & $^{64}$Cu/$^2$D & 27 & \cite{Ashman:1988bf,Ashman:1992kv}\\
\midrule
  SLAC E-139 & $^{108}$Ag/$^2$D & 2 & \cite{Gomez:1993ri}\\
\midrule
 EMC 88 & $^{119}$Sn/$^2$D & 8 & \cite{Ashman:1988bf}\\
 NMC 96, $Q^2$ dependence  & $^{119}$Sn/$^{12}$C & 119 & \cite{Arneodo:1996ru}\\
\midrule
 FNAL E665 & $^{131}$Xe/$^2$D & 4 & \cite{Adams:1992vm}\\
\midrule
  SLAC E-139 & $^{197}$Au/$^2$D & 3 & \cite{Gomez:1993ri}\\
\midrule
 FNAL E665 & $^{208}$Pb/$^2$D & 3 & \cite{Adams:1995is}\\
 NMC 96 & $^{208}$Pb/$^{12}$C & 14 & \cite{Arneodo:1996rv}\\
 \midrule
 \midrule
 {\bf Total NC DIS} & & {\bf 451} & \\
\bottomrule
\end{tabular}
\vspace{4mm}
\caption{\small The
neutral-current nuclear deep-inelastic
  input datasets included in \texttt{nNNPDF2.0}.
  %
  For each dataset, we indicate the nuclei $A_1$ and $A_2$
  involved, the number of data points that
  satisfy the baseline kinematical cuts,
  and the publication reference.
  %
}
\label{tab:nNNPDF20_data}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> _inputs/publications_wdates.tex <==
%\vspace{-360cm}
%\begin{NoHyper} \nobibliography* \end{NoHyper}
\newpage
\addcontentsline{toc}{chapter}{Publications}
\pagestyle{plain}
%
%\section*{Publications}
%\noindent {\LARGE \vspace{-1cm} \textbf{Publications}}
%\rhead{\textbf{My Publications}}
%\noindent      
\begin{table}[!h]
\centering
\begin{adjustwidth}{-1.3cm}{}
%\renewcommand*{\arraystretch}{1.3}
\vspace{-1.5cm}
\begin{tabular}{p{0.03\textwidth}|p{0.15\textwidth}p{0.85\textwidth}}
    \multicolumn{3}{c}{ {\Large \textbf{Publications}}}\\
    \cline{2-3}
    \parbox[c]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{{\Large \textbf{Ongoing}}\textcolor{white}{x}}}}& Sep, 2021 &R. Abdul Khalek,  T. Giani,  E. R. Nocera,  and  J. Rojo, \textbf{nNNPDF3.0: A global analysis of nuclear parton distributions at NNLO} \\
    & \multicolumn{2}{c}{ \vspace{-8pt} }\\
    &Sep, 2021 &R. Abdul Khalek, V. Bertone, D. Pitonyak, A. Prokudin, and N. Sato, \textbf{New ideas for impact studies at the EIC}\\
    \cline{2-3}
    \multicolumn{3}{c}{ \vspace{-8pt} }\\
    \cline{2-3}
    & & R. Abdul Khalek, V. Bertone, and E. R. Nocera, \textbf{A determination of unpolarised pion fragmentation functions using semi-inclusive deep-inelastic-scattering data: MAPFF1.0}, \textit{submission to Phys. Rev. D} \href{http://arxiv.org/abs/arXiv:2105.08725}{arXiv:2105.08725} \\
    &\multicolumn{2}{c}{ \vspace{-8pt} }\\
    & 29 Jan 2021 & R. Abdul Khalek, J. J. Ethier, E. R. Nocera, and J. Rojo, \textbf{Self-consistent determination of proton and nuclear PDFs at the Electron Ion Collider}, \textit{Phys. Rev. D} \textbf{103} (2021), no. 9 096005, [\href{http://arxiv.org/abs/arXiv:2102.00018}{arXiv:2102.00018}] \\
    &\multicolumn{2}{c}{ \vspace{-8pt} }\\
    & 25 Jun 2020 & R. Abdul Khalek, J. J. Ethier, J. Rojo, and G. van Weelden, \textbf{nNNPDF2.0: quark flavor separation in nuclei from LHC data}, \textit{JHEP} \textbf{09} (2020) 183, [\href{http://arxiv.org/abs/arXiv:2006.14629}{arXiv:2006.14629}]\\
    &\multicolumn{2}{c}{ \vspace{-8pt} }\\
    \parbox[c]{-2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{{\Large\textbf{Peer-reviewed}}}}} & 22 May 2020& R. Abdul Khalek et al., \textbf{Phenomenology of NNLO jet production at the LHC and its impact on parton distributions}, \textit{Eur. Phys. J. C} \textbf{80} (2020), no. 8 797, [\href{http://arxiv.org/abs/arXiv:2005.11327}{arXiv:2005.11327}]\\
    &\multicolumn{2}{c}{ \vspace{-8pt} }\\
    &25 Jun 2019 &\textbf{NNPDF} Collaboration, R. Abdul Khalek et al., \textbf{Parton Distributions with Theory Uncertainties: General Formalism and First Phenomenological Studies},\textit{Eur. Phys. J. C} \textbf{79} (2019), no. 11 931, [\href{http://arxiv.org/abs/arXiv:1906.10698}{arXiv:1906.10698}]\\
    &\multicolumn{2}{c}{ \vspace{-8pt} }\\
    &24 Jun 2019 &R. Abdul Khalek, S. Bailey, J. Gao, L. Harland-Lang, and J. Rojo, \textbf{Probing Proton Structure at the Large Hadron electron Collider}, \textit{SciPost Phys.} \textbf{7} (2019), no. 4 051, [\href{http://arxiv.org/abs/arXiv:1906.10127}{arXiv:1906.10127}]\\
    &\multicolumn{2}{c}{ \vspace{-8pt} }\\
    &10 May 2019 &\textbf{NNPDF} Collaboration, R. Abdul Khalek et al., \textbf{A first determination of parton distributions with theoretical uncertainties}, \textit{Eur. Phys. J.} \textbf{C} (2019) 79:838, [\href{http://arxiv.org/abs/arXiv:1905.04311}{arXiv:1905.04311}]\\
    &\multicolumn{2}{c}{ \vspace{-8pt} }\\
    &29 Mar 2019&\textbf{NNPDF} Collaboration, R. Abdul Khalek, J. J. Ethier, and J. Rojo, \textbf{Nuclear parton distributions from lepton-nucleus scattering and the impact of an electron-ion collider}, \textit{Eur. Phys. J. C} \textbf{79} (2019), no. 6 471, [\href{http://arxiv.org/abs/arXiv:1904.00018}{arXiv:1904.00018}]\\
    &\multicolumn{2}{c}{ \vspace{-8pt} }\\
    & 8 Oct 2018 &R. Abdul Khalek, S. Bailey, J. Gao, L. Harland-Lang, and J. Rojo, \textbf{Towards Ultimate Parton Distributions at the High-Luminosity LHC}, \textit{Eur. Phys. J. C} \textbf{78} (2018), no. 11962, [\href{http://arxiv.org/abs/arXiv:1810.03639}{arXiv:1810.03639}]\\
    \cline{2-3}
    \multicolumn{3}{c}{ \vspace{-8pt} }\\
    \cline{2-3}
    %\parbox[c]{-2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{{\Large\textbf{arXived}}}}} 
    &12 May 2020 & R. Abdul Khalek and V. Bertone, \textbf{On the derivatives of feed-forward neural networks}, \href{http://arxiv.org/abs/arXiv:2005.07039}{arXiv:2005.07039}\\
    \cline{2-3}
    \end{tabular}
\end{adjustwidth}
\end{table}

\begin{table}
    \centering
    \begin{adjustwidth}{-1.3cm}{}
    %\renewcommand*{\arraystretch}{1.3}
    \begin{tabular}{p{0.03\textwidth}|p{0.15\textwidth}p{0.85\textwidth}}
    \multicolumn{3}{c}{ {\Large \textbf{Publications}}}\\
    \cline{2-3}
    \parbox[c]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{{\Large\textbf{Proceedings and Reports}}\textcolor{white}{x}}}}&  8 Mar 2021 &R. Abdul Khalek et al., \textbf{Science Requirements and Detector Concepts for the Electron-Ion Collider: EIC Yellow Report}, \href{http://arxiv.org/abs/arXiv:2103.05419}{arXiv:2103.05419} \\
    & \multicolumn{2}{c}{ \vspace{-8pt} }\\
    & 11 Feb 2019 &P. Azzi et al., \textbf{Report from Working Group 1: Standard Model Physics at the HL-LHC and HE-LHC}, \textit{CERN Yellow Rep. Monogr.} \textbf{7} (2019) 1-220, [\href{http://arxiv.org/abs/arXiv:1902.04070}{arXiv:1902.04070}] \\
    & \multicolumn{2}{c}{ \vspace{-8pt} }\\
    & 31 Jan 2019 &M. Cepeda et al., \textbf{Report from Working Group 2: Higgs Physics at the HL-LHCand HE-LHC},\textit{CERN Yellow Rep. Monogr.} \textbf{7} (2019) 221-584, [\href{http://arxiv.org/abs/arXiv:1902.00134}{arXiv:1902.00134}] \\
    & \multicolumn{2}{c}{ \vspace{-8pt} }\\
    & 14 Nov 2018 &\textbf{NNPDF} Collaboration, R. Abdul Khalek, J. J. Ethier, and J. Rojo, \textbf{Nuclear Parton Distributions from Neural Networks}, \textit{Acta Phys. Polon. Supp.} \textbf{12} (2019), no. 4 927, [\href{http://arxiv.org/abs/arXiv:1811.05858}{arXiv:1811.05858}] \\
    \cline{2-3}
\end{tabular}
\end{adjustwidth}
\end{table}

\begin{comment}
\subsection*{Publications in preparation}
\begin{itemize} 
    \item \bibentry{AbdulKhalek:2021xxx1}
    \item \bibentry{AbdulKhalek:2021xxx2}
\end{itemize}
\subsection*{Main Publications}
\begin{enumerate} %https://tex.stackexchange.com/questions/49048/how-to-cite-one-bibentry-in-full-length-in-the-body-text
    \item \bibentry{Khalek:2021ulf}
    \item \bibentry{AbdulKhalek:2020yuc}
    \item \bibentry{AbdulKhalek:2020jut} 
    \item \bibentry{AbdulKhalek:2020uza} 
    \item \bibentry{AbdulKhalek:2019ihb} 
    \item \bibentry{AbdulKhalek:2019mps} 
    \item \bibentry{AbdulKhalek:2019bux} 
    \item \bibentry{AbdulKhalek:2019mzd} 
    \item \bibentry{Khalek:2018mdn}
\end{enumerate}

\newpage
\subsection*{Proceedings and Reports}
\begin{enumerate} 
    \item \bibentry{AbdulKhalek:2021gbh}
    \item \bibentry{Azzi:2019yne}
    \item \bibentry{Cepeda:2019klc}
    \item \bibentry{Khalek:2018bbv}
\end{enumerate}
\end{comment}

==> _inputs/temp.tex <==
\chapter{Projections and impact studies}
\label{chap:Impact}
\vspace{-1cm}
\begin{center}
  \begin{minipage}{1.\textwidth}
      \begin{center}
          \textit{This chapter is based on my results in Refs.~\mycite{AbdulKhalek:2019mps,Khalek:2018mdn,Azzi:2019yne,AbdulKhalek:2020yuc,Cepeda:2019klc,Khalek:2021ulf}}.
      \end{center}
  \end{minipage}
  \end{center}

In this chapter, I review the constraints on PDFs and nPDFs induced by pseudodata projected for several future-colliders as well as the impact of some of the data that is not included in the global analyses of \texttt{nNNPDF2.0}.
%IMPACT STUDIES
In Sect.~\ref{s1:PDF_Impact_studies}, I discuss two different future high energy programs at the LHC, the High Luminosity Large Hadron Collider in Sect.~\ref{s2:PDF_HLLHC} and the Large Hadron Electron Collider in Sect.~\ref{s2:PDF_LHeC}. pseudodata for these two colliders, covering different type of processes is generated according to multiple considerations and scenarios of the projected uncertainties. Based on these projections, I discuss the impact on the proton PDFs by means of Hessian profiling (see Sect.~\ref{s2:hessian_method}). The proton PDF sets used for these two analysis are the \texttt{PDF4LHC15} hessian sets.
%
In Sect.~\ref{s1:nNNPDF20_ImpactStudies}, I discuss the various phenomenological
applications of the \texttt{nNNPDF2.0} determination, starting with isolated photon
production in proton-lead collisions at the LHC, then, I revisit the potential of the FoCal upgrade to the ALICE
detector and finally I provide the predictions based on \texttt{nNNPDF2.0} for inclusive hadron
production in proton-nuclear collisions.
%
Finally, in Sect.~\ref{s1:EIC}, I present an update to the initial studies of the Electron-Ion Collider (EIC) neutral-current DIS pseudodata based on \texttt{\texttt{nNNPDF1.0}} and presented in Ref.~\mycite{AbdulKhalek:2019mzd}. In the updated analysis, we quantify the impact of unpolarized lepton-proton and
lepton-nucleus inclusive DIS cross section
measurements from the the official release of the EIC projections~\mycite{AbdulKhalek:2021gbh}. To this purpose we base our analysis~\mycite{Khalek:2021ulf} on a self-consistent set of proton (\texttt{NNPDF3.1}) and nuclear (\texttt{nNNPDF2.0}) global PDF determinations.

\section{Proton PDFs for future colliders} \label{s1:PDF_Impact_studies}

Measurements of production cross sections provide fundamental tests of theoretical predictions. Higher precision both of the experimental measurements and the theoretical predictions is required in order to determine fundamental parameters of the Standard Model and to discover beyond the Standard Model phenomena.
At the LHC, the precision of cross section measurements is limited by the uncertainty of the integrated luminosity, currently about 2\%. A target uncertainty of 1\% has been set for the High Luminosity phase, which is expected to be achieved by combination of improved luminosity detector instrumentation and refined analysis techniques~\mycite{Khalek:2018mdn, Azzi:2019yne, Cepeda:2019klc} starting its data acquisition in 2027.

In parallel, The Large Hadron electron Collider (LHeC) is also an LHC upgrade projected to operate when the LHC begins its high luminosity phase. This upgrade includes a newly built electron beam of 60 GeV up to possibly 140 GeV, energy colliding with the intense hadron beams of the LHC. The kinematic range covered is extended to that of HERA~\cite{Abramowicz:2015mha,Abramowicz:1900rp,Aaron:2009af,Abramowicz:2014zub}, the first $e$-$p$ collider,  by a factor of twenty in $Q^2$ and $x$ and projected to exceed the integrated HERA luminosity by two orders of magnitude. The physics programme is devoted to an exploration of the energy frontier, complementing the HL-LHC and possibly resolving the observation of new phenomena based on the specifics of deep inelastic $e$-$p$ scattering at energies extending to beyond a TeV~\mycite{AbdulKhalek:2019mps, AbelleiraFernandez:2012cc}.

%HLLHC
In Sect.~\ref{s2:PDF_HLLHC}, we focus on the the High-Luminosity (HL) phase of the LHC, manifested by a major upgrade of the accelerator and detector systems. More details can be found in Refs.~\mycite{Khalek:2018mdn, Azzi:2019yne, Cepeda:2019klc}.
%LHEC
In Sect.~\ref{s2:PDF_LHeC}, we extended the previous study of the HL--LHC impact to include, both individually and in combination, the impact from the Large Hadron electron Collider (LHeC), a high-energy lepton-proton and lepton-nucleus collider based at CERN. More details can be found in Ref.~\mycite{AbdulKhalek:2019mps, AbelleiraFernandez:2012cc}.

\subsection{High Luminosity Large Hadron Collider } \label{s2:PDF_HLLHC}
The High Luminosity phase (HL-LHC) is expected to deliver
a $14$ TeV center-of-mass energy with an integrated luminosity of around $\mathcal{L}=3$ ab$^{-1}$ to ATLAS and CMS and around $\mathcal{L}=0.3$ ab$^{-1}$ to LHCb.
This phase will improve the precision measurements of the Higgs boson properties, the heavy vector bosons masses and mixing angles, as well as extend the sensitivity to physics beyond the Standard model. More opportunities are summarised and detailed in
the CERN Yellow Report~\mycite{Azzi:2019yne, Cepeda:2019klc}.

These measurements are often limited by the uncertainties on PDFs. Therefore, to gauge their reduction, we considered a number of PDF-sensitive
processes presented in Table~\ref{tab:data_HLLHC}. For which, we have
generated HL--LHC pseudodata based on the projected center-of-mass energy and luminosity mentioned above.
%
Statistical uncertainties are evaluated
from the expected number of events per bin,
taking into account branching ratios and
acceptance corrections determined
from the corresponding reference analysis.
%
Systematic uncertainties are taken to be those of the
13~(8) TeV baseline analyses and then rescaled appropriately as shown in Eq.~(\ref{eq:totalExpError})
%
We consider various scenarios for the reduction of systematic errors,
from a more conservative one to a more optimistic one.

%Theoretical predictions are computed
%at next-to-leading order (NLO) in the QCD
%expansion using \text{MCFM}~\cite{Boughezal:2016wmq} interfaced to
%\texttt{APPLgrid}~\cite{Carli:2010rw} to produce
%the corresponding fast grids.
%
%The only exception is inclusive jet production, for which the NLO
%calculation is obtained from the \texttt{NLOJET++} program~\cite{Nagy:2003tz}.
%
Theoretical predictions are computed at NLO in the QCD and the central value of the pseudodata initially coincides with
the corresponding prediction obtained with the \texttt{PDF4LHC15}  NNLO set as input.
%
Subsequently, this central value is fluctuated
according to the prescription in Eq.~(\ref{eq:pseudodataGen}) by the corresponding experimental uncertainties.
%
%This implies that, by construction, one should find $\chi^2/N_\text{dat}\simeq 1$ from the fit to the pseudodata.

For the HL--LHC, we consider three sources of systematic uncertainties:
\begin{itemize}
  \item $\delta^\text{exp}_{\text{tot},i}$ is the total
(relative) experimental uncertainty corresponding to a specific bin $i$
(excluding the luminosity and normalization uncertainties).
\item $\delta^\text{exp}_{\mathcal L}$
is the luminosity uncertainty, which is fully
correlated among all the pseudodata bins of the same experiment
(but uncorrelated among different experiments).
%
We take this luminosity uncertainty to be $\delta^\text{exp}_{\mathcal L}=1.5\%$
for the three LHC experiments.
%
\item $\delta^\text{exp}_{\mathcal N}$
are possible additional normalization uncertainties as in the case of
$W$ boson production in association with charm quarks.
% that will be explained later \todo{is it?}.
\end{itemize}

If $\sigma_i^{\text{th}}$ is the theoretical cross-section
for  bin $i$ of a given process,
then the central value of
the HL--LHC pseudodata $\sigma_i^\text{exp}$ is constructed by means of
\begin{equation}
\label{eq:pseudodataGen}
\sigma_i^\text{exp} = \sigma_i^\text{th} \times \left( 1 + r_i\cdot \delta^\text{exp}_{\text{tot},i}
 + \lambda\cdot \delta^\text{exp}_{\mathcal L}+ s\cdot \delta^\text{exp}_{\mathcal N}\right)
\end{equation}
where $r_i$, $\lambda$, and $s$ are univariate Gaussian random numbers.
The total experimental uncertainty $\delta^\text{exp}_{\text{tot},i}$ is defined as
\begin{equation}
\label{eq:totalExpError}
\delta^\text{exp}_{\text{tot},i} \equiv \left( \left( \delta^\text{exp}_{\text{stat},i}\right) ^2 +
\left( f_\text{corr}\times f_\text{red}\times
\delta^\text{exp}_{\text{sys},i}\right)^2 \right)^{1/2}
\end{equation}
In this expression, the relative statistical error $\delta^\text{exp}_{\text{stat},i}$ is
computed as
\begin{equation}
\label{eq:acceptance}
\delta^\text{exp}_{\text{stat},i} = \left( f_\text{acc} \times N_{\text{ev},i}\right)^{-1/2} \, ,
  \end{equation}
  where $N_{\text{ev},i}=\sigma_i^\text{th} \times \mathcal{L}$ is the expected number
  of events in bin $i$ at the HL--LHC with $\mathcal{L}=3~(0.3)$ ab$^{-1}$ for ATLAS and CMS (LHCb).
  %
  In Eq.~(\ref{eq:acceptance}),
  $f_\text{acc}\le 1$
  is an acceptance correction which accounts for the fact that, for some of the processes
  considered, such as top quark pair production, there is a finite experimental acceptance
  for the final state products
  and/or one needs to include the effects of branching fractions.
  %
  The value of
  $f_\text{acc}$ is determined by extrapolation using the reference dataset,
  except for forward $W$+charm production (where there is no baseline measurement)
  where the acceptance is set to $f_\text{acc}=0.3$, due dominantly to the $c$--jet tagging efficiency.  
  
  In Eq.~(\ref{eq:totalExpError}),   $\delta^\text{exp}_{\text{sys},i}$ indicates the total
  systematic error of bin $i$ taken from the reference LHC measurement at either 8 TeV
  or 13 TeV; and $f_\text{red}\le 1$ is a correction factor that accounts for the fact that on average systematic
  uncertainties will decrease at the HL--LHC as compared to Run-2 due to both detector
  improvements and the enlarged dataset for calibration.
  %
  Finally, $f_\text{corr}$ represents
  an effective correction factor that accounts
  for the fact that data with correlated systematics may be more constraining than the same
  data where each source of error is simply added in quadrature,
  as we do in this analysis.
  %
  We show in Table~\ref{tab:data_HLLHC} the value of $f_\text{corr}$ determined by means of available LHC measurements
  for which the full information on correlated systematics
  is available.

%-------------------------------------------------------------------------------
\input{_tables/data_HLLHC.tex}
%-------------------------------------------------------------------------------


In Fig.~\ref{fig:kinHLLHC} we show  the kinematical coverage in
the $(x,Q^2)$ plane of the
  HL--LHC pseudodata included in this analysis.
  %
  %For each data point, the values of $(x_1,Q^2)$ and $(x_2,Q^2)$
  %corresponding to the two colliding partons are determined
  %approximately from leading-order kinematics, which is sufficient
  %for illustration purposes.
  %
  We assume $x_1=x_2$ if rapidities are not specified for the
  final states. 
  %
  We see that the HL--LHC pseudodata covers a wide kinematic region,
  including the large momentum transfers up to $Q^2\simeq 6^2$ TeV$^2$, as well
  as the large-$x$ region, with several different processes.
  %
  Specifically, the input pseudodata spans
  the range $6\times 10^{-5} \lsim x \lsim 0.7$ and
  $40^2~\text{GeV}^2 \lsim Q^2 \lsim 7^2~\text{TeV}^2$ in
  the $(x,Q^2)$ kinematic plane.
  %
  Note that the LHCb measurements are instrumental to constrain
  the small-$x$ region, $6\times 10^{-5} \lsim x \lsim 10^{-3}$, beyond
  the acceptance of ATLAS and CMS.
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
  \begin{center}
    \makebox[\textwidth]{\includegraphics[width=0.7\textwidth]{_plots/kinHLLHC.pdf}}
  \end{center}
  \vspace{-0.8cm}
\caption{
  The kinematical coverage in the $(x,Q^2)$ plane of the
  HL--LHC pseudodata included in this analysis.}
 \label{fig:kinHLLHC}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Drell-Yan production (both at high dilepton invariant mass and in the forward rapidity
%regions); $W$ production in association with charm quarks (central and forward regions);
%inclusive jet and prompt photon production; the transverse momentum of $Z$ bosons;
%and differential distributions in top quark pair production.
%%
%We have selected those processes that should benefit more directly
%from the increased statistics available at the HL--LHC;
%some available measurements, such as inclusive $W,Z$ production in the
%central region~\cite{Aaboud:2016btc,Khachatryan:2016pev}, are already
%completely limited by systematic uncertainties, with no significant improvement expected from increased statistics alone.
%%
%For each process, the binning and kinematic cuts applied to the pseudodata is constructed
%from a suitable generalisation of reference measurements
%at $\sqrt{s}=8$ and 13 TeV.
%%
%We consider different scenarios for the expected systematic uncertainties,
%from a conservative one with approximately the same systematics
%as the corresponding baseline measurements from Run I
%and a factor of 2 reduction for those from Run-2,
%to an optimistic one with
%a reduction by a factor 2.5 (5) as compared to Run I~(II). More details on the pseudodata can be found in Sect.~2 of Ref.~\cite{Khalek:2018mdn}

Subsequently, we quantify the constraints of the HL--LHC pseudodata on the symmetric Hessian\footnote{See Ref.~\cite{Buckley:2014ana} for the definition.} \texttt{PDF4LHC15}  PDF
set. The analysis is performed by means of the Hessian Profiling
method~\cite{Paukkunen:2014zia, Schmidt:2018hvu} (See
Sect.~\ref{s2:hessian_method}).

In our analysis, we use $T=3$ which roughly corresponds to the average tolerance
determined dynamically in the \texttt{CT14}  and \texttt{MMHT14}  analyses. We then combine the complete set
of HL--LHC pseudodata listed in Table~\ref{tab:data_HLLHC} to produce the final profiled
PDF sets, which quantify the impact of future HL--LHC measurements on our knowledge of the
quark and gluon structure of the proton. We have also performed a systematic study of the
constraints on the PDFs from the individual pseudodatas in Table~\ref{tab:data_HLLHC}
which can be found in Sect.~3 of Ref.\mycite{Khalek:2018mdn}.
%
As the list of processes for which pseudodata has been generated is by no means complete,
the results presented here should be understood as a conservative estimate (that is, an
upper bound) for the potential impact of HL--LHC measurements on PDFs.

In Table~\ref{tab:Scenarios} we list the three scenarios for the systematic uncertainties
of the HL--LHC pseudodata that we assume in the present analysis.
%
\input{_tables/HLLHC_scenarios.tex}
These scenarios, ranging from more conservative to more optimistic, differ among them in
the reduction factor $f_\text{red}$, Eq.~(\ref{eq:totalExpError}), applied to the
systematic errors of the reference 8 TeV or 13 TeV measurements.
%
In particular, in the optimistic scenario we assume a reduction of the systematic errors
by a factor 2.5 (5) as compared to the reference 8 TeV (13 TeV) measurements, while for
the conservative scenario we assume no reduction in systematic errors with respect to 8
TeV reference.
%
We also indicate in each case the name of the corresponding \texttt{LHAPDF} grid.
%
Reassuringly, as we show below, the qualitative results of our study depend only mildly in
the specific assumption for the values of $f_\text{red}$.

In Fig.~\ref{fig:HLLHC_PDFs_Q10} we present a comparison of the baseline \texttt{PDF4LHC15}  set with the
profiled sets based on HL--LHC pseudodata from scenarios A (conservative) and C
(optimistic) as defined in Table~\ref{tab:Scenarios}.
%
Specifically, we show the down quark, up anti-quark, total strangeness and gluon at $Q=10$ GeV, normalized
to the central value of the \texttt{PDF4LHC15}  baseline.
%
In this comparison, the bands correspond to the one-sigma PDF uncertainties.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
  \begin{center}
    \makebox[\textwidth]{\includegraphics[width=\textwidth]{_plots/HLLHC_RatioPDFs_Q10.pdf}}
    \end{center}
    \vspace{-0.8cm}
    \caption{Comparison of the \texttt{PDF4LHC15}  at NNLO set with the HL-LHC profiled set in the conservative and optimistic scenarios, defined in Table~\ref{tab:Scenarios}. We show the down quark, up anti-quark, total strangeness and gluon at $Q$=10 GeV, normalized to the central value of the \texttt{PDF4LHC15}  baseline. The bands correspond to the one-sigma PDF uncertaintes. On the right, same as left but relative uncertainties are shown.}
  \label{fig:HLLHC_PDFs_Q10}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % https://arxiv.org/pdf/2001.04370.pdf

First of all, we observe that the impact of the HL--LHC pseudodata is reasonably similar
in the conservative and optimistic scenarios. Therefore we don't show the intermediate
one.
%
This is not so surprising, as we have explicitly chosen those datasets which will benefit
from a significant improvement in statistics, and these tend to lie in kinematic regions
where the PDFs themselves are generally less well determined.
%
Therefore, the dominant reason for the observed reduction of PDF uncertainties is the
increased statistics and the corresponding extended kinematic reach that becomes
available at the HL--LHC, rather than the specific assumptions about the systematic
uncertainties. This demonstrates that our results are robust against the details of the
projections of how the experimental systematic uncertainties will be reduced in the
HL--LHC era.

From Fig.~\ref{fig:HLLHC_PDFs_Q10} we observe a marked reduction of the PDF uncertainties in
all cases.
%
This reduction is specially significant for the gluon and the sea quarks, for the reason
that these are currently affected by larger uncertainties than in the case of the
valence quarks.
%
In the case of the gluon PDF, there is an improvement of uncertainties in the complete
relevant range of momentum fraction $x$.
%
This is a direct consequence of the fact that we have included here several HL--LHC
processes that have direct sensitivity to the gluon content of the proton, including
jet, direct photon, and top quark pair production, as well as the transverse momentum of
$Z$ bosons.

Another striking feature of Fig.~\ref{fig:HLLHC_PDFs_Q10} concerns the strange PDF.
%
In this case, the PDF uncertainties are reduced by almost a factor 4, from around 15\%
to a few percent, in a wide region of $x$.
%
This result highlights the importance of the $W$+charm measurements at the HL--LHC,
specially those in the forward region by LHCb, which
represent a unique handle on the poorly known strange content of the proton.
%
In turn, such improved understanding of the strange PDF will feed into a reduction of
theory uncertainties in crucial HL--LHC measurements such as those of $M_W$ or
$\sin^2\theta_W$.

We conclude that, even in the most conservative scenario, we find that
HL--LHC measurements can reduce PDF uncertainties by at least a factor between 2 and 3 as
compared to the current \texttt{PDF4LHC15}  baseline.
%
The PDF constraining information from the HL--LHC is expected to be specially significant
for gluon- and for strange-initiated processes.
%
This improved knowledge of the quark and gluon structure of the proton which will become
possible at the HL--LHC will directly benefit a number of phenomenologically important
processes which we present in Ref.~\cite{}, thanks to the reduction of the associated theoretical errors.
%
For instance, the PDF uncertainties in Higgs production in gluon fusion can be reduced
down to $\lsim 2\%$ for the entire range of Higgs transverse momenta accessible at the
HL--LHC.
%
Likewise, PDF uncertainties in high-mass supersymmetric particle production can be
decreased by up to a factor 3 as compared with the current situation.
%
This improvement should strengthen the bounds derived in the case of null searches, or
even facilitate their characterisation in the case of an eventual discovery.
%
Similar improvements are found for Standard Model process, for example dijet production,
which provides a unique opportunity to measurement the running of the strong coupling
constant at the TeV scale.
%
The results of this study are made publicly available in the \texttt{LHAPDF6}
format~\cite{Buckley:2014ana}, with the grid names listed in Table~\ref{tab:Scenarios}
for the three scenarios that have been considered.
%
%These three grid files can be downloaded from:
% \begin{center}
%\texttt{https://data.nnpdf.science/HLLHC\_YR/\texttt{PDF4LHC15} \_nnlo\_hllhc\_scen1.tgz}\\
%\texttt{https://data.nnpdf.science/HLLHC\_YR/\texttt{PDF4LHC15} \_nnlo\_hllhc\_scen2.tgz}\\
%\texttt{https://data.nnpdf.science/HLLHC\_YR/\texttt{PDF4LHC15} \_nnlo\_hllhc\_scen3.tgz}
% \end{center}

\subsection{Large Hadron Electron Collider } \label{s2:PDF_LHeC}
%---
In the previous section we discussed the HL-LHC potential to constrain the PDFs~\mycite{Khalek:2018mdn}
by using projected measurements for a range of SM processes,
from Drell-Yan to top quark pair and jet production.
%
We found that PDF uncertainties on LHC processes can be reduced by a factor between two and five,
depending on the specific flavour combination and on the assumptions about the experimental systematic uncertainties.
%
Our PDF projections have already been used in a number of related HL--LHC studies,
as reported in~\mycite{Azzi:2019yne,Cepeda:2019klc}.

A quite distinct possibility to improve our understanding of proton structure
is the proposal to collide high energy electron and positron beams with the hadron beams from the HL--LHC.
%
This facility, known as the Large Hadron Electron Collider (LHeC)~\cite{AbelleiraFernandez:2012cc,AbelleiraFernandez:2012ty,Klein:2018rhq}, would run concurrently with the HL--LHC and be based on a new purpose--built detector at the designed interaction point.
%
A key outcome of the LHeC operations would be a significantly larger and higher--energy dataset of lepton--proton collisions in comparison to the existing HERA structure function measurements~\cite{Abramowicz:2015mha}.
%
Indeed, the latter to this day form the backbone of all PDF determinations~\cite{Harland-Lang:2014zoa,Dulat:2015mca,Abramowicz:2015mha,Alekhin:2017kpj,Ball:2017nwa}, and thus the LHeC would
provide the opportunity to greatly extend the precision and reach of HERA data in both $x$ and $Q^2$,
highlighting its potential for PDF constraints.
%
Moreover, these measurements
would be taken in the relatively clean environment of lepton--proton collisions, where the corresponding
theoretical predictions are known to a very high level of precision.
%
It should also be emphasized here that the LHeC would reach studies beyond the proton structure, such as the characterization
of the Higgs sector or the study of cold nuclear matter in the small-$x$ region, where new QCD dynamical
regimes such as saturation are expected to appear.

Quantitative PDF projection studies based on LHeC pseudodata have been presented
previously~\cite{AbelleiraFernandez:2012cc,AbelleiraFernandez:2012ty,Paukkunen:2017phq,Cooper-Sarkar:2016udp},
where a sizeable reduction in the resultant PDF uncertainties is reported.
%
These LHeC PDF projections are based upon the HERAPDF-like input PDF parametrization and flavour assumptions~\cite{Abramowicz:2015mha},
with some additional freedom in the input parametrisation
added in the most recent studies~\cite{LHeCtalk1,LHeCtalk2}.
%
However, different
results may be obtained if a more flexible parametrization or alternative flavour assumptions are used,
as shown for example in the study of~\cite{Ball:2017otu} carried out in the \texttt{NNPDF} framework.
%
In addition, the interplay of these constraints from the LHeC with the expected sensitivity from the HL--LHC~\mycite{Khalek:2018mdn} has not yet been studied.
%
Thus in this section we discuss how the projected sensitivity of a state-of-the-art
global PDF determination
will improve with data from the LHeC, and how this will complement the information
contained in the measurements in $pp$ collisions provided by the HL--LHC.
%

We follow the strategy presented in the previous section (Ref.~\mycite{Khalek:2018mdn} for more details), starting from the
\texttt{PDF4LHC15} ~\cite{Gao:2013bia,Carrazza:2015aoa,Butterworth:2015oua} baseline set, and quantify the expected impact of the LHeC measurements both individually and combined
with the information provided by the HL--LHC. For the LHeC pseudodata we use the most recent publicly available official
LHeC projections on the expected statistical and systematic errors, and choice of binning~\cite{mklein} (see also~\cite{Klein:1564929} for
further details)
%
As we will demonstrate, the expected constraints from the LHeC are significant and fully complementary
with those from the HL--LHC.
%
When included simultaneously, a significant reduction in PDF uncertainties in the entire relevant
kinematical range for the momentum fraction $x$ is achieved, with beneficial implications for LHC phenomenology. Additional methodological investigation has been performed in Ref.~\mycite{AbdulKhalek:2019mps, AbelleiraFernandez:2012cc} where we assess the impact of adopting a more restrictive input parameterisation as our baseline PDF set.
%
%The slightly subtle issue here is that when one generates pseudodata assuming an underlying PDF parameterisation one is implicitly assuming that it will be possible to describe the actual data with this parameterisation. If this assumption is too strong, that is the underlying parameterisation is too restrictive, then one is liable to overestimate the impact of the data. Consistent with this, we find a more marked reduction of the
%PDF uncertainties for the rather restrictive HERAPDF baseline in comparison to the global PDF4LHC case. To clarify this further, we present pure `LHeC--only' fits, that is modifying the Hessian prior to effectively remove the impact of the data in the baselines, and isolate the impact of the parameterisation alone. These are therefore directly comparable to other LHeC--only projections; we in particular take a tolerance of $T=1$ here. We again find significantly smaller projected errors when assuming the HERAPDF parameterisation in comparison to the more flexible PDF4LHC one.
%----

For the LHeC pseudodata, we use the most recent publicly available official
LHeC projections~\cite{mklein} (see also~\cite{Klein:1564929} for
further details) for electron
and positron neutral-current (NC) and charged-current (CC) scattering.
%
The main features of the pseudodata sets we consider are summarised in Table~\ref{tab:pseudodataLHeC}, along with the corresponding integrated luminosities and kinematic reach. 
%
While the nominal high energy data ($E_p=7$ TeV) provides the dominant PDF constraints, the
lower energy ($E_p=1$ TeV) data extends the acceptance to higher $x$ and provides a handle on the longitudinal structure function, $F_L$, and hence the gluon PDF (we note that further variations in the electron and/or proton energy will provide additional constraints on this, as well as on other novel low--$x$ QCD phenomena). 
The charm and bottom heavy quark NC structure function pseudodata provide additional constraints on the gluon.
%
In addition, charm production in $e^- p$ CC scattering provides important information on the anti-strange quark distributions
via the $\overline{s}+ W \to \overline{c}$ process. We do not include charm production in $e^+ p$ CC scattering, as the corresponding projections are not currently publicly available, though this would provide an additional constraint on the strange quark PDF.
%
We apply a kinematic cut of $Q \ge 2$ GeV to ensure that the fitted
data lie in the range where perturbative QCD calculations can be reliably
applied.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{_tables/data_LHeC.tex }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The kinematic reach in  the $(x,Q^2)$ plane of the LHeC pseudodata is shown in Fig.~\ref{fig:kinLHeC}.
%
The reach in the perturbative region ($Q\ge 2$ GeV)
is well below $x \approx 10^{-5}$ and extends up to $Q^2 \approx 10^6$ $\text{GeV}^2$
(that is, $Q\simeq 1$ TeV), increasing the HERA coverage
by over an order of magnitude in both cases, via the factor $\sim$ 4
increase in
the collider centre-of-mass energy $\sqrt{s}$.
%
Due to the heavy quark tagging requirements, the reach for semi-inclusive structure functions
only extends up to $x\simeq 0.3$ in the large-$x$ region.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
  \begin{center}
    \makebox[\textwidth]{\includegraphics[width=0.7\textwidth]{_plots/kinplot_fcc.pdf}}
  \end{center}
  \vspace{-0.8cm}
\caption{
  The kinematic coverage in the $(x,Q^2)$ plane of the LHeC pseudodata~\cite{mklein} included in this analysis.}
  %the inclusive NC and CC structure functions both for high energy (HE) and low energy (LE) datasets, the NC charm and bottom semi-inclusive structure functions $F_2^{c\bar{c}}$ and $F_2^{b\bar{b}}$, and the CC charm structure functions $F_2^c$ providing direct information on the strange content of the proton.}
 \label{fig:kinLHeC}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this analysis, we use $T=3$ same as in the HL--LHC study, except that in this case we don't need for uncertainty-tuners ($f_\text{corr}$,$f_\text{red}$ and $f_\text{acc}$) as we're using the official LHeC projections. 
%
The resulting profiled PDF set is shown in Fig.~\ref{fig:LHeCandHLLHC_PDFs_Q10}.
%
We find that
the LHeC and HL--LHC datasets both place significant constraints on the PDFs, with some differences
depending on the kinematic region or the specific flavour combination being considered.
%
Most importantly, we deduce that these are rather complementary: while the LHeC places the most significant constraint at low to intermediate $x$ in general (though in the latter case the HL--LHC impact is often comparable in size), at high $x$ the HL--LHC places the dominant constraint on the gluon and strangeness, while the LHeC dominates for the up and down quarks.
%
Moreover, when both the LHeC and HL--LHC pseudodata are simultaneously included
in the fit, all PDF flavours can be constrained across a wide range of $x$, providing a strong motivation
to exploit the  input for PDF fits from both experiments, and therefore for realising the LHeC itself.

Finally, a few important caveats concerning this exercise should be mentioned.
%
First, the processes included for both the LHeC and HL--LHC, while broad in scope, are by no means exhaustive.
%
Most importantly, no jet production were included for the LHeC, which
would certainly improve the constraint on the high-$x$ gluon. In addition, the inclusion of charm production in $e^+ p$ CC scattering would further constrain the strange quark.
%
In the case of the HL--LHC, only those processes which provide an impact at high-$x$ were included, and hence the lack of constraint at low-$x$ that is observed occurs essentially by construction.
%
In particular, there are a number of processes that will become available
with the legacy HL--LHC dataset, or indeed those in the current LHC dataset that are not currently included in global fits, but which can in principle constrain the low-$x$ PDFs, from low mass Drell--Yan to inclusive $D$ meson production~\cite{Zenaiev:2015rfa,Gauld:2016kpd} and exclusive vector meson photoproduction~\cite{Jones:2016ldq}, though here the theory is not available at the same level of precision to the LHeC case.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
  \begin{center}
    \makebox[\textwidth]{\includegraphics[width=\textwidth]{_plots/LHeCandHLLHC_RatioPDFs_Q10.pdf}}
    \end{center}
    \vspace{-0.8cm}
    \caption{On the left, Comparison of the \texttt{PDF4LHC15}  at NNLO set with the LHeC profiled set, the HL-LHC profiled set in optimistic scenario (see Table~\ref{tab:Scenarios}) and their combinations. We show the down quark, up anti-quark, total strangeness and gluon at $Q$=10 GeV, normalized to the central value of the \texttt{PDF4LHC15}  baseline. The bands correspond to the one-sigma PDF uncertaintes. On the right, same as left but relative uncertainties are shown.}
  \label{fig:LHeCandHLLHC_PDFs_Q10}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%A further point of note is the value of the tolerance $T$ used in this %analysis.
%%
%By performing a closure test using \texttt{PDF4LHC15}  as input, we are implicitly %assuming that the final LHeC (and HL--LHC) data will be describable by this %set, within the $T=3$ tolerance criteria to allow for some degree of %tension among datasets.
%%
%That is, one is implicitly assuming that no greater tension between %datasets than this will occur.
%%
%While this assumption is guided by previous experience with the wide range %of measurements included in existing global PDF fits, it may turn out to be %too strong and if this is the case we would expect the resulting PDF %uncertainties to be larger, though at this point there is no strong %motivation for believing that this will indeed be the case.
%On the other hand, as shown in Fig.~\ref{fig:pdf_tolerance}, a more %aggressive, smaller, choice for the LHeC leads to smaller uncertainties in %that case, though the interpretation of such a choice in the context of %this global fit to both HL--LHC and LHeC pseudodata is far from clear,
%being inconsistent with the assumptions used to construct the \texttt{PDF4LHC15}  %baseline to begin with.


%\subsection{Photon and hadron production in pA at the LHC}
%\label{s2:nNNPDf20_pheno}

\section{Nuclear PDFs for the Large Hadron Collider} 
\label{s1:nNNPDF20_ImpactStudies}
In this section, I discuss various phenomenological
applications of the \texttt{nNNPDF2.0} determination.
%
%
I start by focusing on theoretical predictions for isolated photon
production in proton-lead collisions at the LHC, compared with recent 
measurements from the ATLAS collaboration taken at $\sqrt{s}=8.16$ TeV.
%
%
Then, I revisit the potential of the FoCal upgrade to the ALICE
detector in constraining the small-$x$ gluon nuclear PDF using
measurements of direct photon production in the forward region.
%
%
Afterwards, I provide the predictions based on \texttt{nNNPDF2.0} for inclusive hadron
production in proton-nuclear collisions, a process that can constrain both the
quark and gluon nuclear PDFs as well as the corresponding fragmentation
functions in vacuum and in medium.


\myparagraph{Isolated photon production in pA collisions with ATLAS}
%\label{s2:nNNPDF20_photonproduction_ATLAS}
%
Production of isolated photons in proton-proton collisions is
primarily sensitive to the gluon content of the proton via the QCD Compton
scattering process~\cite{Vogelsang:1995bg,Ichou:2010wc}.
%
However, several complications associated with
the measurement of photon production 
complicate a clean interpretation in terms of 
hard-scattering cross-sections, such as 
the need for subtracting the fragmentation 
component and the removal of photons coming
from pion decays.
%
Although early PDF fits used photon production 
in fixed-target scattering to constrain the
gluon data, the data were eventually discarded in favour of
the cleaner and more abundant data on jet production at the
TeVatron~\cite{Gao:2017yyd}.
%
However, photon production measurements from ATLAS and CMS were
later revisited using NLO QCD theory in Ref.~\cite{d'Enterria:2012yj}
and again at NNLO in Ref.~\cite{Campbell:2018wfu}.
%
These studies demonstrated the consistency of collider-based 
isolated photon production measurements 
with QCD predictions and with the rest of
the datasets in the global analysis.
%
Moreover, they help to reduce the uncertainties on the gluon PDF
at $x\simeq 10^{-2}$, a region that is particularly 
relevant for theoretical predictions of Higgs production in gluon fusion.

Photon production is also a highly relevant process in the context of
heavy ion collisions.
%
Being a QCD-neutral probe, it traverses the quark-gluon plasma without
modifications and thus represents a robust baseline to study the hot and
dense medium properties~\cite{Vitev:2008vk}.
%
In order to disentangle hot from cold nuclear matter effects, photon
production has been measured in proton-lead collisions at the LHC,
providing a new channel to constrain the nuclear modifications of the
gluon PDF.
%
Here we focus on the recent ATLAS measurements
from Run II at $\sqrt{s}=8.16$ TeV based on an integrated luminosity of
$\mathcal{L}=165$ nb$^{-1}$~\cite{Aaboud:2019tab}.
%
This analysis provides the inclusive production rates of isolated prompt
photons in three different rapidity regions as a function of
$E_{T}^{\gamma}$, the photon transverse energy, in the range 20
GeV to 550 GeV.

To compute the corresponding theoretical predictions, 
we use NLO QCD theory with the same settings as
in Ref.~\cite{Campbell:2018wfu} by adopting a modified 
version of {\tt MCFM} v6.8 interfaced to {\tt APPLgrid}.
%
The settings of the calculation have been adjusted to map the
experimental isolation conditions and thus bypass the need to explicitly
account for the fragmentation component.
%
We have benchmarked the results of this {\tt MCFM}-based calculation
with the theory predictions presented in Ref.~\cite{Aaboud:2019tab} based on
the {\tt JETPHOX} program~\cite{Catani:2002ny}, finding a reasonable
agreement but also some differences at large rapidities.

In Fig.~\ref{fig:ATLASthdat}, we display the comparison between the ATLAS
measurements of the photon transverse energy ($E_T^\gamma$)
distributions in three rapidity bins with the corresponding NLO QCD
theory calculations based on {\tt MCFM} with \texttt{nNNPDF2.0} and \texttt{EPPS16} as
input.
%
For each rapidity bin, the upper panels display the absolute
distributions and the lower panels the corresponding ratio between the
central value of the experimental data and the theory calculations.
%
The error bands in the experimental measurements indicate the sum in
quadrature of the statistical and systematic experimental uncertainties, while in
the theory calculations the error bands correspond to the 90\% CL ranges.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.90\textwidth]{_inputs/nNNPDF20/plots/nATLAS_PHT.pdf}
 \end{center}
\vspace{-0.8cm}
\caption{Comparison between the ATLAS measurements of the photon
  $E_T^\gamma$ distributions in three rapidity bins in the center of
  mass frame with the corresponding  NLO QCD theory calculations based
  on {\tt MCFM} with \texttt{nNNPDF2.0} and \texttt{EPPS16} as input.
  %
  For each rapidity bin, the upper panels display the absolute
  distributions and the lower panels the corresponding ratio between the
  theory calculations and the central value of the experimental data.
  \label{fig:ATLASthdat}
}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

From this comparison one finds that the theory calculations appears to
undershoot the experimental data by roughly $25\%$ 
in the three rapidity bins for most of
the $E_T^\gamma$ range, both for \texttt{nNNPDF2.0} and \texttt{EPPS16}.
%
This discrepancy cannot be accommodated within the stated experimental
and theoretical uncertainties.
%
A similar qualitative behaviour was reported in the
original ATLAS publication based on the {\tt JETPHOX} predictions.
%
On the other hand, the NNPDF3.1 proton PDFs are known to describe well the
corresponding isolated photon measurements from proton collisions 
at both $\sqrt{s}=8$ and 13 TeV~\cite{Campbell:2018wfu}.

As expected, the disagreement between the experimental data and the
theory calculations found in Fig.~\ref{fig:ATLASthdat} is
translated into poor $\chi^2$ values.
%
Using \texttt{nNNPDF2.0}, one obtains that $\chi^2/N_{\rm dat}=9.1, 10.5,$ and
$8.5$ in the forward, central, and backwards rapidity bin.
%
Similar numbers are obtained in the case of the theory predictions based
on \texttt{EPPS16}.
%
The situation does not improve by much if the ATLAS photon data is added
to the \texttt{nNNPDF2.0} global analysis.
%
In such a case the agreement between the theory calculations and the
experimental data improves somewhat, with $\chi^2/N_{\rm dat}=6.1, 7.5,$
and $5.7$ for the three rapidity bins, but it remains far from
satisfactory.

Until the origin of this disagreement between theory and data is better
understood, it will not be possible to include the ATLAS prompt photon
production measurements in a global nPDF fit.
%
Alternatively, one could instead consider fitting related observables
that are presented in the same ATLAS publication.
%
The first of these is the nuclear modifications ratio $R_{p{\rm Pb}}$,
where the absolute $E_{T}^\gamma$ distributions in pPb collisions are
normalized to their pp counterparts, the latter being derived from a
simulation-derived extrapolation from data in proton-proton collisions
at $\sqrt{s}=8$ TeV.
%
The second is the ratio between different rapidity bins, such as between
forward and backward rapidities, as a function of $E_T^\gamma$.
%
The advantages of such ratios is that many experimental systematic
uncertainties partially cancel out, thus facilitating the comparison
with theoretical predictions.
%
On the other hand, these observables might also exhibit a reduced nPDF
sensitivity, in particular for the ratio between different rapidity
bins.
%
Future studies should shed more light on the usefulness of the prompt
photon measurements to constrain nuclear PDFs within a global analysis.

\myparagraph{Isolated photon production in pA collisions with FoCal}
%\label{s2:nNNPDF20_photonproduction_FoCal}
%
Current measurements of direct photon production at the LHC, such as
those discussed above from the ATLAS collaboration~\cite{Aaboud:2019tab}
as well as related measurements from CMS and
ALICE~\cite{Acharya:2020sxs}, are restricted to the central rapidity
region.
%
The reason is that this is the only region instrumented with
electromagnetic calorimeters and thus suitable to identify photons.
%
A measurement of isolated photon production in the forward region,
however, is also highly interesting for nPDF studies.
%
Not only would such measurements provide direct access to the
poorly-known gluon nuclear modifications at small-$x$, but 
it would also allow testing for the possible onset of QCD non-linear
dynamics~\cite{Benic:2016uku}.

With this motivation, a new forward calorimeter extension of the ALICE
detector, dubbed
FoCal~\cite{vanderKolk:2020fqo,ALICECollaboration:2719928}, has been
proposed.
%
Both the acceptance and instrumentation of this detector have been optimized
to provide access to the nuclear PDFs at low scales and small momentum
fractions via the measurement of isolated photon production at low
transverse momenta and forward rapidities in proton-ion collisions.
%
The FoCal is proposed for installation during the Long Shutdown 3
(2025-2026) phase of the LHC.

The impact of future FoCal measurements on the small-$x$ nuclear PDFs
was first studied in Ref.~\cite{vanLeeuwen:2019zpz}.
%
In that analysis, pseudodata based on the expected kinematical reach
and experimental uncertainties for FoCal was generated and used to
constrain the \texttt{nNNPDF1.0} determination by means of the Bayesian
reweighting method~\cite{Ball:2010gb,Ball:2011gg}.
%
It was found that the FoCal measurement would constrain the nuclear
gluon modifications down to $x\simeq 10^{-5}$, leading to an uncertainty
reduction by up to an order of magnitude as compared to the baseline
fit.
%
These results indicated a comparable or superior constraining power on
the small-$x$ nPDFs when compared to related projections from future
facilities, such as the Electron Ion Collider~\cite{Accardi:2012qut}.

Motivated by the new and improved projections for the FoCal 
pseudodata that have recently became available, 
we revisit their impact on nuclear PDFs
using the present nPDF determination. 
%
In this case, the \texttt{nNNPDF2.0} PDFs represent a more realistic 
baseline since they provide a robust quark flavour
separation with a better handle on the gluon.
%
Moreover, the positivity of physical cross-sections is guaranteed, 
a constraint that helps to reduce the small-$x$ nuclear PDF uncertainties.

For this study we have adopted the same settings as
in Ref.~\cite{vanLeeuwen:2019zpz} and computed NLO QCD predictions with a
modified version of {\tt INCNLO} that benefits from improved numerical
stability at forward rapidities~\cite{Helenius:2014qla}.
%
Theoretical predictions for FoCal cross-sections have been computed with
$N_{\rm rep}=400$ replicas of \texttt{nNNPDF2.0}, which are subsequently used to
account for the impact of the FoCal pseudodata by means of Bayesian
reweighting.\footnote{We are grateful to Marco van Leeuwen for providing
us with the results presented here.}
%
Fig.~\ref{fig:focal} displays the nuclear modification factor $R_{\rm
  pPb}(p_T^\gamma)$ for direct photon production in pPb collisions at
  $\sqrt{s}=8.8$ TeV for a rapidity of $\eta_\gamma=4.5$ as a function
  of the photon's transverse momentum $p_T^\gamma$.
  %
  The theoretical predictions based on NLO QCD theory are compared with
  the FoCal pseudodata for two sets of input nPDFs: the original
  \texttt{nNNPDF2.0} set, and the variant that has been reweighted with the FoCal
  projections.
  %
  Here the central value of the FoCal pseudodata has been
  chosen to be the same as that of the \texttt{nNNPDF2.0} prediction.
  %
  In the right panel of Fig.~\ref{fig:focal} we show the gluon nuclear
  modification factor $R_g(x,Q)$ for $Q^2=10$ GeV$^2$ for both the
  original and the reweighted \texttt{nNNPDF2.0} fits.
  %
  In all cases, the nPDF uncertainty bands correspond to the 90\%
  confidence level intervals.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.49\textwidth]{_inputs/nNNPDF20/plots/RpPb_gamma_eta45_reweight_nNNPDF20.pdf}
\includegraphics[width=0.49\textwidth]{_inputs/nNNPDF20/plots/Rg_nNNPDF20_FoCal_reweight_nNNPDF20_centralvalue.pdf}
  \end{center}
  \vspace{-0.8cm}
\caption{Left: the nuclear modification factor $R_{\rm pPb}(p_T^\gamma)$
  for direct photon production in pPb collisions at $\sqrt{s}=8.8$ TeV
  for a rapidity of $\eta_\gamma=4.5$ as a function of the photon
  transverse momentum $p_T^\gamma$.
  %
  The theoretical predictions are compared with the FoCal pseudodata
  for two sets of input nPDFs: the original \texttt{nNNPDF2.0} set, and the
  variant that has been reweighted with with FoCal projections.
  %
  Here the FoCal pseudodata assumes the central value of the \texttt{nNNPDF2.0}
  prediction.
  %
  Right: the gluon nuclear modification factor $R_g(x,Q)$ for $Q^2=10$
  GeV$^2$ for both the original and the reweighted \texttt{nNNPDF2.0} fits.
  %
  The nPDF uncertainties correspond in both cases to the 90\% confidence
  level intervals.
  \label{fig:focal}
}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

From the results of Fig.~\ref{fig:focal}, one finds that the FoCal
measurements would still impact the uncertainties of the nuclear gluon
modifications at small-$x$, especially in the upper limit of the
uncertainty band.
%
The effective number of replicas in this case is $N_{\rm
eff}=345$.
%
Note that \texttt{nNNPDF2.0} exhibits a preference for $R_{\rm pPb}\simeq 1$,
and thus shadowing is not favoured in the gluon sector, consistent
with the results reported in Fig.~\ref{R_A}.
%
On the other hand, \texttt{nNNPDF2.0} does not contain any dataset with
particular sensitivity to the nuclear gluon modifications, implying that
the projections for the impact of FoCal in the global nPDF analysis
could be somewhat over-optimistic.% (see also the discussion in Sect.~\ref{sec:summary}).

Crucially, however, we have assumed in this exercise that the central value of the
FoCal measurement would be unchanged compared to the initial baseline
prediction.
%
In Fig.~\ref{fig:focal2} we display instead the results of the
reweighting for a scenario in which the FoCal pseudodata 
have a value of $R_{\rm pPb} \simeq 0.6$.
  %
  In this case, the effective number of replicas is much smaller, $N_{\rm
  eff}=117$, indicating that the FoCal data are adding a significant
  amount of new information to the global fit.
  %
  Here the resulting value for the gluon nuclear modification
  ratio at small-$x$ would be $R_g\simeq 0.7$.\footnote{
  Note that the reweighting technique may lead to unreliable 
  uncertainty bands when using data values that fall 
  outside the predictions produced by the prior.}
  %
  Therefore, this analysis indicates that FoCal measurements could be
  sensitive either to the gluon shadowing effects or to possible
  non-linear QCD dynamics.
  %
  To disentangle one from the other, a dedicated analysis of the
  $\chi^2$ and nPDF behaviour in the small-$x$ region would
  be required, following the approach developed in Ref.~\cite{Ball:2017otu}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
  \begin{center}
    \includegraphics[width=0.49\textwidth]{_inputs/nNNPDF20/plots/RpPb_gamma_eta45_reweight_nNNPDF20_lowvals.pdf}
    \includegraphics[width=0.49\textwidth]{_inputs/nNNPDF20/plots/Rg_nNNPDF20_FoCal_reweight_nNNPDF20_lowvals.pdf}
    \end{center}
    \vspace{-0.8cm}
\caption{Same as Fig.~\ref{fig:focal} now for the case where the FoCal
  pseudodata has been generated under the assumption that $R_{\rm pPb}
  \simeq 0.6$ rather than based on the \texttt{nNNPDF2.0} central value.
  \label{fig:focal2}
}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\myparagraph{Inclusive hadron production in pA collisions}
%\label{s2:nNNPDF20_Inclusive_hadron_production}
%
The inclusive production of pions and kaons in hadronic collisions
provides information not only on the initial state (parton
distribution functions) but also on the final-state hadronisation
mechanism of partons into hadrons.
%
The latter is described by the fragmentation functions (FFs), which are
extracted from experimental data by means of a global analysis akin to
that of the PDFs~\cite{deFlorian:2014xna,Sato:2019yez,d'Enterria:2013vba,Bertone:2018ecm,Bertone:2017tyb,Albino:2005me,Hirai:2007cx}.
%
Likewise, in proton-nuclear collisions the production of identified
hadrons can provide information on the initial state nuclear PDFs
as well the parton-to-hadron hadronisation in the
presence of cold nuclear matter effects.

In Fig.~\ref{fig:plot_R_all}, we display the nuclear modification ratio
  $R_{\rm Pb}^{\pi^0}$ for the production of neutral pions in
  proton-lead collisions as a function of the pion transverse momentum
  $p_T$.
  %
  The theoretical calculations
  are based on NLO QCD and use the DSS14
  hadron fragmentation functions~\cite{deFlorian:2014xna}
  for both the \texttt{nNNPDF2.0} and \texttt{EPPS16} predictions.\footnote{We are grateful to Ilkka Helenius for providing us with the results of this calculation.}
  %
  Moreover, the central values and 90\% CL uncertainties 
  are provided for RHIC kinematics, corresponding to
  $\sqrt{s}=200$ GeV, and for LHC kinematics, where $\sqrt{s}=8.16$
  TeV.
  %
  In both cases, the pions are assumed to be measured at central
  rapidities, $y_{\pi^0}= 0$. 
  %
  See Refs.~\cite{d'Enterria:2013vba,Albacete:2017qng} for additional details
  regarding the theoretical calculation of inclusive pion production in
  hadronic collisions.

%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb]
\begin{center}
  \includegraphics[width=0.99\textwidth]{_inputs/nNNPDF20/plots/R_Pb_pi0.pdf}
 \end{center}
 \vspace{-0.8cm}
\caption{\small The nuclear modification ratio $R_{\rm Pb}^{\pi^0}$ for
  the production of neutral pions in proton-lead collisions as a
  function of the pion transverse momentum $p_T$.
  %
  We provide theoretical predictions based on NLO QCD and the DSS14
  hadron fragmentation functions both for \texttt{nNNPDF2.0} and \texttt{EPPS16}, with the
  corresponding nPDF uncertainties in each case.
  %
  Results are provided for the RHIC kinematics (left), corresponding to
  $\sqrt{s}=200$ GeV, and for the LHC kinematics (right), where
  $\sqrt{s}=8.16$ TeV, and in both cases pions are produced centrally,
  $|y_{\pi^0}|=0$.
  %
  \label{fig:plot_R_all}
}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%

From Fig.~\ref{fig:plot_R_all} we can see that the \texttt{nNNPDF2.0} prediction
for $R_{\rm Pb}^{\pi^0}$ is consistent with unity within uncertainties
for all values of $p_T$ both at RHIC and LHC kinematics.
%
At RHIC kinematics, we find that the ratio is less than one at the
smallest $p_T$ values, becomes $R > 1$ between $p_T=3$ and 17 GeV, and
then goes back to $R<1$.
%
Since inclusive hadron production is dominated by quark-gluon
scattering, in particular the scattering of valence quarks for
neutral pion production, this behaviour is consistent with the results shown in
Fig.~\ref{fig:R_Pb}. 
%
From low to high $p_T$, one moves from the
shadowing region to the anti-shadowing enhancement, and ends
in the region sensitive to EMC suppression.
%
A similar explanation can be made for the trends in $R_{\rm Pb}^{\pi^0}$
at the LHC kinematics. 
%
However, here the ratio
$p_T/\sqrt{s}$ does not become large enough to reach the EMC region, and
thus the ratio remains larger than one for most of the $p_T$ range as a result 
of anti-shadowing effects.
%
Lastly, the \texttt{EPPS16} predictions agree with the \texttt{nNNPDF2.0}
result well within uncertainties, reflecting the underlying consistency 
at the nPDF level.

Overall, the results of Fig.~\ref{fig:plot_R_all} confirm that inclusive hadron
production in proton-nucleus collisions can provide 
a handle on the nuclear PDF modifications at medium and large-$x$, 
although an optimal interpretation of the experimental data can only be 
achieved by the simultaneous determination of the nPDFs together 
with the hadron fragmentation functions.


\section{Proton and nuclear PDFs for the Electron-Ion Collider} 
\label{s1:EIC}
The construction of an Electron-Ion Collider
(EIC)~\cite{Accardi:2012qut,Aschenauer:2017jsk} has been recently approved by
the United States Department of Energy at Brookhaven National Laboratory, and
could record the first scattering events as early as 2030. By colliding
(polarized) electron or positron beams with proton or ion beams for a range of
center-of-mass energies, the EIC will perform key measurements to investigate
quantum chromodynamics (QCD) at the intensity frontier. These measurements will
be fundamental to understand how partons are distributed in position and
momentum spaces within a proton, how the proton spin originates from the spin
and the dynamics of partons, how the nuclear medium modifies partonic
interactions, and whether gluons saturate within heavy nuclei.

In this section we focus on one important class of EIC measurements, namely
inclusive cross sections for unpolarized lepton-proton and lepton-nucleus
deep-inelastic scattering (DIS). In particular we study how such data could
improve the determination of the unpolarized proton and nuclear parton
distribution functions (PDFs)~\cite{Ethier:2020way} by incorporating suitable
pseudodata in a self-consistent set of PDF fits based on the NNPDF methodology
(see Ref.~\cite{Ball:2014uwa} and references therein for a comprehensive
description). The unique ability of an EIC to measure inclusive DIS cross
sections consistently for the proton and a wide range of nuclei will be
exploited also to update the proton PDFs used as a boundary condition in the
nuclear PDF fit. This feature distinguishes our analysis from previous
studies~\cite{Aschenauer:2017oxs,AbdulKhalek:2019mzd}, and may be extended to a
simultaneous determination of proton and nuclear PDFs in the future. The
results presented in this work integrate those contained in Sects.~7.1.1 and
7.3.3 of the upcoming EIC Yellow Report~\mycite{AbdulKhalek:2021gbh}. They systematically
account for the impact of projected inclusive DIS measurements at an EIC on the
unpolarized proton PDFs for the first time (for projected semi-inclusive DIS
measurements see Ref.~\cite{Aschenauer:2019kzf}), and supersede a previous
NNPDF analysis of the impact of EIC measurements on nuclear
PDFs~\mycite{AbdulKhalek:2019mzd}. Similar studies for polarized PDFs have been
performed elsewhere~\cite{Aschenauer:2012ve,Aschenauer:2013iia,
  Aschenauer:2015ata,Aschenauer:2020pdk}, including in the NNPDF
framework~\cite{Ball:2013tyh}.

We first describe how EIC pseudodata
are generated. We then study how they affect the proton and nuclear PDFs once
they are fitted. Lastly, we illustrate how an updated determination of nuclear
PDFs can affect QCD at the cosmic frontier, in particular predictions for
the interactions of highly-energetic neutrinos with matter as they propagate
through Earth towards large-volume detectors.

\myparagraph{Pseudodata generation}
In this analysis we use the same pseudodata as in the EIC Yellow
Report~\mycite{AbdulKhalek:2021gbh}, see in particular Sect.~8.1. In the case of lepton-proton
DIS, they consist of several sets of data points corresponding to either the
neutral-current (NC) or the charged-current (CC) DIS reduced cross sections,
$\sigma^\text{NC}$ and $\sigma^\text{CC}$, respectively. See, \textit{e.g.}, Eqs.~(7)
and (10) in Ref.~\cite{Ball:2008by} for their definition.
Both electron and positron beams are considered, for various forecast energies
of the lepton and proton beams. In the case of lepton-nucleus DIS, the
pseudodata correspond only to NC DIS cross sections, see, \textit{e.g.}, the
discussion in Sect.~2.1 of Ref.~\mycite{AbdulKhalek:2019mzd} for their definition.
Both electron and positron beams are considered in conjunction with a deuteron
beam; only an electron beam is instead considered for other ions, namely
$^4$He, $^{12}$C, $^{40}$Ca, $^{64}$Cu, and $^{197}$Au.
A momentum transfer $Q^2>1$~GeV$^2$, a squared invariant mass of the system
$W^2>10$~GeV$^2$ and a fractional energy of the virtual particle exchanged in
the process $0.01\leq y \leq 0.95$ are assumed in all of the above cases,
consistently with the detector requirements outlined in Sect.8.1
of~\mycite{AbdulKhalek:2021gbh}.

The pseudodata distribution is assumed to be multi-Gaussian, as in the case
of real data. It is therefore uniquely identified by a vector of mean values
$\bm{\mu}$ and a covariance matrix $\bm{C}$, for which the following
assumptions are made. The mean values correspond to the theoretical expectations
$\bm{t}$ of the DIS cross sections obtained with a \textit{true} underlying set of
PDFs, and smeared by normal random numbers $\bm{r}$ sampled from the Cholesky decomposition $\bm{L}$ of the covariance matrix such that $\bm{\mu = t + L\cdot r}$ (see Sect.~\ref{s2:monte_carlo}). Specifically we use a recent
variant~\cite{Faura:2020oom} of the NNPDF3.1 determination~\cite{Ball:2017nwa},
and the \texttt{nNNPDF2.0} determination~\mycite{AbdulKhalek:2020yuc}, for proton and
nuclear PDFs, respectively. The covariance matrix is made up of three
components, which correspond to a statistical uncertainty, an additive
uncorrelated systematic uncertainty, and a multiplicative correlated
systematic uncertainty. The statistical uncertainty is determined by assuming
an integrated luminosity $\mathcal{L}$ of 100 fb$^{-1}$ for electron-proton
NC and CC DIS, and of 10 fb$^{-1}$ in all other cases. The systematic
uncertainties are instead determined with the \textsc{djangoh} event
generator~\cite{Charchula:1994kf}, which contains the Monte Carlo program
\textsc{heracles}~\cite{Kwiatkowski:1990es} interfaced to
\textsc{lepto}~\cite{Ingelman:1996mq}. These pieces of software collectively allow
for an account of one-loop electroweak radiative corrections and radiative
scattering. The Lund string fragmentation model, as implemented in
\textsc{pythia/jetset} (see, \textit{e.g.}, Ref.~\cite{Sjostrand:2019zhc} and
references therein) is used to obtain the complete hadronic final state.
The non-perturbative proton and nuclear PDF input is made available to
\textsc{djangoh} by means of numeric tables corresponding to the relevant NC and
CC DIS structure functions, which were generated with
\textsc{apfel}~\cite{Bertone:2013vaa} in the format of
\textsc{lhapdf}~\cite{Buckley:2014ana} grids. The optimal binning of the pseudodata
is determined accordingly.

The complete set of pseudodata considered in this work is summarized in
Table~\ref{tab:EIC_pseudodata}. For each pseudodata set, we indicate the
corresponding DIS process, the number of data points $N_\text{dat}$ before (after)
applying kinematic cuts (see below), the energy of the lepton and of the proton
or ion beams $E_\ell$ and $E_p$, the center-of-mass energy $\sqrt{s}$, the
luminosity $\mathcal{L}$, and the relative uncorrelated and correlated
systematic uncertainties (in percentage) $\sigma_u$ and $\sigma_c$.
Two different scenarios, called \textit{optimistic} and \textit{pessimistic}
henceforth, are considered, which differ for the number of data points and
for the size of the projected systematic uncertainties. In the case of NC
cross sections, the uncorrelated uncertainty was estimated to be 1.5\% (2.3\%)
in the optimistic (pessimistic) scenario. These uncertainties originated from a 1\%
uncertainty on the radiative corrections, and a 1\% (2\%) uncertainty due to
detector effects. The normalization uncertainty was set to 2.5\% (4.3\%). This
included a 1\% uncertainty on the integrated luminosity and a 2\% (4\%)
uncertainty due to detector effects. In the case of CC cross sections,
an uncorrelated uncertainty of 2\% was used in both the optimistic and
pessimistic scenarios, while a normalization uncertainty of 2.3\% (5.8\%)
was used in the optimistic (pessimistic) scenario. This uncertainty includes
contributions from luminosity, radiative corrections and simulation errors.

Estimating systematic uncertainties for an accelerator and a detector which
have not yet been constructed is particularly challenging. The percentages
given in Table~\ref{tab:EIC_pseudodata} build upon the experience of previous
experiments (primarily those at HERA) as well as simulation studies performed
using the EIC Handbook detector and the current EIC detector
matrix~\cite{AbdulKhalek:2021gbh}. Relative systematic uncertainties are
estimated to be independent from the values of $x$ and $Q^2$, in contrast to
statistical uncertainties. For NC pseudodata (with $\mathcal{L}$=100~fb$^{-1}$),
systematic uncertainties are significantly larger than statistical
uncertainties in much of the probed kinematic phase space, see \textit{e.g.}
Figs.~7.1 and 7.67 in~\mycite{AbdulKhalek:2021gbh}. Conversely, for CC pseudodata,
systematic uncertainties are comparable to statistical uncertainties for most
of the measured kinematic space.

%-------------------------------------------------------------------------------
\begin{table}%[ht] %%[ht]
  \footnotesize
  \centering
  \input{_tables/EIC_pseudodata.tex}
  \vspace{0.3cm}
  \caption{The EIC pseudodata sets considered in this work. For each of them we
    indicate the corresponding DIS process, the number of data points
    $N_\text{dat}$ in the optimistic/pessimistic scenarios before (after)
    kinematic cuts, the energy of the lepton and of the proton or ion beams
    $E_\ell$ and $E_p$, the center-of-mass energy $\sqrt{s}$, the integrated
    luminosity $\mathcal{L}$, and the relative uncorrelated and correlated
    systematic uncertainties (in percentage) $\sigma_u$ and $\sigma_c$
    in the optimistic/pessimistic scenarios.}
  \label{tab:EIC_pseudodata}
\end{table}
%-------------------------------------------------------------------------------

%-------------------------------------------------------------------------------
\begin{figure}[htb]
 \centering
 \includegraphics[width=\textwidth,clip=true,trim=0 0cm 0 0cm]{_plots/EIC_kinematics.pdf}
 \vspace{-0.8cm}
 \caption{The expected kinematic coverage in the $(x,Q^2)$ plane of the EIC
   pseudodata for lepton-proton or lepton-deuteron (left) and lepton-nucleus
   (right panel) collisions, see Table~\ref{tab:EIC_pseudodata}. Shaded areas
   indicate the approximate kinematic coverage of the available inclusive DIS
   measurements. The dashed lines denote the kinematic cuts used in the PDF
   fits, $Q^2 \ge 3.5$ GeV$^2$ and $W^2 \ge 12.5$ GeV$^2$.}
 \label{fig:EIC_kinematics}
\end{figure}
%-------------------------------------------------------------------------------

The kinematic coverage of the EIC pseudodata in the ($x,Q^2$) plane is displayed
in Fig.~\ref{fig:EIC_kinematics} for the optimistic scenario. Pseudodata for
lepton-proton and lepton-deuteron are separated from pseudodata for electron-ion
collisions via different panels. The approximate coverage of currently available
inclusive DIS measurements is shown as a shaded area. Dashed lines correspond
to the kinematic cuts used in the PDF fits described below. From
Fig.~\ref{fig:EIC_kinematics}, we already can appreciate the relevance of the EIC
for the determination of nuclear PDFs. In this case, the EIC measurements extend
the kinematic reach of DIS by more than one order of magnitude in both $x$ and
$Q^2$. In the case of proton PDFs, instead, the EIC measurements mostly
overlap with those already available, in particular from HERA, except for a
slightly larger extension at very high $x$ and $Q^2$.

\myparagraph{Fitting procedure}
We include the pseudodata in the series of fits summarized in
Table~\ref{tab:fits}. All these fits use the NNPDF methodology. Because nuclear
PDFs are correlated with proton PDFs (the former should reduce to the latter in
the limit $A\to 1$, where $A$ is the nucleon number), and because the EIC
measurements of Table~\ref{tab:EIC_pseudodata} will affect both, we determine them
sequentially.
%-------------------------------------------------------------------------------
\begin{table}%[ht] %%[ht]
  \footnotesize
  \centering
  \input{_tables/EIC_fits.tex}
  \caption{A summary of the fits performed in this study, see text for details.}
  \label{tab:fits}
\end{table}
%-------------------------------------------------------------------------------

First, we focus on the proton PDFs, and perform the NNPDF3.1+EIC optimistic and
pessimistic fits. These are a rerun of the \texttt{base} fit of
Ref.~\cite{Faura:2020oom}, which is now augmented with the $e^\pm p$ (CC and NC)
and $e^\pm d$ (NC) EIC pseudodata sets for the optimistic and pessimistic
scenarios. As in Ref.~\cite{Ball:2017nwa,Faura:2020oom}, they are all
made of $N_\text{rep}=100$ Monte Carlo replicas. After kinematic cuts, the fits
include a total of 5264 (5172) data points in the optimistic (pessimistic)
scenario, out of which 1286 (1194) are EIC pseudodata and 3978 are real data
(see Ref.~\cite{Faura:2020oom} for details). Kinematic cuts are the same as
in Ref.~\cite{Ball:2017nwa,Faura:2020oom}, specifically
$Q^2>3.5$~GeV$^2$ and $W^2>12.5$~GeV$^2$. These cuts, which serve the purpose
of removing a kinematic region in which potentially large higher-twist and
nuclear effects may spoil the accuracy of the PDF analysis, are more
restrictive than those used to generate the pseudodata. This fact is however
not contradictory, and reproduces what customarily happens with real data, when
different kinematic cuts are used in the experimental analysis and in a fit.
These fits are accurate to next-to-next-to-leading order (NNLO) in perturbative
QCD, they utilize the FONLL scheme~\cite{Forte:2010ta,Ball:2015tna,Ball:2015dpa}
to treat heavy quarks, and they include a parametrization of the charm PDF on
the same footing as the lighter quark PDFs. In comparison to the original
NNPDF3.1 fits~\cite{Ball:2017nwa}, a bug affecting the computation of
theoretical predictions for charged-current DIS cross sections has been
corrected, the positivity of the $F_2^c$ structure function has been enforced,
and NNLO massive corrections~\cite{Berger:2016inr,Gao:2017kkx} have been
included in the computation of neutrino-DIS structure functions.

We then focus on nuclear PDFs, and perform the NNPDF3.1\_pch+EIC and
\texttt{nNNPDF2.0}+EIC optimistic and pessimistic fits. These are a rerun of the
proton and nuclear baseline determinations of Ref.~\mycite{AbdulKhalek:2020yuc},
augmented respectively with the $e^\pm p$ (CC and NC) and the $e^-A$ (NC),
$A=d$, $^4$He, $^{12}$C, $^{40}$Ca, $^{64}$Cu, and $^{197}$Au,
pseudodata sets for the optimistic and pessimistic scenarios.
As in Ref.~\mycite{AbdulKhalek:2020yuc}, the proton (nuclear) fits are made of
$N_\text{rep}=100$ ($N_\text{rep}=250$) Monte Carlo replicas. After kinematic 
cuts, the NNPDF3.1\_pch+EIC fits include a total of 4147 (4055) data points
in the optimistic (pessimistic) scenario, out of which 846 (754) are EIC
pseudodata and 3301 are real data (see Ref.~\mycite{AbdulKhalek:2020yuc} for
details). The nuclear fits include a total of 3007 data points, out of which
1540 are EIC pseudodata and 1467 are real data. Kinematic cuts are the same as
above, and are in turn equivalent to these used in
Refs.~\cite{Ball:2017nwa,AbdulKhalek:2020yuc}. These fits are accurate to
next-to-leading order (NLO) in perturbative QCD, and assume that charm is
generated perturbatively, consistent with Ref.~\mycite{AbdulKhalek:2020yuc}.

Although the proton and nuclear PDF fits are performed independently,
they remain as consistent as possible. Most importantly, the unique
feature of an EIC to measure DIS cross sections with a comparable accuracy and
precision for a wide range of nuclei and for the proton is
key to inform the fit of nuclear PDFs as much as possible. Not only
do the measurements on nuclear targets enter the fit directly, but also the
measurements on a proton target are first used to update the necessary
baseline proton PDF determination. This feature distinguishes our work from
previous similar studies~\cite{Aschenauer:2017oxs,AbdulKhalek:2019mzd}, where
only the effect of measurements on nuclear targets were taken into account in
the determination of nuclear PDFs. A simultaneous determination of proton and
nuclear PDFs might eventually become advisable at an EIC, should the
measurements be sufficiently precise to make an independent determination
less reliable.

We also note that the pseudodata sets for a deuteron target are alternatively
included in the fit of proton PDFs or in the fit of nuclear PDFs. To avoid
double counting, they are not included in the fit of proton PDFs used
as baseline for the fit of nuclear PDFs. This choice follows the common
practice to include fixed-target DIS data on deuteron targets in fits of proton
PDFs, as done, \textit{e.g.}, in NNPDF3.1 and in the variant fit used here to
generate the pseudodata. The reason being that they are essential to achieve a
good quark flavour separation. The EIC pseudodata sets for a deuteron target
are then treated, in the proton PDF fits performed here, similarly to the
fixed-target DIS data already included in NNPDF3.1. Specifically we assume
that nuclear corrections are negligible, and therefore we do not include them.
This assumption could be overcome by means of a simultaneous fit of proton and
nuclear PDFs, or by means of the iterative procedure proposed
in Ref.~\cite{Ball:2020xqw}, whereby proton and deuteron PDFs are determined by
subsequently including the uncertainties of each in the other. Any of these
approaches goes beyond the scope of this work, as they will have little
applicability in the context of pseudodata.

\myparagraph{Results} We now turn to discuss the results of the fits collected
in Table~\ref{tab:EIC_pseudodata}. As expected, the goodness of each fit 
measured by the $\chi^2$ per number of data points is comparable to that of the
fits used to generate the pseudodata. The description of each data set remains
unaltered within statistical fluctuations, and the $\chi^2$ per
number of data points for each of the new EIC pseudodata sets is of order one,
as it should by construction. In the following we therefore exclusively discuss
how the EIC pseudodata affect PDF uncertainties.

In Fig.~\ref{fig:ppdfs} we show the relative uncertainty of the proton PDFs
in the NNPDF3.1 fit variant used to generate the pseudodata, and in the
NNPDF3.1+EIC fits, both for the optimistic and pessimistic scenarios. In each
case, uncertainties correspond to one standard deviation, and are computed
as a function of $x$ at $Q^2=100$~GeV$^2$. Only the subset of flavours (or
flavour combinations) that are the most affected by the EIC
pseudodata are shown: $u$, $d/u$, $s$ and $g$.

%-------------------------------------------------------------------------------
\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth,clip=true,trim=1.5cm 0cm 1.5cm 2cm]{_plots/EIC_pPDFs.pdf}
  \vspace{-0.8cm}
  \caption{The relative uncertainty of the proton PDFs determined in the
  NNPDF3.1 fit variant used to generate the pseudodata, and in the
  NNPDF3.1+EIC fits, in the optimistic and pessimistic scenarios. Uncertainties
  correspond to one standard deviation and are computed as a function of $x$
  at $Q^2=100$~GeV$^2$. Only the subset of flavours (or flavour combinations) that
  are the most affected by the EIC pseudodata are shown, namely $u$,
  $d/u$, $s$ and $g$. Note the use of a log/linear scale on the $x$ axis.}
  \label{fig:ppdfs}
\end{figure}
%-------------------------------------------------------------------------------

Fig.~\ref{fig:ppdfs} allows us to make two conclusions. First, the impact of the
EIC pseudodata is localized in the large-$x$ region, as expected from their
kinematic reach (see Fig.~\ref{fig:EIC_kinematics}). This impact is significant in
the case of the $u$ PDF, for which PDF uncertainties could be reduced by up to
a factor of two for $x\gtrsim 0.7$. The impact is otherwise moderate for the
$d/u$ PDF ratio (for which it amounts to an uncertainty reduction of about
one third for $0.5\lesssim x \lesssim 0.6$) and for the $s$ PDF (for which 
it amounts to an uncertainty reduction of about one fourth for
$0.3\lesssim x \lesssim 0.6$). The relative uncertainty of the gluon PDF, and
of other PDFs not shown in Fig.~\ref{fig:ppdfs}, remains unaffected.
These features rely on the unique ability of the EIC to perform precise DIS
measurements at large $x$ and large $Q^2$: their theoretical interpretation
remains particularly clean, as any non-perturbative large-$x$ contamination
due, \textit{e.g.}, to higher-twist effects, is suppressed. This possibility
distinguishes the EIC from HERA, which had a similar reach at high $Q^2$ but a
more limited access at large-$x$, and from fixed-target experiments
(including the recent JLab-12 upgrade~\cite{Dudek:2012vr}), which can access the
high-$x$ region only at small $Q^2$. Secondly, the impact of the EIC pseudodata
does not seem to depend on the scenario considered: the reduction of PDF
uncertainties remains comparable irrespective of whether optimistic or
pessimistic pseudodata projections are included in the fits. Because the two
scenarios only differ in systematic uncertainties, we conclude that it may be
sufficient to control these to the level of precision forecast
in the pessimistic scenario.

A similar behaviour is observed for the NNPDF3.1\_pch fits, which are therefore
not displayed. In Figs.~\ref{fig:npdfs} we show the relative uncertainty of the
nuclear PDFs in the \texttt{nNNPDF2.0} fit used to generate the pseudodata, and in the
\texttt{nNNPDF2.0}+EIC fits, both in the pessimistic and in the optimistic scenarios.
Uncertainties correspond to one standard deviation, and
are computed as a function of $x$ at $Q^2$=100~GeV$^2$. Results
are displayed for the ions with the lowest and highest atomic mass, $^4$He and
$^{197}$Au, and for an intermediate atomic mass ion, $^{64}$Cu,
and only for the PDF flavours that are the most affected by
the EIC pseudodata: $u$, $\bar{d}$, $s$ and $g$.

%-------------------------------------------------------------------------------
\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth,clip=true,trim=1.5cm 2.5cm 1.5cm 3.5cm]{_plots/He_Au_nPDFs.pdf}
  \vspace{-0.8cm}
  \caption{The relative uncertainty of the nuclear PDFs determined in the
  \texttt{nNNPDF2.0} fit used to generate the pseudodata, and in the \texttt{nNNPDF2.0}+EIC fits,
  in the optimistic and pessimistic scenarios. Uncertainties correspond to one
  standard deviation, and are computed as a function of $x$ at
  $Q^2$=100~GeV$^2$. Results are displayed for the ions with the lowest and
  highest atomic mass, $^4$He (left) and $^{197}$Au (right), and for an
  intermediate atomic mass ion, $^{64}$Cu (middle column), and only for the
  PDF flavours that are the most affected by the EIC pseudodata: $u$, $\bar{d}$,
  $s$ and $g$. Note the use of a log/linear scale on the $x$ axis.}
  \label{fig:npdfs}
\end{figure}
%-------------------------------------------------------------------------------

From Fig.~\ref{fig:npdfs} we observe a reduction of nuclear
PDF uncertainties, due to EIC pseudodata, that varies with the nucleus, the
$x$ region considered, and the PDF. Overall, the heavier the nucleus,
the largest the reduction of PDF uncertainties. This is a consequence of the
fact that nuclear PDFs are customarily parametrized as continuous functions
of the nucleon number $A$: nuclear PDFs for $^4$He, which differ from the proton
PDF boundary by a small correction, are better constrained than nuclear PDFs
for $^{197}$Au because proton data are more abundant than data for nuclei.
In this respect, the EIC will allow one to perform a comparatively accurate
scan of the kinematic space for each nucleus individually, and, as shown in
Fig.~\ref{fig:npdfs}, to determine the PDFs of all ions with a similar
precision. The reduction of PDF uncertainties is localized in the small-$x$
region, where little or no data are currently available
(see Fig.~\ref{fig:EIC_kinematics}), and
in the large-$x$ region, where nuclear PDF benefit from the increased precision
of the baseline proton PDFs. In the case of the gluon PDF, the reduction of
uncertainties is seen for the whole range in $x$. This is a consequence of the
extended data coverage in $Q^2$, which allows one to constrain the gluon PDF
even further via perturbative evolution. As observed in the case of
proton PDFs, the fits obtained upon inclusion of the EIC pseudodata do not
significantly differ whether the optimistic or the pessimistic scenarios are
considered, except for very small values of $x$. In this case the optimistic
scenario leads to a more marked reduction of PDF uncertainties, especially for
the total PDF combinations $u^+$ and $d^+$. This feature is mainly driven by the
smaller systematic uncertainties that affect the NC pseudodata in the optimistic
scenario (about 3\%) with respect to the pessimistic one (about 5\%), see
Table~\ref{tab:EIC_pseudodata}. That is aligned with the fact that the statistical
uncertainties are comparable between the two scenarios. 

\myparagraph{Implications for neutrino astrophysics} The reduction of PDF
uncertainties due to EIC pseudodata, in particular for
nuclear PDFs, may have important phenomenological implications. Not only at the
intensity frontier, \textit{e.g.} to characterize gluon saturation at small $x$,
but also at the energy frontier, \textit{e.g.}, for searches of new physics that
require a precise knowledge of PDFs at high $x$, and at the cosmic frontier,
\textit{e.g.}, in the detection of highly energetic neutrinos from astrophysical
sources. We conclude this section by focusing on this last aspect. Specifically
it was shown in Ref.~\cite{Garcia:2020jwr} that the dominant source of
uncertainty in the theoretical predictions for the cross section of
neutrino-matter interactions is represented by nuclear effects.
The corresponding NC and CC inclusive DIS cross sections may differ
significantly depending on whether they are computed for neutrino-nucleon or
neutrino-nucleus interactions. The uncertainty is larger in the latter case,
because nuclear PDFs are not as precise as proton PDFs, and is such that it
encompasses the difference in central values. We revisit this statement in
light of the precise nNNPDF3.0+EIC fits.

In Fig.~\ref{fig:UHExsec} we show the CC (left) and NC (right)
neutrino-nucleus inclusive DIS cross sections, with their one-sigma PDF
uncertainties, as a function of the neutrino energy $E_\nu$. Moreover, in
Fig.~\ref{fig:attenuation} we show the transmission coefficient $T$ for muonic
neutrinos, defined as the ratio between the incoming neutrino flux $\Phi_0$ and
the flux arriving at the detector volume $\Phi$ (see Eq.~(3.1) and the ensuing
discussion in Ref.~\cite{Garcia:2020jwr} for details); $T$ is displayed for two
values of the nadir angle $\theta$ as a function of the neutrino energy $E_\nu$.
In both cases, we compare predictions obtained with the calculation presented
in Refs.~\cite{Bertone:2018dse,Garcia:2020jwr} and implemented in
\textsc{hedis}~\cite{Brown:1971qr}. For a proton target the prediction is made
with the proton PDF set determined in Ref.~\cite{Gauld:2016kpd},
a variant of the NNPDF3.1 PDF set in which small-$x$ resummation
effects~\cite{Ball:2017otu} and additional constraints from $D$-meson
production measurements in proton-proton collisions at 5,7 and
13~TeV~\cite{Aaij:2013mga,Aaij:2015bpa,Aaij:2016jht} have been included.
This prediction is labeled HEDIS-BGR in
Figs.~\ref{fig:UHExsec}-\ref{fig:attenuation}. For a nuclear
target ($A=31$ is adopted as in Ref.~\cite{Garcia:2020jwr}), the prediction is
made alternatively with the \texttt{nNNPDF2.0} and the \texttt{nNNPDF2.0}+EIC (optimistic) PDFs.
The corresponding predictions are labeled HEDIS-nBGR [\texttt{nNNPDF2.0}] and HEDIS-nBGR
[\texttt{nNNPDF2.0} (EIC)] in Figs.~\ref{fig:UHExsec}-\ref{fig:attenuation}. Predictions
are all normalized to the central value of the proton result. In comparison to
\texttt{nNNPDF2.0}, the effect of the EIC pseudodata is seen to reduce the uncertainty
of the prediction for a nuclear target by roughly a factor of two for
$E_\nu\simeq 10^6$~GeV. The reduced uncertainty no longer encompasses the
difference between predictions obtained on a proton or on a nuclear target,
except in the case of an attenuation rate computed with a large nadir angle.
Furthermore, this reduction extends to much larger neutrino energy
($E_\nu \gtrsim 10^7$), beyond the EIC-sensitive $x$-region
of the PDFs. We believe this to be partly due to DGLAP evolution and sum rules
that smoothen the low-$x$ PDF behaviour, but also potentially a consequence of
the factorisation approximation used to account for nuclear corrections in the
ultra high-energy cross-sections highlighted by Eqs.~(5.2, 5.3) in
Ref.~\cite{Garcia:2020jwr}.

%-------------------------------------------------------------------------------
\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth]{_plots/xsec_nuclear_new-2.pdf}
  \vspace{-0.8cm}
  \caption{The CC (left) and NC (right) neutrino-nucleus DIS cross
  sections, with their one-sigma uncertainties, as a function of the neutrino
  energy $E_{\nu}$. Predictions correspond to the HEDIS-BGR
  computation~\cite{Garcia:2020jwr} with the proton PDF of~\cite{Gauld:2016kpd},
  and with the \texttt{nNNPDF2.0} and \texttt{nNNPDF2.0}+EIC nuclear PDFs. They are all
  normalized to the central value of the proton results. See text for details.}
  \label{fig:UHExsec}
\end{figure}
%-------------------------------------------------------------------------------

%-------------------------------------------------------------------------------
\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth]{_plots/attenuation-2.pdf}
  \vspace{-0.8cm}
  \caption{The transmission coefficient $T$ for muonic neutrinos as a function
  of the neutrino energy $E_\nu$ and for two values of the nadir angle $\theta$.
  Predictions correspond to the computation of~\cite{Garcia:2020jwr} with the
  proton PDF of~\cite{Gauld:2016kpd}, and with the \texttt{nNNPDF2.0} and \texttt{nNNPDF2.0}+EIC
  nuclear PDFs. They are all normalized to the central value of the proton
  results. See text for details.}
  \label{fig:attenuation}
\end{figure}
%-------------------------------------------------------------------------------
\begin{comment}
\myparagraph{Summary} In this section we have quantified the impact that
unpolarized lepton-proton and lepton-nucleus inclusive DIS cross section
measurements at the future EIC will have on the unpolarized proton and nuclear
PDFs. In particular, we have extended the NNPDF3.1 and \texttt{nNNPDF2.0} global
analyses by including suitable NC and CC DIS pseudodata corresponding to a
variety of nuclei and center-of-mass energies. Two different scenarios,
optimistic and pessimistic, have been considered for the projected systematic
uncertainties of the pseudodata. We have found that the EIC could reduce the
uncertainty of the light quark PDFs of the proton at large $x$, and, more
significantly, the quark and gluon PDF uncertainties for nuclei in a wide range
of atomic mass $A$ values both at small and large $x$. In general the size of
this reduction turns out to be similar for both the optimistic and
pessimistic scenarios. We therefore conclude that it may be sufficient to
control experimental uncertainties to the level of precision forecast in the
latter scenario. Lastly, we have illustrated how theoretical predictions
obtained with nuclear PDFs constrained by EIC data will improve the modelling
of the interactions of ultra-high energy cosmic neutrinos with matter.
In particular we have demonstrated that nuclear PDF uncertainties may
no longer encompass the difference between predictions obtained on a proton and
on a nuclear target. This fact highlights the increasing importance of carefully
accounting for nuclear PDF effects in high-energy neutrino astrophysics.

Further phenomenological implications could be investigated
in the future, for instance whether a simultaneous determination of proton and
nuclear PDFs can improve the constraints provided by the EIC data in comparison
to the self-consistent strategy adopted in this analysis, or the extent to which
semi-inclusive DIS (SIDIS) data can further improve both proton and nuclear
PDF determinations. The PDF sets discussed in this work are available in the
LHAPDF format~\cite{Buckley:2014ana} from the NNPDF website:
\begin{center}
\url{http://nnpdf.mi.infn.it/for-users/nnnpdf2-0eic/}
\end{center}
\end{comment}

==> _inputs/theory_appendices.tex <==
%% The "\appendix" call has already been made in the declaration
%% of the "appendices" environment (see thesis.tex).

%\setsecnumdepth{subsection}
%\settocdepth{section}

%\setcounter{chapter}{-1}
%\chapter{Basics}
%\chapterquote{You first learn Newton's law of motion in terms of position and velocities of particles, then you learn about more general formulation of the equations: the Lagrangian formulation where you have quite a general dynamical coordinates, coordinates which are any functions of the position of the particles and then you have the velocities corresponding to these coordinates. Now Hamilton, a hundred years previously has setup another form of dynamics in which the coordinates are replaced by momentum variables, now you might think that this is not an important change but it led to greater symmetry and beauty in the equations, and Hamilton pursued this line of investigation just because he was thriving for mathematical beauty, I believe this shows very strongly the genius of Hamilton that he was able to follow through a line of work whose importance was not made evident until a hundred years later. I don't think there's any other such examples in the history of physics.}{Paul Dirac, From Dirac's Lectures - Christchurch, New Zealand (1975)} 
%\label{chap:0}
\chapter{Theoretical foundations}
The leap from Lagrangian~\cite{lagrange1853mecanique} and Hamiltonian~\cite{hand1998analytical} classical mechanics~\cite{landau2000mechanics,landau2013classical} to the state of the art quantum chromodynamics~\cite{cowan1964electron,
gell1964schematic,
zweig1964,
bloom1969high,
bjorken1969asymptotic,
callan1969high,
feynman1969very,
feynman2018photon,
Blumlein:2012bf,
nambu1966preludes,
faddeev1967feynman,
hooft1971renormalization,
fritzsch2002current,
fritzsch1973advantages,
gross1973ultraviolet,
politzer1973reliable}
is at the least that of the last two centuries of scientific progress. This gigantic leap is not uniform as most of the revolutionary theories and discoveries were piled rapidly within the last century, nor is it continuous as we have gained fundamentally new perspectives on nature at the scale of atoms and subatomic particles~\cite{Dirac1930-DIRTPO,peskin2018introduction}. Therefore, by no means this chapter is meant to encapsulate nor do justice this important evolution of subatomic physics; nowadays, with the level of advancements particle physics is witnessing, one might even question the relevancy of classical mechanics with respect to the main topic of this thesis. However, I think that these few pages will serve as a historical base and smooth introduction to quantum electrodynamics that I will build upon its structure and findings to introduce quantum chromodynamics and discuss my research on the hadronic structure of nucleons and nuclei. More importantly than the historical aspect and the natural connection between these theories, I will highlight in this chapter the important role symmetry played in shaping their mathematical formalisms. This specific aspect has always been a source of my fascination particularly with how it was distilled by Landau and Lifshitz in Refs.~\cite{landau2000mechanics,landau2013classical} and Dirac in Ref.~\cite{Dirac1930-DIRTPO,peskin2018introduction} which Sects.~\ref{s1:CM} and \ref{s1:CED} will be based upon.

In Sect.~\ref{s1:CM}, I discuss the theory of non-relativistic classical mechanics, that relied on an
\textit{inertial}\footnote{Inertial: a frame of reference that is not undergoing
acceleration.} reference frame with time and space as
\textit{homogeneous}\footnote{Homogeneity: various positions/instants in time and space
are equivalent.} and \textit{isotropic}\footnote{Isotropy: different orientations are
equivalent.}. This theory was adopted for centuries and was built based on the concept of absolute time and instantaneous propagation of interaction. However, it showed limitation describing light and its interaction with other particles. 

In Sect.~\ref{s1:CED}, I discuss the theory of relativistic classical mechanics in order to adress this limitation. Therefore introducing a new framework in which light has a finite speed and considered absolute (instead of time) with respect to different observers. This was rectified most generally by Einstein with his theory of special relativity~\cite{einstein2015relativity}, that reduces to Newtonian physics when the speed of the objects considered is far less than the speed of light. Building on the latter principle, Maxwell established his equations to describe light in terms of an electromagnetic field~\cite{maxwell1890scientific}. 

In Sect.~\ref{s1:QED}, I introduce quantum mechanics and electrodynamics that were a first attempt to solve the utlra-violet catastrophe~\cite{klein1961max} manifested by studying the black body radiation by means of relativistic classical mechanics. The other limitation was the photoelectric effect~\cite{einstein1905photoelectric} in which the number of emitted electrons of materials undergoing electromagnetic radiation, increased with the frequency instead of intensity (as in Maxwell's). Both of these observations required the transition from the classical point of view of seeing light as an electromagnetic wave to the quantum mechanical one where light is described as discrete bundle of energies or simply a particle.

\section{Classical mechanics} \label{s1:CM}
In classical mechanics, the state of a mechanical system is completely determined if all the coordinates and velocities are simultaneously specified. The system is characterised by a function called Lagrangian $L(\bm{q},\bm{\dot{q}},t)$ where $t$ is the absolute time and $\bm{q}$, $\bm{\dot{q}}$ are respectively the generalised coordinates and velocities of the system.

\myparagraph{Hamilton's principle of Least Action}
The motion of a mechanical system is such that the
\textit{action} defined as:
\begin{align}
    S = \int_{t_1}^{t_2} L(\bm{q},\bm{\dot{q}},t)dt,
\end{align}
takes the least possible value. Hence the motion equations are:
\begin{equation} \label{eq:Lagrange_motion_equations}
    \delta S = \int_{t_1}^{t_2} (\bm{\partial_{q}} \,L\, \cdot \bm{\delta q} + \bm{\partial_{\dot{q}}} \,L\, \cdot \bm{\delta \dot{q}}) dt =0 \implies \left(\bm{\partial_{q}} \,L\,\, - d_t \bm{\partial_{\dot{q}}} \,L\,\, \right)= 0
\end{equation}
which are invariant up to an additive total derivative to
$L$ with respect of time of some function $f(\bm{q},t)$.
%%===

\myparagraph{Galilean relativity} 
The emphasis here is on how the choice of the
relativity principle and the interpretation of space and
time dictates our laws of physics.   
Starting from the homogeneous and isotropic time and space
hypothesis, one can already make inferences concerning the
form of the Lagrangian of a particle moving freely in an
inertial frame.
 
Starting from the \textbf{Homogeneity of space and time} one deduces that
the Lagrangian cannot contain explicitly neither the radius
vector $\bm{q}$ of the particle nor the time t, i.e
$L(\bm{q},\bm{\dot{q}},t) = L(\bm{\dot{q}})$. Secondly, considering the \textbf{Isotropy of space} we further deduce that the Lagrangian must also be independent of the direction of
$\bm{\dot{q}}$, i.e $L(\bm{\dot{q}}) = L(\dot{q}^2)$. Finally and since homogeneity implies
$\bm{\partial_{\bm{q}}}\,L = 0$, we are left with
$d_t(\bm{\partial_{\bm{\dot{q}}}}\,L)=0$ from
Eq.~(\ref{eq:Lagrange_motion_equations}) hence,
$\bm{\partial_{\dot{q}}}\,L=\bm{\text{\textbf{Const}}}$ and
since it is only a function of the velocity, it follows that
$\bm{\dot{q}} = \bm{\text{\textbf{Const}}}$ which is the \textbf{Law of Inertia}.

Let us consider an inertial frame $(K)$ moving (as
of $t=0$) with velocity $\bm{\dot{\epsilon}}$ relatively to
a different frame $(K')$. The Galilean
transformations between $(K)$ and $(K')$ read:
\begin{align}
    \label{eq:galilean_transformations}
    \bm{q'} = \bm{q} + \bm{\dot{\epsilon}} t, \qquad t' &= t
\end{align} 
In order for our theory to be invariant under Eq.~(\ref{eq:galilean_transformations}), $L(\dot{q}^2)$ must then be converted by this
transformation into a function $L'$ which differs from
$L(\dot{q}^2)$, if at all, only by the total time derivative
of a function of coordinates and time. Therefore:
\begin{align}
    L' = L(\dot{q}'^2)
    = L(\dot{q}^2 + 2\bm{\dot{q} \cdot \dot{\epsilon}} + \dot{\epsilon}^2) 
    \stackrel[\text{order}]{\text{first}}{=} L(\dot{q}^2) + 2\bm{\dot{q} \cdot \dot{\epsilon}}(\partial_{\dot{q}^2}\,L)
\end{align}

Since $2\bm{\dot{q}\dot{\epsilon}}(\partial_{\dot{q}^2}\,L)$
must be a total time derivative to respect invariance, it
has to be a linear function of the velocity $\bm{\dot{q}}$,
hence $\partial_{\dot{q}^2}\,L$ should be independent of the
velocity and
therefore the Lagrangian is in this case proportional to the
square of velocity:
\begin{align}
    L &\propto \dot{q}^2 \equiv \frac{1}{2}m\dot{q}^2
\end{align}
The quantity $m$ which appears in the Lagrangian for a
freely moving particle is called the \textit{mass} of the
particle which becomes meaningful only when the additive
property is taken into account in a system of particles.

\myparagraph{System of particles interacting} 
The interaction between the particles can be described by adding to the Lagrangian, a certain function of the coordinates which depends on the nature of the interaction\footnote{This statement is only valid in classical mechanics where interactions are meant to happen instantaneously.}. We denote this function by $-U$, and thus:
\begin{align}
L = \sum_a\frac{1}{2}m_a \dot{q}_a^2 - U(\bm{q_1}, \bm{q_2},...)
\end{align}
with $q_a$, the radius vector of the $a^{th}$ particle.
We will designate the first term by a variable ${\displaystyle T =
\sum_a\frac{1}{2}m_a \dot{q}_a^2}$. $T$ and $U$ are called
respectively kinetic and potential energy and these will gain significance when we introduce formally the concept of energy.

The fact that the potential energy depends only on the
positions of the particles at a given instant shows that a
change in the position of any particle instantaneously
affects all the other particles. We may say that the
interactions are instantaneously propagated. The necessity
for interactions to be instantaneous is closely related to
the absolute nature of time in Galileo's principle of
relativity and will be invalid in relativistic mechanics.

%\myparagraph{Isotropy of time} The form of the Lagrangian: 
%\begin{align}
%    L = \sum_a\frac{1}{2}m_a \dot{q}_a^2 - U(\bm{q_1}, \bm{q_2},...)
%\end{align}
%shows that time is both homogeneous and isotropic, i.e if
%$t$ is replaced by $-t$, the Lagrangian remains unchanged
%hence if a given motion is possible in a system, so is the
%reverse motion.
%
%\myparagraph{Newton's second Law} if we substitute this
%Lagrangian, in the motion equations:
%\begin{align}
%    L = \sum_a\frac{1}{2}m_a \dot{q}_a^2 - U(\bm{q_1}, \bm{q_2},...),\,\,\, \text{in} \,\,\, d_t%(\bm{\partial_{\dot{q}_a}} L) - \bm{\partial_{q_a}} L = 0 \implies m_a d_t \bm{\dot{q}_a} = %- \bm{\partial_{q_a}} U \equiv \bm{F}
%\end{align} 
%Like $U$, $F$ depends only on the coordinates of the
%particles and not on their velocities, hence the
%acceleration depends as well only on the coordinates.

\myparagraph{Constants of motion}
During the motion of a system, there exist functions of
coordinates and velocities whose values remain constant
during the motion, and depend only on the initial
conditions. We will only consider the constants deriving from the fundamental homogeneity and isotropy of space and time, which have the important common
property of being additive.

First, and by virtue of \textbf{time
homogeneity}, the Lagrangian of a \textit{closed
system}\footnote{A closed mechanical system isn't subject to
any net force whose source is external to the system.}
system does not depend explicitly on time. The total time
derivative of the Lagrangian can therefore be written as:
\begin{align}
d_t L = \bm{\partial_{q}} L\,\bm{\dot{q}} + \bm{\partial_{\bm{\dot{q}}}}\,L\,\bm{\ddot{q}}
\end{align}
Note that if $L$ depends explicitly on time, a term
$\partial_t L$ would have to be added. Replacing
$\bm{\partial_{q}}\,L$ in accordance with Lagrange's
equations by $d_t(\bm{\partial_{\bm{\dot{q}}}}\,L)$ we
obtain:
\begin{align}
    d_t L = d_t(\bm{\partial_{\bm{\dot{q}}}}\,L)\cdot \bm{\dot{q}} + \bm{\partial_{\bm{\dot{q}}}}\,L\, \cdot \bm{\ddot{q}}
    =  \bm{\dot{u} \cdot v} + \bm{u \cdot \dot{v}}
    =  d_t(\bm{\dot{q} \cdot }\bm{\partial_{\bm{\dot{q}}}}\,L)
\end{align}
Hence we can write:
\begin{align}
    d_t(\bm{\dot{q}}\cdot \bm{\partial_{\bm{\dot{q}}}}\,L - L) \equiv d_t E = 0
\end{align}
therefore the energy $E$ is constant during the motion of a
closed system. The additivity of the energy follows
immediately from that of the Lagrangian since $E$ is a linear
function of the latter. The Lagrangian of a closed system (or one in a constant
external field) is of the form: $L = T(q,\dot{q}) - U(q)$,
where $T$ is quadratic function of the velocities.
Therefore:
\begin{align}
    \bm{\dot{q}}\cdot \bm{\partial_{\dot{q}}}\,L = 2T \implies
    E = 2T - L = 2T - T + U = T(q,\dot{q}) + U(q)
\end{align}

Second, and by virtue of
\textbf{space homogeneity}, the Lagrangian of a closed system is
unchanged by any parallel displacement of the entire system
in space. Let us therefore consider an infinitesimal
displacement $\bm{r} \rightarrow \bm{r}+\bm{\epsilon}$ and
obtain the condition for the Lagrangian to remain unchanged.
The resulting change in L:
\begin{align}
    \delta L = \sum_a \bm{\partial_{r_a}}\,L\,\cdot\delta\bm{r}_a
    =\bm{\epsilon} \cdot \sum_a \bm{\partial_{r_a}}\,L\,
    = 0 \rightarrow \sum_a \bm{\partial_{r_a}}\,L = 0
\end{align}
and since the Lagrange's equation implies:
\begin{align}
    \sum_a d_t(\bm{\partial_{\bm{\dot{q}_a}}}\,L) = d_t(\sum_a\bm{\partial_{\bm{\dot{q}_a}}}\,L) \equiv d_t(\bm{P})= 0
\end{align}
We deduce that $\bm{P} = \sum_a\bm{\partial_{\bm{\dot{q}_a}}}\,L =
\sum_a m_a\bm{\dot{q}_a}$, called the momentum of the
system, remains constant during the motion. The additivity of the momentum is evident. Moreover, unlike
the energy, the momentum of a system is equal to the sum
of its individual particles momenta $\bm{p}_a = m_a \bm{\dot{q}_a}$ whether or not their can be neglected.

%\myparagraph{Newton's third law} From the definition of
%momentum above:
%\begin{align}
%    \sum_a \bm{\partial_{q_a}}\,L = \sum_a \bm{F}_a = 0
%\end{align}
%we deduce that in a closed system, the sum of the forces on
%all the particles is zero.

\myparagraph{Canonical equations}
The Lagrangian formulation of field theory is particularly suited to relativistic dynamics because all expressions are explicitly Lorentz invariant. However we introduce in this section the Hamiltonian (or canonical) formulation that will ease our transition from classical to quantum mechanics.

While the Lagrangian formulation relies on generalised coordinates and velocities, the alternative Hamiltonian one relies on generalised coordinates and momenta:
\begin{alignat}{2}
    dL %&=  \bm{\partial_{q}}L \cdot \bm{dq} + \bm{\partial_{\dot{q}}}L \cdot \bm{d\dot{q}} \nonumber\\
       %&=  \bm{\dot{p}\cdot dq} + \bm{p \cdot d\dot{q}} \qquad && \text{Using Eq.~(\ref{eq:Lagrange_motion_equations})} \nonumber \\
       &= \bm{\dot{p}\cdot dq} + \left(d(\bm{p\cdot \dot{q}}) - \bm{\dot{q}\cdot d\dot{p}}\right) \qquad && \text{Using Eq.~(\ref{eq:Lagrange_motion_equations})} \nonumber \\
    dH & \equiv d(\bm{p\cdot \dot{q}}-L) = \bm{\dot{q}\cdot dp} - \bm{\dot{p} \cdot dq} \nonumber \\
    &H(\bm{p},\bm{q},t) = \bm{p\cdot \dot{q}} - L \qquad && \text{Hamiltonian}
\end{alignat}
Hence the Hamiltonian motion equations are:
\begin{equation}
    \label{eq:Hmotion}
    \bm{\dot{q}} = \bm{\partial_{p}}H,\qquad \bm{\dot{p}}=-\bm{\partial_{q}}H
\end{equation}

\myparagraph{Canonical transformations} 
The motion equations Eq.~(\ref{eq:Lagrange_motion_equations}) are invariant with respect to a transformation from a choice of generalised coordinates $\bm{q}$ to any other independent ones $\bm{Q}$ such as $\bm{q} \rightarrow \bm{Q} = \bm{Q}(\bm{q},t)$. Therefore the Hamiltonian equations are also invariant. One of the main advantages of the Hamiltonian formulation (that will be very relevant in Sect.~\ref{s1:QED}) is that the momenta $\bm{p}$ are independent of the coordinates $\bm{q}$ hence the transformations could be extended to:
\begin{equation}
    \bm{Q} = \bm{Q}(\bm{p},\bm{q},t), \qquad \bm{P}=\bm{P}(\bm{p},\bm{q},t)
\end{equation}
With this extension however, and in order for the Hamiltonian equations Eq.~(\ref{eq:Hmotion}) to retain their canonical form under these transformations, we must derive  conditions on $\bm{P}$ and $\bm{Q}$ which are:
\begin{equation}
    \label{eq:Canonical_conditions}
    \bm{\dot{Q}} = \bm{\partial_{P}H},\qquad \bm{\dot{P}} = - \bm{\partial_Q}H
\end{equation}
Any transformation respecting Eq.~(\ref{eq:Canonical_conditions}) is called canonical and keep the motion equations intact.

Due to the symmetry of the Hamiltonian formulation and the canonical transformations, the distinction between $\bm{Q}$ and $\bm{P}$ is irrelevant as one can see for example that setting $\bm{Q} = \bm{p}$ and $\bm{P}=-\bm{q}$ does not affect the canonical form of the equations. Taking into account this arbitrariness of nomenclature, we call $\bm{p}$ and $\bm{q}$ to be canonically conjugate quantities in the Hamiltonian formulation.

\myparagraph{Poisson brackets} 
We define the Poisson brackets to be:
\begin{equation} \label{eq:Poisson_brackets}
    \{H,f\}_{Poisson} \equiv \bm{\partial_p}H \cdot \bm{\partial_q} f - \bm{\partial_q}H \cdot \bm{\partial_p}f
\end{equation}
where $H$ is the Hamiltonian and $f=f(\bm{p},\bm{q},t)$ an arbitrary function of coordinates momenta and time and its total time derivative is:
\begin{equation}
    d_t f = \partial_t f + \{H,f\}_{Poisson}     
\end{equation}
It follows that $\{H,f\}_{Poisson}=0$ if $f$ is a constant of motion and independent of time.

The conditions relating canonically conjugate quantities in the Hamiltonian formulation can be compacted in terms of Poisson brackets that are invariant under canonical transformations:
\begin{equation} \label{eq:Canonical_conditions2}
    \{Q_i,Q_k\}_{Poisson} = 0,\qquad \{P_i,P_k\}_{Poisson} = 0, \qquad \{P_i,Q_k\}_{Poisson} = \delta_{ik}
\end{equation}
Poisson algebra appear naturally in Hamiltonian mechanics and we will see in Sect.~\ref{s1:QED} that it is only a special case of Galilean Lie algebra that satisfies Leibniz's law, that is, the bracket of commutation is also a derivation. %https://en.wikipedia.org/wiki/Poisson_algebra

%======================================== NR mechanics (end)
%======================================== 
\section{Classical electrodynamics} 
\label{s1:CED}
As shown in the previous
Sect.~\ref{s1:CM}, the interaction of
particles in non-relativistic classical mechanics is expressed by a potential
energy $U$ function of the coordinates of the interacting
particles only, hence containing the assumption of
instantaneous propagation of interactions. However, as was
evident in the late nineteenth century, this assumption
conflicted with Maxwell's equations for electromagnetism
which we will briefly summarise. the
latter, relied on light being the mediator of interaction
with a finite speed of propagation.

\myparagraph{Theory of special relativity} 
The combination of the principle of relativity with the
finiteness of the velocity of propagation of interactions leads to the theory of special relativity. One of the main consequence of this theory is that time is not absolute, and that only the
speed of light does not depend on the choice of reference
frame. That can be mathematically written as:
\begin{align}
    \label{eq:Lorentz_invariance}
    ds^2 = dt^2 - \bm{dq}^2, \qquad ds^2 = ds'^2
\end{align}
where $ds$ is the
interval in a reference frame (K)
between two infinitely close events separated by
$(\bm{dq},dt)$ and $ds'$ is the interval of the same two
events in (K').

\myparagraph{Lorentz transformations} 
As a consequence of
the interval invariance defined in
Eq.~(\ref{eq:Lorentz_invariance}), we can deduce the relativistic
transformations required to transition from an inertial
frame of reference to another, these are called the Lorentz
transformations. For an inertial frame (K) moving (as of
$t=0$) with velocity $\bm{\dot{\epsilon}}$ with respect to a
different frame (K'), they read:
\begin{align}
    \bm{q'} = \gamma(\bm{q}+\bm{\dot{\epsilon}}t), \qquad
    t' = \gamma\left(t + \bm{\dot{\epsilon}}\cdot \frac{\bm{q'}}{c^2}\right)
\end{align}
where $\gamma \equiv \left(1-\frac{\dot{\epsilon}^2}{c^2}\right)^{-\frac{1}{2}}$ is the
Lorentz factor. Note that the Lorentz transformations
reproduce the Galilean ones defined in
Eq.~(\ref{eq:galilean_transformations}) at the limit where
$\dot{\epsilon} \ll c$.

\myparagraph{Free relativistic particle} 
The simplest form the action integral could take to be
invariant under Lorentz transformations is a scalar. The
integrand must be a differential of the first order and the
only scalar of this kind is the interval $ds$ defined in
Eq.~(\ref{eq:Lorentz_invariance}). Therefore, the action of a free
particle has the form:
\begin{align}
    S = - \alpha \int_a^b ds = -\alpha \int_a^b \sqrt{c^2dt^2 - \bm{dq}^2} \equiv \int_{t_1}^{t_2} L dt =  - \alpha \int_{t_1}^{t_2} c\sqrt{1-\frac{\dot{q}^2}{c^2}}dt
\end{align}
where $\alpha$ is a positive constant characterising the
particle, $a$ and $b$ represent the events of arrival of the
particle at the initial and final position at times $t_1$
and $t_2$ and the minus sign is introduced in order that $S$
has a minimum as $\int_a^b ds > 0$.

To determine $\alpha$ we use the fact that for $c\rightarrow
\infty$ we retrieve the classical expression $L=m\dot{q}^2$.
Therefore expanding $L$ in powers of $\dot{q}/c$:
\begin{align}
    L = -\alpha \sqrt{1-\frac{\dot{q}^2}{c^2}} \stackrel{c \rightarrow \infty}{\simeq} -\alpha c + \alpha \frac{\dot{q}^2}{2c} = m\dot{q}^2
\end{align}
Since the constant $-\alpha c$ can be seen as the exact
differential $-\alpha c(d_t\,t)$, it is of no relevance in $L$
therefore we can write $L = \frac{\dot{q}^2}{2c} =
m\dot{q}^2$ and deduce that $\alpha = mc$. Therefore, the action and Lagrangian of a free particle reads:
\begin{align}
    S = -mc \int_a^b ds, \qquad L = -mc^2 \sqrt{1-\frac{\dot{q}^2}{c^2}}
\end{align}

\myparagraph{Relativistic particles interaction} 
Instead of interpreting the interaction between particles as
one particle acting on another, we can see it as one
particle creating a field around itself which in turn acts
on every other particle located in this field. In classical
mechanics, the field is only another mode of description of
the interaction but in the theory of special relativity and
due to the finite velocity of propagation of interactions
the field itself acquires physical reality. Therefore we
need to formulate our laws to describe the interaction of a
particle with a field and vice versa. 

The interaction
between a given electromagnetic field and a particle
is characterised only by the particle's
charge. The action for a \textit{charge}\footnote{Charge: a
charged particle.} in an electromagnetic field is:
\begin{align}
    \label{eq:EM_field_action}
S = S_p + S_{pf} = \int_a^b\left(-mc ds + \frac{e}{c}A^{\mu} dx_{\mu}\right)
\end{align}
where the left term is the action of a free particle, the
right term describing the electromagnetic interaction with
$e$ being the charge (in an arbitrary unit), $A^\mu = (\bm{A}, \phi/c)$ being
the four-potential of the electromagnetic field and $dx_\mu = (\bm{dq},\,dt)$, the
infinitesimal four-vector.

% Separating the spatial and time component of the potential
% field $A^\mu$ we can write Eq.~(\ref{eq:EM_field_action}) as:
% \begin{align} S = \int_{t_1}^{t_2}\left(-mc
% ds+\frac{e}{c}\bm{A} \cdot \bm{dq}-e\phi dt\right),
% \end{align} therefore: \begin{align}
% \label{eq:EMlagrangian} L =
% -mc^2\sqrt{1-\frac{\dot{q}^2}{c^2}}+\frac{e}{c}\bm{A\cdot
% \dot{q}}-e\phi. \end{align}

\myparagraph{The electromagnetic field tensor} 
The motion
equations of a charge in an electromagnetic field can be
written in four-dimensional form $F_{\mu\nu}$ called \textit{tensor field}. Starting from the
principle of least action and with some algebraic
manipulations, one gets:
\begin{alignat}{2}
    F_{\mu\nu} &= \partial_\mu A_\nu - \partial_\nu A_\mu
    \qquad &&\text{Tensor Field} \\
    F^{\mu\nu}&=-F^{\nu\mu}\qquad &&\text{Antisymmetric} \\
    F_{\mu\nu}F^{\mu\nu} &= 2\left(B^2 -
    \frac{E^2}{c^2}\right)\qquad &&\text{Invariant}\\
    \partial_{\mu}F_{\nu\eta} + &\partial_{\nu}F_{\eta\mu} +
    \partial_{\eta}F_{\mu\nu} = 0\qquad &&\text{Bianchi
    identity} \label{eq:Bianchi} 
\end{alignat}
With the above definitions and properties one can deduce the particle motion equations and expressions of the electric and magnetic field in a rather compact way:
\begin{alignat}{2}
    d_\tau p_\mu &= e F_{\mu\nu} u^\nu \qquad
    &&\text{Particle motion equations}\\ 
    E_i &= c F_{0i} = -\partial_t\bm{A} - \bm{\nabla}\phi \qquad &&\text{Electric field} \\
    B_i &= -\frac{1}{2} \epsilon_{ijk}F^{jk} = \bm{\nabla \times A} \qquad
    &&\text{Magnetic Field} 
\end{alignat}
where $\tau=\frac{1}{\gamma}dt=\frac{1}{c}ds$ is the
particle's proper time, $u^\nu$ is the four-velocity,
$A_\mu$ is the four-potential and $\epsilon_{ijk}$ is the
Levi-Civita tensor.

\myparagraph{Four-current density charge} So far, we've
considered only a punctual charge. The moment we consider
charges to be continuously distributed in space, we talk
instead of charge density $\rho$ such that:
\begin{alignat}{2}
    de &= \rho dV \qquad &&\text{Density charge}\\
    de dx_\mu &= \rho \dot{x}_\mu d^4x \equiv J_\mu d^4x = (\rho\bm{\dot{q}},c\rho)
              \qquad &&\text{Four-current density} \\
    \partial_\mu J^\mu &= 0 \qquad &&\text{Conservation} \label{eq:current_conservation}
\end{alignat}
which allows us to formulate the particle-field interaction
action in a more general way as:
\begin{equation}
    S_{pf} = \frac{e}{c} \int A^{\mu} dx_{\mu} = \frac{1}{c}\int A_uJ^\mu d^4x
\end{equation}
\myparagraph{Field motion equations}
Now that we have derived the motion equations of a particle
interacting with an electromagnetic field, We extend the
action principle to the field itself $S_f$, where for the
whole system it is:
\begin{align}
    S = S_p + S_{pf} + S_f = -mc\int ds + \frac{1}{c}\int A_uJ^\mu d^4x - \frac{1}{4\mu_0c}\int F_{\mu\nu}F^{\mu\nu}d^4x
\end{align}

\myparagraph{Maxwell's equations} To derive Maxwell's
equations that describes the motion of the electromagnetic
field, it suffices to (1) derive the principle of least
action on $S_{pf} + S_f$ with respect to $A_\mu$ and (2)
consider the electromagnetic tensor's Bianchi idendity
Eq.~(\ref{eq:Bianchi}) which leads to:
\begin{alignat}{2}
    (1)\quad \delta S &= \frac{1}{\mu_0c}\int(\partial_\mu
    F^{\mu\nu} + \mu_0 J^\nu)\delta A_\nu d^4x = 0 \\
    &\implies \partial_\mu F^{\mu\nu} = -\mu_0 J^\nu 
    \begin{cases} 
        \bm{\nabla\cdot E} &= \frac{\rho}{\epsilon_0} \quad
        \text{Gauss}\\
        \bm{\nabla \times B} - \frac{1}{c^2}\partial_t\bm{E}
    &= \mu_0\bm{J} \quad \text{Amp\'{e}re} \end{cases} \\
    \nonumber \\
    (2)\quad \partial_{\mu}&F_{\nu\eta} +
    \partial_{\nu}F_{\eta\mu} + \partial_{\eta}F_{\mu\nu} =
    0 \\
    &\implies
    \begin{cases} 
        \bm{\nabla\cdot B} &= 0 \quad \text{Gauss}\\
        \partial_t\bm{B} + \bm{\nabla \times E} &= \bm{0}
        \quad \text{Maxwell-Faraday}
    \end{cases}
\end{alignat}

\myparagraph{Gauge invariance} The Lagrangian is defined only up to an additive total time derivative of any function of coordinates and time:
\begin{equation}
L \rightarrow L' = L + d_t f(\bm{q},t) \implies \delta S = \delta S'    
\end{equation}
The reason being that this quantity does not contribute to the Action variation. This redundant degree of freedom is called \textit{gauge} freedom. The transition from $L$ to $L'$ is called gauge transformation. Gauge fixing or choosing a gauge denotes a specific choice of this degree of freedom which can be useful to simplify some calculations while describing the same physics.

Similarly, in electrodynamics, since $F_{\mu\nu} = \partial_\mu A_\nu - \partial_\nu A_\mu$, we have the following gauge transformation:
\begin{align}
    A^\mu \rightarrow \tilde{A}^\mu = A^\mu + \partial^\mu \chi \implies \delta S = \delta \tilde{S} \implies
    \begin{cases} 
        \bm{E} = \bm{\tilde{E}} = -\partial_t\bm{A} - \bm{\nabla}\phi \\
        \bm{B} = \bm{\tilde{B}} = \bm{\nabla \times A} 
    \end{cases}
\end{align}
Two of the most used gauge fixings in electrodynamics are:
\begin{enumerate}
    \item Coulomb gauge: $\bm{\nabla}\cdot \bm{A}(\bm{q},t) = 0$ which leads to simple wave equations when no sources are present and simple for far field radiation problems.
    \item Lorenz gauge: $\partial_\mu A^\mu = 0$ which is Lorentz invariant, and commonly used because it leads to similar wave equations for both $\phi$ and $\bm{A}$.
\end{enumerate}
In the next section, we will also emphasize on the importance of gauge fixing in quantum electrodynamics.
%======================================== R mechanics (end)
%======================================== 
\section{Quantum electrodynamics} \label{s1:QED}

%\subsection{QED Lagrangian}
%\label{s2:QED_Lagrangian}
% read https://www.quantamagazine.org/what-is-a-particle-20201112/ and shape the intro of this chapter.
% Define operators in quantum mechanics, Read "Single particle systems" in https://en.wikipedia.org/wiki/Canonical_quantisation#First_quantisation 
% first and second quantisation, why do we quantize a field? (https://en.wikipedia.org/wiki/quantisation_of_the_electromagnetic_field)
% transition through poisson brackets http://www.phys.lsu.edu/~jarrell/COURSES/ADV_SOLID_HTML/Other_online_texts/Fradkin/webusers.physics.illinois.edu/~efradkin/phys582/582-chapter4.pdf 
% Canonical quantisation of EM: https://www.damtp.cam.ac.uk/user/tong/qft/six.pdf

Classical electrodynamics summarized in the previous section, fails to describe \textit{elementary}\footnote{Elementary: on the atomic and subatomic scale.} particles and their interactions.
So far, we have only considered particles in the classical view of mechanics as point-like mathematical constructs behaving like macro-scale objects we see with naked eyes. This view is altered completely when describing particles at the \textit{quantum-scale}\footnote{quantum-scale: typically the size of atoms and lower, around $\simeq 100$ pm.}. The first failures of classical electrodynamics were observed with the black body radiation spectrum~\cite{klein1961max} and photoelectric effect~\cite{einstein1905photoelectric}.

Non-relativistic quantum mechanics was proposed as a quantized particle theory in which electromagnetic waves are seen as discrete quanta of energy (photons) and particles described as collapsed probability wave functions~\cite{Dirac1930-DIRTPO}. However, quantum mechanics was not consistent with the principle of special relativity and failed to describe the dynamics of particles moving with a velocity close to the speed of light. The remedy was achieved with the quantum electrodynamics theory, in which fields (instead of particles) are quantized and could only oscillate in discrete amounts, an idea that was extrapolated not only to photons but also to all the other elementary particles which became merely excitations of quantum fields that fill all of space~\cite{peskin2018introduction}.

The transition from a classical to quantum theory requires methods of quantisation such as the canonical~\cite{Dirac1930-DIRTPO, hall2013quantum} or the path integral~\cite{weinberg1995quantum}.
The canonical quantisation is a procedure introduced by Paul Dirac based on the classical canonical conditions in the Hamiltonian formulation introduced in Eq.~\ref{eq:Canonical_conditions2}. In the following, we will revisit very briefly quantum mechanics to deduce the correspondence principle which is at the origin of canonical quantisation, and then use it directly in the context of quantum field theory, where fields are to be quantized instead of being treated as wave-functions as in quantum mechanics.

%We further introduce elements of group theory, namely the Galilean (Sect.~\ref{s2:Galilean_group}) and the Lorentz (Sect.~\ref{s2:Lorentz_group}) groups in order to obtain a precise distinction between the relativistic properties of elementary quantum mechanical systems and those which are also shared by non-relativistic systems.


\myparagraph{Non-relativistic quantum mechanics} In the context of quantum mechanics, a particle is represented by a \textit{wave function}\footnote{Wave function: probability amplitude of finding a particle in a certain position or carrying a certain momentum.} that is a superposition of states Eq.~(\ref{eq:Superposition_of_states}). The act of measuring the state of a particle Eq.~(\ref{eq:Measuring_state_energy}) collapses its wave function. The evolution of the particle state in time is dictated by Shr\"{o}dinger equation Eq.~(\ref{eq:Shrodinger_equation}) in which the operators are non-dependent on time or equivalently by the Heisenberg equation Eq.~(\ref{eq:Heisenberg_equation}) in which the operators incorporate time dependency while the wave function does not. The free particle solution of the Shr\"{o}dinger equation is given by Eq.~(\ref{eq:free_particle_QM}). The probability amplitude for a particle to travel from one point $(\bm{x_1},t_1)$ to a later different point $(\bm{x_2},t_2)$, i.e the propagator is given by Eq.~(\ref{eq:QM_propagator}).
%more info here: https://web2.ph.utexas.edu/~vadim/Classes/2019f/brackets.pdf
\begin{alignat}{2}
    \ket{\psi} &= \sum_n a_n \ket{\psi_n} \qquad && \text{Superposition of states} \label{eq:Superposition_of_states}\\
    \hat{H} \ket{\psi_n} &= E_n \ket{\psi_n} \qquad && \text{Measuring a state's energy}
    \label{eq:Measuring_state_energy} \\ 
    i\hbar (\partial_t &+ \frac{\hbar^2}{2m} \bm{\nabla}^2_x)\psi = 0 \qquad && \text{Shr\"{o}dinger equation}
    \label{eq:Shrodinger_equation} \\ 
    d_t \hat{A}(t) &= -\frac{i}{\hbar}[\hat{A},\hat{H}]+\partial_t \hat{A}\qquad && \text{Heisenberg equation}
    \label{eq:Heisenberg_equation} \\ 
    \psi(\bm{x},t) &\propto e^{i(\bm{p}\cdot{r}-Et)/\hbar} \qquad && \text{Free particle solution} \label{eq:free_particle_QM} \\
    G(\bm{x_2},t_2,\bm{x_1},t_1) &\propto e^{-\frac{m(\bm{x_2}-\bm{x_1})^2}{2i\hbar(t_2-t_1)}} \qquad && \text{Free particle propagator} \label{eq:QM_propagator} 
\end{alignat}

By comparing Eq.~(\ref{eq:Heisenberg_equation}) to the classical Poison brackets Eq.~(\ref{eq:Poisson_brackets}) Paul Dirac and by virtue of the \textit{correspondence principle}\footnote{Correspondence principle: quantum equations of states must reduce to their classical form in the limit $\hbar \rightarrow 0$.} connected the two as in Eq.~(\ref{eq:Correspondence_principle}) and introduced the canonical quantisation, \textit{i.e} replacing any classical variable $A$ by its quantum counter part $\hat{A}$ as follows:
\begin{alignat}{2}
    & \begin{cases} %see https://physics.stackexchange.com/questions/19770/what-is-the-connection-between-poisson-brackets-and-commutators
    \{A,H\}_{Poisson} &\rightarrow -\frac{i}{\hbar} [\hat{A},\hat{H}] \\
    H&\rightarrow \hat{H} = i\hbar \partial_t\\
    p&\rightarrow \hat{p} = -i\hbar\bm{\nabla_x}\\
    x&\rightarrow \hat{x} = x
    \end{cases}&& \text{Correspondence principle} \label{eq:Correspondence_principle} 
\end{alignat}
Any operator can be expressed in either one of the canonical variables spaces: position $\bm{x}$, Eq.~(\ref{eq:Position_space}) or momentum $\bm{p}$, Eq.~(\ref{eq:Momentum_space}). This duality stems from the Heisenberg uncertainty principle Eq.~(\ref{eq:Heisenberg_uncertainty}) translating the fact that position and momentum cannot be simultaneously known to arbitrary precision and the de Broglie relation $p=\frac{h}{\lambda}$ stating that a momentum $p$ of a particle is anti-proportional to it's wavelength $\lambda$ translating the particle-wave duality. 
\begin{alignat}{2}
    \braket{[\hat{x},\hat{p}]} &= i\hbar \qquad && \text{Canonical commutation relation} \label{eq:Canonical_commutation_relation}\\
    \Delta_x \Delta_p &\geq \frac{1}{2i}\braket{[\hat{x},\hat{p}]} = \frac{\hbar}{2} \qquad && \text{Heisenberg uncertainty principle} \label{eq:Heisenberg_uncertainty}\\
    & \begin{cases} 
        \bm{\hat{x}} \ket{\psi_n(\bm{x})} &= \bm{x_n}\ket{\psi_n(\bm{x})}\\
        \bm{\hat{p}} \ket{\psi_n(\bm{x})} &= -i\hbar \bm{\nabla_x} \ket{\psi_n(\bm{x})}
    \end{cases} \qquad && \text{Position space} \label{eq:Position_space}
    \\ & \begin{cases} 
        \bm{\hat{x}} \ket{\psi_n(\bm{p})} &= i\hbar \bm{\nabla_p} \ket{\psi_n(\bm{\bm{p}})}\\
        \bm{\hat{p}} \ket{\psi_n(\bm{p})} &= \bm{p_n} \ket{\psi_n(\bm{p})}
    \end{cases} \qquad && \text{Momentum space} \label{eq:Momentum_space}
\end{alignat}
The Galilean invariance of the Shr\"{o}dinger equation Eq.~(\ref{eq:Shrodinger_equation}) is usually overlooked, and we will briefly discuss how it describes spinless particles with mass $m$ in non relativistic quantum mechanics~\cite{LevyLeblond:1967zz}. 
Let us consider $\psi_n(\bm{p})$ a state $n\in[-s,\dddot{},\,+s]$ expressed in momentum space, then by applying the Galilean transformation $\mathcal{U}(\bm{R},\bm{\dot{\epsilon},\bm{a},b})$ defined in Appendix.~(\ref{s2:Galilean_group}) we get:
\begin{equation}
\psi_n'(\bm{p}) = \mathcal{U}\, \psi_n(\bm{p}) = e^{(iEb - i\bm{p\cdot a})} \sum_{m=-s}^{+s} D^s_{nm}(\bm{R}) \psi_m(\bm{R}^{-1}(\bm{p}-m\bm{\dot{\epsilon}}))  \label{eq:NR_wavefunction_representation}
\end{equation}
where $E=\frac{\bm{p}^2}{2m}$ and $D^s$ is the $(2s+1)$-dimensional unitary\footnote{Unitary: as it satisfies ${\displaystyle |\psi|^2 = \sum_{n=-s}^{+s} \int d^3p|\psi_n(\bm{p})|^2 = 1}$.} representation of the rotation group and $\psi_n(\bm{p})$ is the wave function of a particle with mass $m$ and spin $s$.

Galilean invariance requires that a transformed $\psi'$ differs only by a phase factor:
\begin{align} 
\text{Galilean invariance} &\implies \psi(\bm{x'},t') = e^{if(\bm{x},t)} \psi(\bm{x},t) \label{eq:Galilean_Invariance_SE}\\
\text{Shr\"{o}dinger equation}& \implies f(\bm{x},t)=\frac{1}{2}m \bm{\dot{\epsilon}}^2t + m\bm{\dot{\epsilon}}\cdot \bm{R}\cdot\bm{x} \label{eq:Shrodinger_condition}
\end{align} 
Thus by comparing Eq.~(\ref{eq:Galilean_Invariance_SE}, \ref{eq:Shrodinger_condition}) to the general non relativistic particle representation Eq.~(\ref{eq:NR_wavefunction_representation}) we conclude that the Shr\"{o}dinger equation must describe a spinless particle ($s=0$) with mass $m$.

\textbf{Important note:} It is common to work with Planck units in quantum electrodynamics so for the rest of the thesis we will use $c=1$, $\hbar = \frac{h}{2\pi} = 1$, $\epsilon_0=1$ and $\mu_0=\frac{1}{\epsilon_0 c^2}=1$, the speed of light, reduced Planck constant, permittivity and permeability respectively in Planck units. Implying that, $[length]=[time]=[energy]^{-1}=[mass]^{-1}$.

\myparagraph{Canonical quantisation of the electromagnetic field} 
%see http://www.damtp.cam.ac.uk/user/tong/qft/six.pdf 
%See section 5.2 of Lie algebra book
Quantum mechanics describes particles as wave functions that are bounded by probability conservation, hence fails to describe the creation and annihilation of particles allowed by $E=mc^2$. For that reason, and among others, we head towards a quantum field theory in which the field can be visualized as three-dimensional harmonic oscillators that oscillate with discrete energies. In this schematic picture, every excitation of the field is seen as a particle.

The quantization procedure of the electromagnetic field is complicated by the gauge invariance which renders one of degrees of freedom unphysical. We choose to work in the Lorentz gauge wherein the free theory is:
\begin{alignat}{2}
    L_f &= -\frac{1}{4} F_{\mu\nu}F^{\mu\nu} %- \frac{1}{2}(\partial_\mu A^\mu)^2
    \qquad &&\text{Field Lagrangian} \\
    F_{\mu\nu} &= \partial_\mu A_\nu - \partial_\nu A_\mu \qquad && \text{Tensor field} \\
    \partial_\mu F^{\mu\nu} + \partial^\nu(\partial_\mu A^\mu)&=\partial_\mu \partial^\mu A^\nu= 0 \qquad && \text{Field motion equations}
\end{alignat}
According to the canonical conditions Eq.~(\ref{eq:Canonical_conditions2}) and the canonical commutation relation Eq.~(\ref{eq:Canonical_commutation_relation}), the field $A_\mu$ and its conjugate momentum $\pi^\mu = \frac{\partial L}{\partial \dot{A}_\mu}$ obeys:
\begin{align}
    [A_\mu(\bm{x}),A_\nu(\bm{y})] &= [\pi^\mu(\bm{x}),\pi^\nu(\bm{y})] = 0 \\
    [A_\mu(\bm{x}),\pi_\nu(\bm{y})] & = i g_{\mu\nu}\delta^{(3)}(\bm{x}-\bm{y})
\end{align}
However, for convenience, we choose to work with another set of conjugate operators, the annihilation $a$ and creation operators $a^\dagger$ that are derived from the quantisation of the harmonic oscillator (HO) to the free scalar field. This is motivated by the fact that the quantum HO is one of the few quantum-mechanical systems for which an exact analytical solution is known~\cite{griffiths2018introduction}. The canonical transformation between $A_\mu$ and $\pi^\mu$ to $a$ and $a^\dagger$ is translated by the following \textit{Fourier transform}\footnote{Fourier transform: decomposes functions depending on momentum to functions depending on space and vice versa as in: $\phi(\bm{x},t) = \int \frac{d^3p}{(2\pi)^3} e^{i\bm{p}\cdot \bm{x}}\phi(\bm{p},t)$.}:
\begin{align}
    A_\mu(\bm{x}) &= \int \frac{d^3p}{(2\pi)^3}\frac{1}{\sqrt{2|\bm{p}|}} \sum^3_{\lambda=0}\left[a_{\bm{p}}^\lambda \epsilon_\mu^\lambda e^{i\bm{p}\cdot \bm{x}} + a_{\bm{p}}^{\lambda\,\dagger} \epsilon_\mu^{*\lambda} e^{-i\bm{p}\cdot \bm{x}} \right] \\
    \pi^\mu(\bm{x}) &= i\int \frac{d^3p}{(2\pi)^3} \sqrt{\frac{|\bm{p}|}{2}}\sum_{\lambda=0}^3\left[a_{\bm{p}}^\lambda (\epsilon^\mu)^\lambda e^{i\bm{p}\cdot \bm{x}} - a_{\bm{p}}^{\lambda\,\dagger} (\epsilon^{*\mu})^\lambda e^{-i\bm{p}\cdot \bm{x}} \right]
\end{align} 
where $\epsilon^\lambda_\mu(p)$ is a basis of polarization vectors depending on the photon four-momentum. Due to Lorentz gauge $\partial_\mu A^\mu=0$, $\epsilon^\lambda_\mu$ are transversal and obey $p^\nu\epsilon^\lambda_\nu = p^\nu \epsilon^{*\lambda}_\nu =0$. $\eta^{\lambda \lambda'}$ is the polarisation metric and is usually chosen to be aligned with the photon propagation direction $\bm{p}=(0,0,p_z)$.% and the time direction then $\epsilon^0_\mu(\bm{p})=(1,0,0,0)$ and $\epsilon^3_\mu = (0,0,0,1)$. 
Based on the properties we know about the quantisation of the harmonic oscillator~\cite{griffiths2018introduction}, we can now write the Hamiltonian of a free scalar field theory of light as follows:
\begin{gather}
    H = \int \frac{d^3p}{(2\pi)^3}E_{\bm{p}}\sum_{\lambda=1,2}a^{\lambda,\dagger}_{\bm{p}}a^\lambda_{\bm{p}} \\
    [a^{\lambda}_{\bm{p}},a^{\lambda'}_{\bm{q}}] = [a^{\lambda}_{\bm{p}},a_{\bm{p}}^{\lambda'\,\dagger}] =0,\quad \text{and} \quad [a^{\lambda}_{\bm{p}},a_{\bm{q}}^{\lambda'\,\dagger}] = -\eta^{\lambda \lambda'} (2\pi)^3 \delta^{(3)}(\bm{p}-\bm{q}) \label{eq:bose-einstein} \\
    a^\lambda_{\bm{p}}\ket{0} = 0,\quad \text{and} \quad \ket{\bm{p,\lambda}} \equiv a^{\lambda \dagger}_{\bm{p}}\ket{0} %= \sqrt{2E_{\bm{p}}}a^{\lambda \dagger}_{\bm{p}}\ket{0}
\end{gather} %https://www.imperial.ac.uk/media/imperial-college/research-centres-and-groups/theoretical-physics/msc/current/qed/Photons.pdf


We finally, summarized the quantisation of the electromagnetic field using the canonical commutation relations. A direct implication of this derivation is that annihilation/creation operators obey the Bose-Einstein statistics in which swaping two boson leave the state of the system unchanged, and that can be easily seen in Eq.~(\ref{eq:bose-einstein}).

\myparagraph{Coupling to matter} The first attempt to build a quantized relativistic free particle theory started by considering the relativistic energy-momentum relationship:
\begin{equation} \label{eq:energy-momentum}
    p_\mu p^\mu = E^2 - |\bm{p}|^2 = m^2
\end{equation}
then by canonical quantisation using Eq.~(\ref{eq:Correspondence_principle}) one gets the Klein-Gordon equation:
\begin{equation}
    \left(\bm{\nabla}^2 -\partial^2_{t^2} \right) \psi(\bm{x},t) = m^2 \psi(\bm{x},t)
\end{equation}
which leads to the plane waves particle solution: $\psi(\bm{x},t) \propto e^{-p_\mu x^\mu}$ with the problem of negative energy solutions $E=\pm\sqrt{p^2+m^2}$  associated with negative probabilities.

Dirac searched for an alternative equation in which time and space derivatives are of the first order while still being Lorentz invariant, therefore considered instead the square root form of Eq.~(\ref{eq:energy-momentum}):
\begin{equation}
    E = \sqrt{|\bm{p}|^2+m^2}
\end{equation}
and made the following analogy with the Klein-Gordon equation:
\begin{alignat}{2}
    &\left(\bm{\nabla}^2 - \partial^2_{t^2} \right) = -\beta^2( \bm{\alpha} \cdot \bm{\nabla} + \partial_t)^2 \qquad && \text{Analogy} \label{eq:KG-analogy}\\
    &\implies \begin{cases} 
        \{\alpha_i,\alpha_j\} &= \delta_{ij} \\
        \{\alpha_i, \beta\} &= 0 \quad \forall i \\
        \beta^2 &= 1
    \end{cases} \qquad && \text{Conditions} \label{eq:Dirac-conditions}\\
    & \left(\beta m + \bm{\alpha}\cdot \bm{\nabla}\right)\psi(\bm{x},t) = i\partial_t \psi(\bm{x},t) \qquad && \text{Dirac equation} \label{eq:QMv0-Dirac-equation}
\end{alignat}
the equation has to satisfy the conditions Eq.~(\ref{eq:Dirac-conditions}) in order to reproduce Klein-Gordon when squared. It is found that all representations of such algebra Eq.~(\ref{eq:Dirac-conditions}) can be obtained from those of a Clifford algebra (see Appendix.~(\ref{s2:Lorentz_group})) with dimension 4:
\begin{equation}
    \{\gamma_i,\gamma_j\} = \begin{cases} 2 \delta_{ij} \quad &\text{Galilean group} \\ 2 g_{ij} \quad &\text{Lorentz group} \end{cases} \quad \iff \quad \begin{cases} \gamma^0\alpha_i=\gamma^i \\ \beta = \gamma^0 \end{cases}  
\end{equation}
Therefore, this condition is met if and only if $\alpha_i$ and $\beta$ are $(4\times4)$ matrices following Clifford algebra which implies that the wave function has four components.
We therefore deduce that the Dirac equation explains naturally the appearance of two-component wave functions in Pauli's theory of spin~\cite{pauli1925zusammenhang}.

Substituting $\bm{\alpha}$ and $\beta$ by the $\gamma^\mu$ matrices in Eq.~(\ref{eq:QMv0-Dirac-equation}), the Dirac equation could finally be written as:
\begin{gather}\label{eq:QMv1-Dirac-equation}
i \gamma^\mu \partial_\mu \psi - m\psi = 0 \\
\text{with: }\gamma ^{0}={\begin{pmatrix}\bm{I_2}&0\\0&-\bm{I_2}\end{pmatrix}}~,\gamma ^{i}=\left({\begin{array}{cccc}0&\bm{\sigma_{i}}\\-\bm{\sigma_{i}}&0\end{array}}\right)
\end{gather}
where $\sigma_{x,y,z}$ are the $(2\times 2)$ are the spin-$1/2$ representation of SU(2) algebra, i.e Pauli matrices (see Appendix.~\ref{s3:SU2}) and $I_i$ the identity matrix of dimension $i$ and where the boost and rotation generators are given by Eq.~(\ref{eq:Clifford_algebra}).

The Dirac equation leads to a solution of the form:
\begin{equation} \label{eq:Dirac_field_solution}
    \psi(x^\mu) = u(p^\mu)e^{-p_\mu x^\mu},
\end{equation}
a product of a plane wave and a Dirac spinor $u(p^\mu)$ which can be obtained from the motion equation of the Lagrangian:
\begin{equation}
 L_{Dirac} = \bar{\psi}(i\gamma^\mu \partial_\mu - m)\psi
\end{equation}
%Fermi-stat https://www.damtp.cam.ac.uk/user/tong/qft/five.pdf
where $\bar{\psi} \equiv \psi^\dagger \gamma^0$ chosen to make the latter Lorentz invariant with $\psi^\dagger = (\psi^*)^T$ the complex conjugate of $\psi$ transposed. This solution, once quantized, will describe the behavior of spin-$1/2$ particles or simply fermions. By plugging the solution back into the Dirac equation Eq.~(\ref{eq:QMv1-Dirac-equation}) for a particle (with $p^\mu \neq 0$) we get:
\begin{equation}
    (\gamma^\mu p_\mu - m) (u_A\,\,u_B) = {\begin{pmatrix} (E-m)\bm{I_2} & -\bm{\sigma \cdot p} \\ \bm{\sigma \cdot p} & -(E-m)\bm{I_2}  \end{pmatrix}} {\begin{pmatrix} u_A \\ u_B \end{pmatrix}}=0
\end{equation}
where $u_{A,B}$ are the $(1\times 2)$ upper and lower components of $u$ respectively. Therefore:
\begin{equation}
u_A = \frac{\bm{\sigma \cdot p}}{(E-m)\bm{I_2} }u_B \qquad u_B=\frac{\bm{\sigma \cdot p}}{(E+m)\bm{I_2} }u_A
\end{equation}
The four solutions are obtained by setting successively $u_A$ and $u_B$ to the two different spin states, up: $\begin{pmatrix} 1 \\ 0 \end{pmatrix}$ and down: $\begin{pmatrix} 0 \\ 1 \end{pmatrix}$ as follows:
%http://physics.gu.se/~tfkhj/TOPO/DiracEquation.pdf
\begin{align}
u^1&=\left(1,\quad 0,\quad p_z/(E+m),\quad (p_x+ip_y)/(E+m)\right) \nonumber\\
u^2&=\left( 0,\quad  1,\quad  (p_x-ip_y)/(E+m),\quad  -p_z/(E+m)\right) \nonumber\\
u^3&=\left(-p_z/(-E+m),\quad (-p_x-ip_y)/(-E+m),\quad 1,\quad 0\right) \nonumber\\
u^4&=\left((-p_x+ip_y)/(-E+m),\quad p_z/(-E+m),\quad 0,\quad 1\right) \label{eq:Dirac_solutions}
\end{align}
For a fermion and anti-fermion with momentum $\bm{p}$ along the $z$-axis:
\begin{itemize}
    \item $u^1$ and $u^2$ describe the spin-up and spin-down fermion of energy $E=+\sqrt{m^2 + \bm{p}^2}$ and momentum $\bm{p}$
    \item $u^3$ and $u^4$ the spin-up and spin-down with energy $E=-\sqrt{m^2 + \bm{p}^2}$ and momentum $\bm{p}$. We will define $v^1=u^4(-p)$ and $v^2=u^3(-p)$ instead to translate the fact that they're positive energy anti-fermion states.
\end{itemize}
Both positive and negative energy states solutions in Dirac equations were interpreted to be associated with positive probabilities and therefore not problematic. Dirac attributed the negative energy solutions to positive energy \textit{antiparticle}~\cite{dirac1928quantum,dirac1930theory} propagating forward in time. The prediction of antiparticles was one of the main features of Dirac's theory that was later confirmed by the discovery of positrons~\cite{anderson1933positive}. %(see https://alpha.physics.uoi.gr/foudas_public/APP/Lecture5-Klein-Gordon-Dirac.pdf)

We can now write the general solution of the Dirac equation as a superposition of the solutions given in Eq.~(\ref{eq:Dirac_field_solution}):
\begin{align}
    \psi(x)&=\int \frac{d^3p}{(2\pi)^3}\frac{1}{\sqrt{2E_p}}\sum_s\left(a^s_{\bm{p}}u^s(\bm{p})e^{-ip^\mu x_\mu}+ b^{s\dagger}_{\bm{p}}v^s(\bm{p})e^{ip^\mu x_\mu}\right)\\
    \bar{\psi}(x)&=\int \frac{d^3p}{(2\pi)^3}\frac{1}{\sqrt{2E_p}}\sum_s\left(b^s_{\bm{p}}\bar{v}^s(\bm{p})e^{-ip^\mu x_\mu}+ a^{s\dagger}_{\bm{p}}\bar{u}^s(\bm{p})e^{ip^\mu x_\mu}\right)
\end{align}
where $\sum_s$ is the sum over all the spin-states and $a^s_{\bm{p}}$, $b^s_{\bm{p}}$ are simply the Fourier-coefficients so far.
%A more general definition, is the helicity $h$ where we project spin along %the particle's momentum direction:
%\begin{equation}
%    h=\frac{\bm{S \cdot p}}{|\bm{S}||\bm{p}|} = \begin{cases} +1 &\quad \text%{right-handed} \\ -1 &\quad \text{left-handed} \end{cases}
%\end{equation}

In order to canonically quantize the Dirac field, $\psi$ and the Fourier-coefficients are promoted as quantum operators where $a^s_{\bm{p}}$ corresponds to the annihilation operator (for a fermion), $b^s_{\bm{p}}$ (for an anti-fermion) and $a^{s\dagger}_{\bm{p}}$ the creation operator (for a fermion), $b^{s\dagger}_{\bm{p}}$ (for an anti-fermion).
In the case of the electromagnetic field quantisation, the commutation relations of the creation/annihilation operators, specifically Eq.~(\ref{eq:bose-einstein}), dictated completely that the photons follow Bose-Einstein statistics. Fermions however are spin-$1/2$ particles that obey Fermi-Dirac statistics with the quantum state picking up a minus sign upon the interchange of any two particles. This fact is embedded into the structure of relativistic quantum field theory where a particle is represented by the Lorentz group who's algebra (App.~\ref{s2:Lorentz_group}) is dictated by the anti-commutation relations: %https://www.damtp.cam.ac.uk/user/tong/qft/five.pdf
\begin{equation}
    \{a^{r}_{\bm{p}},a^{s\dagger}_{\bm{q}}\} = \{b^{r}_{\bm{p}},b^{s\dagger}_{\bm{q}}\} = (2\pi)^3\delta^{(3)}(\bm{p}-\bm{q})\delta^{rs} \\
    \{a^{r}_{\bm{p}},a^{s}_{\bm{q}}\} = \{a^{r\dagger}_{\bm{p}},a^{s\dagger}_{\bm{q}}\} = \{b^{r}_{\bm{p}},b^{s}_{\bm{q}}\} = \{b^{r\dagger}_{\bm{p}},b^{s\dagger}_{\bm{q}}\} = 0
    \end{equation}
which therefore implies:
\begin{align}
    \{\psi_\alpha(\bm{x}),\psi_\beta(\bm{y})\} &= \{\psi^\dagger_\alpha(\bm{x}),\psi^\dagger_\beta(\bm{y})\} = 0 \\
    \{\psi_\alpha(\bm{x}),\psi^\dagger_\beta(\bm{y})\} &= \delta_{\alpha \beta}\delta^{(3)}(\bm{x}-\bm{y})
\end{align}
%https://www.desy.de/~jlouis/Vorlesungen/QFTI10/QFTI.pdf
Finally we can write the full quantum electrodynamic Lagrangian using the quantised electromagnetic and Dirac fields as well as their interaction term as:
\begin{align}   \label{eq:L_QED}
    L_{QED} &= L_{Maxwell} + L_{Dirac} + L_{int}\\
            &= -\frac{1}{4} F_{\mu\nu}F^{\mu\nu} + \sum_{j} \bar{\psi}_j(i\gamma^\mu \partial_\mu - m_j)\psi_j - \overbrace{\sum_{j} q_j \bar{\psi}_j\gamma^\mu\psi_j}^{j^\mu}  A_\mu  \\
            &\equiv -\frac{1}{4} F_{\mu\nu}F^{\mu\nu} + \sum_{j}\bar{\psi}_j(i\slashed{D}-m_j)\psi_j
\end{align}
with $q_j$ being the electric charge of the respective field, $\slashed{D} = \gamma^\mu D_\mu = \gamma^\mu (\partial_\mu + iqA_\mu)$ the covariant derivative and $A_\mu$ is the photon field and the index $j$ runs over all known elementary fermions:
\begin{align}
    \text{leptons: } &e,\,\mu,\,\tau,\,\nu_e,\,\nu_\mu,\,\nu_\tau\\
    \text{quarks: } &u,\,d,\,c,\,s,\,t,\,b
\end{align}
The Lagrangian in Eq.~(\ref{eq:L_QED}) is invariant under the gauge transformations:
\begin{align} \label{eq:QED_gauge_transformations} %Schwartz page 481
    \psi_j &\rightarrow \psi'_j = e^{iq_j\alpha(x)}\psi_j \\
    A_\mu &\rightarrow A_\mu' = A_\mu + \frac{1}{q} \partial_\mu \alpha(x)
\end{align}
and the associated motion equations are given by:
\begin{align}
    (i\slashed{D}-m_j)&\psi_j =0,\qquad \partial_\mu F^{\mu\nu}=j^\nu \\
    &\text{with: } k^\mu j_\mu = 0 \label{eq:Ward_idendity}
\end{align}
with the \textit{Ward identity} Eq.~(\ref{eq:Ward_idendity}) being equivalent to the current conservation Eq.~(\ref{eq:current_conservation}) in classical electrodynamics.

\myparagraph{Propagators} The propagator of a relativistic spin-$1/2$ particle equivalent to Eq.~(\ref{eq:QM_propagator}) could be derived by finding the Green's function of the Dirac operator Eq.~(\ref{eq:QMv1-Dirac-equation}):
\begin{alignat}{2}
(i\slashed{\partial}-m)S_F(x-y)&=iI_4\delta^4(x-y) \qquad &&\text{space-time representation} \\
(\slashed{p}-m)\tilde{S}_F(p)&=iI_4 \qquad &&\text{momentum representation}
\end{alignat} 
which leads to the following solutions:
\begin{alignat}{2}
    S_F(x-y)&=\int \frac{d^4p}{(2\pi)^4} e^{-ip(x-y)}S_F(p) \equiv \bra{0}T\psi(x)\bar{\psi}(y)\ket{0} \\
    \tilde{S}_F(p)&=\frac{(\slashed{p}+m)}{p^2-m_e^2+i\epsilon} \equiv \frac{1}{\slashed{p}-m+i\epsilon} \label{eq:fermion_propagator}
\end{alignat} 
where $i\epsilon$ is used as a prescription for integration in the complex plane, uniquely fixing the contour over which the integration is performed to obtain the Green's function~\cite{peskin2018introduction}. $T$ is for time-ordering allowing to sort out both cases where $x^0>y^0$ or $x^0<y^0$.
%and can be generally defined as:
%\begin{equation}
%    T\{A(x)B(y)\equiv \theta(t_x - t_y)A(x)B(y)\pm\theta(t_y-t_x)B(y)A(x)
%\end{equation}
%with $\theta$ denoting the Heaviside step function and the $\pm$ depends on %if the operators are bosonic ($+$) or fermionic ($-$).

Similarly, the photon propagator in Lorentz gauge is given by:
\begin{align}
    D(x-y)&=\bra{0}TA_\mu(x)A_\nu(y)\ket{0} = \int \frac{d^4k}{(2\pi)^4}\frac{-ig_{\mu\nu}}{k^2+i\epsilon}e^{-ik(x-y)}\\
    \tilde{D}(p)&= \frac{-ig_{\mu\nu}}{k^2+i\epsilon} \label{eq:photon_propagator}
\end{align}


\myparagraph{Perturbation theory and Feynman rules} Our final goal is to compute scattering cross sections in order to probe and analyse the hadronic structure in Chapter~\ref{chap:1}. The cross section is formally defined as:
\begin{equation}
\sigma = \frac{N}{\rho_A\cdot l_A\cdot\rho_B l_B\cdot A}    
\end{equation}
where $N$ is the number of scattering events, $A$ and $B$ are two colliding particle bunches having densities $\rho_A$ and $\rho_B$ and length $l_A$ and $l_B$ with A as the common area.
The probability that the initial state $\ket{\psi_A\psi_B}_{in}$ evolves into the final state $_{out}\bra{\psi_1\psi_2\dddot{}}$ is given by:
\begin{align}
    P &= |_{out}\braket{\psi_1\psi_2\dddot{}|\psi_A\psi_B}_{in}|^2\\
    _{out}\braket{\psi_1\psi_2\dddot{}|\psi_A\psi_B}_{in}  &=\lim_{T\rightarrow\infty}\braket{\bm{p}_1\bm{p}_2\dddot{}|e^{-iH(2T)}|\bm{k}_A\bm{k}_B} \\ &\equiv \braket{\bm{p}_1\bm{p}_2\dddot{}|S|\bm{k}_A\bm{k}_B} =\braket{\bm{p}_1\bm{p}_2\dddot{}|(\bm{1}+iT)|\bm{k}_A\bm{k}_B}
\end{align}
where the $S$-matrix or \textit{scattering matrix}~\cite{PhysRev.52.1107} encapsulates the scattering process of the initial and final states. When there's no interaction, $S=\bm{1}$ and therefore all the non-trivial scattering is captured by the T-matrix that we can express as follows:
\begin{align}
    \braket{\bm{p}_1\bm{p}_2\dddot{}|iT|\bm{k}_A\bm{k}_B} &\equiv (2\pi)^4\delta^{(4)}(k_Ak_b-\sum_fp_f)i\mathcal{M}(k_A,k_b\rightarrow p_f) \label{eq:T_matrix}\\
    &\implies d\sigma \propto |\mathcal{M}(k_A,k_B\rightarrow p_f)|^2
    \label{eq:cross_section}
\end{align}
with the $\delta^{(4)}$ function ensures momentum conservation. Unfortunately, we cannot solve analytically Eq.~(\ref{eq:cross_section}), i.e the interacting field theory as we did for the free theories. For that reason, we use perturbative expansion to derive the interaction term $H_{int}$ in terms of the coupling constant\footnote{Coupling constant: the couplings are not really constant, in QED the coupling becomes large at short distance and in QCD the opposite (asymptotic freedom).} (the fine structure constant $\alpha$ in QED). This approximation is valid and approaches the exact answer as long as the coupling is small enough to justify it.

\begin{comment}
For that reason, Let us isolate our Hamiltonian in terms of the free theory $H_0$ and the interaction one $H_{int}$ such that the total theory is $H = H_0 + H_{int}$.
We can write any field operator $\psi$ in either the Heisenberg (H), the Schr\"{o}dinger (S) or the Interaction (I) picture as follows:
\begin{align}
    \psi_H(t,\bm{x})&=e^{iH(t-t_0)}\psi_S(t_0,\bm{x})e^{-iH(t-t_0)}\\
    \psi_I(t,\bm{x})&=e^{iH_0(t-t_0)}\psi_S(t_0,\bm{x})e^{-iH_0(t-t_0)}\\
    \psi_H(t,\bm{x})&=e^{-iH_0(t-t_0)}e^{iH_(t-t_0)}\psi_I(t_0,\bm{x})e^{iH_0(t-t_0)}e^{-iH_(t-t_0)} \nonumber\\
    &\equiv U^\dagger(t,t_0)\psi_IU(t,t_0)
\end{align}
And since:
\begin{align} \label{eq:dt_U}
    i\partial_tU=H_I U \implies U(t,t_0)=1-i\int_{t_0}^t dt' H_I(t')U(t',t_0)
\end{align}
which can be solved iteratively by inserting Eq.~(\ref{eq:dt_U}) into itself leading to:
\begin{equation}
    U(t,t_0)=T\{e^{-i\int_{t_0}^t dt' H_I(t')}\}
\end{equation}
where the time-ordering is the Taylor series of the exponential with each term time-ordered.

Let $\ket{\mathcal{O}}$ be the ground state of $H$ and $\ket{0}$ the ground state of $H_0$ such as:
\begin{align}
    H_0\ket{0}&=0,\qquad H\ket{\mathcal{O}}=E_0\ket{\mathcal{O}},\\
    e^{-iHT}\ket{0}&= \sum_n e^{-iHT}\ket{n}\braket{n|0}=\sum_ne^{-iE_nT}\ket{n}\braket{n|0}
\end{align}
as we take the limit $T\rightarrow \infty(1-i\epsilon)$ and since $e^{-iE_n}$ dies the slowest for n=0 we thus end up with:
\begin{equation}
    \ket{\mathcal{O}}=\lim_{T\rightarrow\infty(1-i\epsilon)}\frac{e^{-iHT}\ket{0}}{e^{-iE_0T}\braket{\mathcal{O}|0}} = \lim_{T\rightarrow\infty(1-i\epsilon)}\frac{U(t_0,-T)\ket{0}}{e^{-iE_0(T+t_0)}\braket{\mathcal{O}|0}} 
\end{equation} 
which allows us to write any propagator of any field $\psi$ as:
\begin{equation}
    \bra{\mathcal{O}}T{\psi(x)\psi(y)}\ket{\mathcal{O}}=\lim_{T\rightarrow\infty(1-i\epsilon)}\frac{\bra{0}T\{\psi_I(x)\psi_I(y)e^{-i\int_{-T}^{T}dtH_I(t)}\}\ket{0}}{\bra{0}T\{e^{-i\int_{-T}^{T}dt H_I(t)}\}\ket{0}}
\end{equation}
Going back to Eq.~(\ref{eq:T_matrix}) we can connect the dots and write:
\begin{align}
    \braket{\bm{p}_1\bm{p}_2\dddot{}|S|\bm{k}_A\bm{k}_B} = \lim_{T\rightarrow\infty(1-i\epsilon)}\,_0\bra{\bm{p}_1\bm{p}_2\dddot{}}T\{e^{-i\int_{-T}^{T}dt H_I(t)}\}\ket{\bm{p}_A\bm{p}_B}_0
\end{align}
\end{comment}
This expansion can be represented diagrammatically as a sum of \textit{Feynman diagrams}~\cite{feynman1949theory}, a tool developed by Feynman 
%by means of \textit{Wick's theorem} that reduces the products of creation and annihilation operators to sums of products of their pairs. 
which allows to express the $S$-matrix up to any order of the perturbative expansion in terms of propagators and Dirac solutions. In case of QED the summary of Feynman rules reads:
%%! https://www.desy.de/~jlouis/Vorlesungen/QFTI10/QFTI.pdf

\begin{table}[!h] 
    \centering
    \renewcommand*{\arraystretch}{1.1}
    \begin{tabular}{ccccc}
  \toprule
        & Propagators & Incoming & Outgoing & Vertex \\
  \midrule
    Photon & $\tilde{D}(p)$ in Eq.~(\ref{eq:photon_propagator}) & $\epsilon_\mu^r(k)$ & $\epsilon_\mu^{\dagger r}(k)$ & \multirow{3}{*}{$-iq\gamma^\mu$}\\
    Fermion & \multirow{2}{*}{$\tilde{S}_F(p)$ in Eq.~(\ref{eq:fermion_propagator})}  & $u^s(p)$ & $\bar{u}^s(p)$ & \\
    Anti-fermion & & $\bar{v}^s(p)$ & $v^s(p)$ & \\
  \bottomrule
\end{tabular}
\caption{\small The QED Feynman rules. \label{tab:QEDFeynmanRules}}
\end{table}

\section{Group theory}
\label{app:group_theory}
The entirety of this appendix relies on \cite{Georgi:1999wka} and contains the main definitions and notions in group theory needed to construct our gauge theories. 

\subsection*{Definitions} 

\myparagraph{Group} A group $G$ is a set with a rule for assigning to every ordered pair of elements, a third element satisfying:
\begin{enumerate}
    \item if $f,g \in G$ then $h=fg \in G$.
    \item For $f,g,h \in G$, $f(gh)=(fg)h$.
    \item There's an identity element $e$ such that for all $f \in G, ef=fe=f$.
    \item Every element $f\in G$ has an inverse $f^{-1}$ such that $ff^{-1}=f^{-1}f=e$.
\end{enumerate}
An \textit{Abelian} group is one in which the multiplication law is commutative $g1g2=g2g1$.

\myparagraph{Representation} \label{s3:representation} A representation of $G$ is a mapping $D$ of the elements of $G$ onto a set of linear operators with the following properties:
\begin{enumerate}
    \item $D(e) = 1$, where $1$ is the identity operator in the space on which the linear operators act.
    \item $D(g_1)D(g_2)=D(g_1g_2)$, \textit{i.e} the group multiplication law is mapped onto the natural multiplication in the linear space on which the linear operators act.
\end{enumerate}

Some properties of representations:
\begin{itemize}
    \item As long as a transformation $S$ is invertible, one can always define a new representation $D'$ such that:
    \begin{equation}
        D(g) \rightarrow D'(g) = S^{-1}D(g)S
    \end{equation}
    where $D'$ is an \textit{equivalent} representation of $D$ differing only by the choice of basis.
    \item \textit{Unitary} representations are such that all operators $D(g)\dagger = D(g)^{-1} \quad [\forall g \in G]$.
    \item A representation is \textit{completely reducible} if it is equivalent to a representation whose matrix elements are in block diagonal form.
    \item Every representation of a finite group is equivalent to a unitary representation.
\end{itemize}

\subsection*{Lie groups}
We are mainly interested in continuously generated groups in the context of quantum field theory. Suppose our group elements $g \in G$ depend \textit{smoothly}\footnote{Smooth: If two elements of a group are "close" in the space of the group elements, so are the parameters that describe them.} on a set of continuous parameters $g(\alpha)$.

\myparagraph{Generators}
It is useful to parameterize the elements $g$ of the group $G$ that they're close to the identity element of the group, and such that $\alpha =0$ corresponds to the identity element $g(\alpha=0)=e$. We can therefore Taylor expand any representation $D(\alpha)$ in terms of the infinitesimal $d\alpha$ as:
\begin{equation} \label{eq:generators}
    D(d\alpha) = 1 + id\alpha_aX_a
\end{equation}
where $X_a=-i\partial_{\alpha_a}D(\alpha)$ for $a=1,...,N$ are the \textit{generators of the group}. There is enormous freedom to parameterise the group elements, we chose one by simply raising eq.~(\ref{eq:generators}) to some large power:
\begin{equation}
    D(\alpha)=\lim_{k\rightarrow\infty}(1 + id\alpha_aX_a)^k = e^{i\alpha_aX_a}
\end{equation}
which defines a particular \textit{exponential parameterization} of the representations.

\myparagraph{Lie algebra} 
Let $U(\lambda) = D(\alpha)^\lambda= e^{i\lambda\alpha_aX_a}$ the representation of a Lie group $G$. The multiplication law (See Section.~\ref{s3:representation}) is simply:
\begin{equation}
    U(\lambda_1)U(\lambda_2) = U(\lambda_1+\lambda_2)
\end{equation}
However if we multiply group elements generated by two different linear combinations of generators $X_a$ and $X_b$, in general:
\begin{equation}
    e^{i\alpha_aX_a}e^{i\beta_bX_b} \neq e^{i(\alpha_a+\beta_a)X_a}
\end{equation}
But since the exponentials form a representation of the group, we have to find a $\delta$ such as:
\begin{equation}
    e^{i\alpha_aX_a}e^{i\beta_bX_b} = e^{i\delta_aX_a}
\end{equation}
Interestingly, by Taylor expanding both sides, we can write:
\begin{align}
    i\delta_aX_a = i\alpha_aX_a + i\beta_aXa - \frac{1}{2}[\alpha_aX_a,\beta_bX_b]+\dddot{}
\end{align}
which we obtained only using the group property and smoothness. We conclude that:
\begin{equation}
    [\alpha_aX_a,\beta_bX_b]=-2i(\delta_c - \alpha_c - \beta_c)X_c+\dddot{} \equiv \gamma_cX_c
\end{equation}
Since the equality above must be true $\forall \alpha, \beta$, we must have $\gamma_c = \alpha_a\beta_bf_{abc}$ for some constants $f_{abc}$ and thus:
\begin{equation}
    [X_a,X_b]=if_{abc}X_c, \qquad f_{abc}=-f_{bac}
    \label{eq:Lie_algebra}
\end{equation}
We finally deduce the following properties of the Lie algebra:
\begin{itemize}
    \item The commutator in Lie algebra plays a role similar to the multiplication law for the group therefore it is enough to define the group.
    \item $f_{abc}$ are called the \textit{structure constants} of the group and the summarize the entire group multiplication law.
    \item eq.~(\ref{eq:Lie_algebra}) is called \text{Lie algebra} of the group which is completely determined by $f_{abc}$.
    \item A unitary representation of the algebra, requires that $f_{abc}$ are real.
    \item The matrix generators satisfy: $[X_a,[X_b,X_c]]+\text{cyclic permutations}=0$ called the Jacobi identity.
    \item The \textit{compact} Lie algebra is the special case where $f_{abc}$ is completely antisymmetric.
\end{itemize}

\myparagraph{SU(2)} \label{s3:SU2} The SU(2) algebra is defined by:
\begin{equation}
    [J_i,J_j]=i\epsilon_{ijk}J_k
    \label{eq:SU2_algebra}
\end{equation}
which is the simplest of the compact Lie algebras because $\epsilon_{ijk}$ is the simplest possible completely antisymmetric object with three indices.

The spin $1/2$ representation in terms of Pauli matrices:
\begin{align}
    J_1^{1/2} &= \frac{1}{2}\begin{pmatrix}
        0 & 1 \\ 1 & 0
    \end{pmatrix}
    = \frac{1}{2}\sigma_1 \\
    J_2^{1/2} &= \frac{1}{2}\begin{pmatrix}
        0 & -i \\ i & 0
    \end{pmatrix}
    = \frac{1}{2}\sigma_2\\
    J_3^{1/2} &= \frac{1}{2}\begin{pmatrix}
        1 & 0 \\ 0 & -1
    \end{pmatrix}
    = \frac{1}{2}\sigma_3
    \label{eq:Pauli}
\end{align}
is the simplest representation of SU(2), satisfying $\sigma_a\sigma_b=\delta_{ab}+i\epsilon_{abc}\sigma_c$ and given by the representation $e^{i\bm{\alpha}\cdot \bm{\sigma}/2}$ which makes it responsible for the name \textit{Special Unitary} as it has a determinant of $1$. All the other representations can be constructed by following a systematic procedure.

\myparagraph{SU(3)} SU(3) is the group of $(3\times 3)$ unitary matrices with determinant 1. It is generated by $t^a = \frac{1}{2}\lambda^a$ where $\lambda^a$ are the hermitian, traceless Gell-Mann matrices (considered as the standard basis):
\begin{align}
    \lambda_{1}&={\begin{pmatrix}0&1&0\\1&0&0\\0&0&0\end{pmatrix}} \quad
    \lambda_{2}={\begin{pmatrix}0&-i&0\\i&0&0\\0&0&0\end{pmatrix}} \quad
    \lambda_{3}={\begin{pmatrix}1&0&0\\0&-1&0\\0&0&0\end{pmatrix}} \quad\\
    \lambda_{4}&={\begin{pmatrix}0&0&1\\0&0&0\\1&0&0\end{pmatrix}} \quad
    \lambda_{5}={\begin{pmatrix}0&0&-i\\0&0&0\\i&0&0\end{pmatrix}} \quad
    \lambda_{6}={\begin{pmatrix}0&0&0\\0&0&1\\0&1&0\end{pmatrix}} \quad\\
    \lambda_{7}&={\begin{pmatrix}0&0&0\\0&0&-i\\0&i&0\end{pmatrix}} \quad
    {\displaystyle \lambda_{8}={\frac {1}{\sqrt {3}}}{\begin{pmatrix}1&0&0\\0&1&0\\0&0&-2\end{pmatrix}}.}
    \label{eq:Gell-Mann}
\end{align}
which are generalisations of the Pauli matrices as the first three Gell-Mann matrices contain the latter.

The generators obey the following relations:
\begin{align}
[t^a,t^b]&=if^{abc}t^c \\
Tr\{t^a t^b\} &= T_R \delta^{ab} \\
\sum_a t^a_{ij}t^a{jk} &= C_F \delta_{ik} \\
\sum_{c,d} f^{acd}f^{bcd} &= C_A \delta_{ab} \\
t^a_{ij}t^a_{kl} = T_R (\delta_{kl}\delta_{il}-\frac{1}{N_C}\delta_{ij}\delta_{kl})
\end{align}
where $f^{abc}$ is a totally antisymmetric structure constant of the group and $T_R=\frac{1}{2}$, $C_F=\frac{4}{3}$, $C_A=N_C=3$ are called the Casimirs of SU(3).


\subsection*{Unitary representation of the Galilean group} \label{s2:Galilean_group} 
%https://arxiv.org/pdf/2004.08661.pdf
The quantum non-relativistic particle is a unitary representation (See Appendix.~\ref{app:group_theory}) of the Galilean group, as much as a relativistic one (Section.~\ref{s3:Coupling_to_matter}) is a representation of the Lorentz group. We derive in the following very briefly the Galilean group and use it to show that the intrinsic spin, for instance, is not a specifically relativistic effect \cite{LevyLeblond:1967zz} in Section.~\ref{s3:Canonical_quantisation_EM}.

The Hilbert space formalism of quantum mechanics leads naturally to a study of the unitary representations of the Galilei group, therefore the matrix representation of the Galilean transformation $\mathcal{U}(\bm{R},\bm{\dot{\epsilon}},\bm{a},b)$ is given by:

\vspace{-15pt}\begin{minipage}{0.25\textwidth}
    \begin{equation*}
        \mathcal{U}=
        \begin{pmatrix}
            \bm{R} & \bm{\dot{\epsilon}} & \bm{a} \\
            0 & 1 & b \\
            0 & 0 & 1  
        \end{pmatrix}
    \end{equation*}
\end{minipage}
\begin{minipage}{0.7\textwidth}
\begin{alignat}{3}
    \text{Tran}&\text{sformations}  \qquad \text{Unitary}&&\text{ Operator} \nonumber\\%&&\qquad \text{ } \nonumber \\
    \bm{x} &\rightarrow R_i(\theta_i)\bm{x} \qquad &&e^{-i\theta_i \hat{J}^i} \\%&&\qquad \text{Rotations}\\
    \bm{x} &\rightarrow \bm{x} + \bm{a} \qquad &&e^{-i a_i \hat{P}^i} \\%&&\qquad \text{Space translations}\\
    \bm{x} &\rightarrow \bm{x} + \bm{\dot{\epsilon}}t \qquad &&e^{i \epsilon_i \hat{G}^i} \\%&&\qquad \text{Boosts}\\
    t &\rightarrow t + b \qquad &&e^{i b \hat{H}} %&&\qquad \text{Time translations}\\
\end{alignat}
\end{minipage}

where $\bm{R}$ is the ($3\times3$) rotation matrix, $\dot{\epsilon}$ and $a$ are the three-vectors of velocities and space-constants, $b$ is a time-constant. We notice that:
\begin{itemize}
    \item Setting $\bm{R}=I_3$, $\bm{a}=\bm{0}$ and $b=0$ reproduces the special case of uniform motion transformations in eq.~(\ref{eq:galilean_transformations}), denoted $(\bm{R}^3,+)$.
    \item Setting $\bm{v}=\bm{0}$, $\bm{a}=\bm{0}$ and $b=0$ lead to the rotation group SO(3).
\end{itemize}
% https://en.wikipedia.org/wiki/Galilei-covariant_tensor_formulation
% https://en.wikipedia.org/wiki/Galilean_transformation

the Galilean transformation $\mathcal{U}$ is represented by a set of four generators, $\hat{H}$ the generator of time translations (Hamiltonian operator), $\hat{\bm{P}}$ the generator of translations (momentum operator), $\hat{\bm{G}}$ is the generator of Galilean transformations (Boosts) and $\hat{\bm{J}}$ generator of rotations (angular momentum operator). The Lie algebra is represented by the following commutation relations:
\begin{align}
    &[\hat{H},\hat{P}_i] = [\hat{P}_i,\hat{P}_j] = [\hat{J}_{ij},\hat{H}] = [\hat{G}_i, \hat{G}_j] = 0\\
    &[\hat{J}_{i},\hat{J}_{j}] = i\hbar\epsilon_{ijk}\hat{J}_k; \qquad [J_{i},P_j]  = i\hbar\epsilon_{ijk} P_k; \qquad [J_{i},G_k] = i\hbar\epsilon_{ijk} \hat{G}_k \\
    &[\hat{G}_i, \hat{H}] = i\hbar \hat{P}_i; \qquad [\hat{G}_i,\hat{P}_j] = i\hbar M\delta_{ij}
\end{align}

The dual Galilean metrics are the time metric $t_{\mu\nu}=diag(1,0,0,0)$ and space metric $h_{\mu\nu}=diag(0,1,1,1)$ that satisfies the orthogonality condition $h^{\mu\nu}t_{\mu\nu}=0$, and by which $x_\mu x_\nu t^{\mu\nu}=t^2$ and $x_\mu x_\nu h^{\mu\nu}=|\bm{x}|^2$ are invariant.

\subsection*{Representation theory of the Lorentz group} \label{s2:Lorentz_group}
%http://physics.unm.edu/Courses/Finley/p581/Handouts/CompleteLorentzGroup.pdf
Similar to Section.~(\ref{s2:Galilean_group}), the Lorentz group denoted SO(1,3) (See Appendix.~\ref{app:group_theory}) expresses the invariance of the relativistic Lagrangian under Lorentz transformations $\Lambda_{\mu\nu}$ is represented by a set of six generators $J^{\mu\nu} = i(x^\mu \partial^\nu - x^\nu \partial^\mu)$ that consists of three rotations and three boosts in Minkowsi space such that $\Lambda^Tg\Lambda = g$ and with the associated unitary operator $e^{-iw_{\mu\nu}J^{\mu\nu}}$. 
The Lie algebra of the group is encapsulated in the following commutation relations:
\begin{align}
    [J^{\mu\nu},J^{\rho\sigma}] & =i(g^{\nu\rho}J^{\mu\sigma}-g^{\mu\rho}J^{\nu\sigma}-g^{\nu\sigma}J^{\mu\rho}+g^{\mu\sigma}J^{\nu\rho})
\end{align}

The Minkowsi metric is $g_{\mu\nu}=diag(1,-1,-1,-1)$ by which $x_\mu x_\nu g^{\mu\nu}=t^2 - |\bm{x}|^2$ is invariant.

At this stage, it is very useful to know that the $\Lambda$ matrices satisfies the Clifford algebra of some matrices $\gamma^\mu$ given by:
\begin{equation} \label{eq:Clifford_algebra}
\{\gamma^\mu,\gamma^\nu\}=2\eta^{\mu\nu} \implies \gamma^{'\mu}=\Lambda^{\mu\nu}\gamma_\nu = S^{-1}\gamma^\mu S \implies S^{\mu\nu}=\frac{i}{4}[\gamma^\mu,\gamma^\nu]
\end{equation}
when $\eta^{\mu\nu} = g^{\mu\nu}$ and where $\{A,B\} = AB + BA$ denotes the anti-commutation relation and $S$ is an invertible transformation that is determined by matching the infinitesimal transformation of $\Lambda = \delta - \frac{i}{2}w_{\mu\nu}J^{\mu\nu}$.

==> _tables/CMS2JET_chi2s.tex <==
\begin{comment}
%-------------------------------------------------------------------------------
\begin{table}%[ht]
    \centering
    \begin{tabular}{lccccc}  \toprule
        Dataset              & $n_{\text{dat}}$ &  w/o (NLO)     & w/ (NLO) &  w/o (NNLO)     & w/ (NNLO)\\
        \midrule
      DIS NC                      &    2113  &   1.28  & 1.31 &   1.25   &    1.27  \\
      DIS CC                      &    81    &   1.24  & 1.25 &   1.15   &    1.16  \\
      Drell-Yan                   &    440   &   1.36  & 1.33 &   1.21   &    1.24  \\
      $Z$ $p_T$                   &    120   &   2.22  & 2.26 &   1.11   &    1.09  \\
      Top pair                    &    25    &   1.67  & 1.11 &   1.27   &    1.27  \\
      Dijets (all)                &    351   &   3.27  & 2.43 &   4.21   &    3.00  \\
      \ \ ATLAS 7 TeV             &    90    &   1.03  & 1.01 &   1.98   &    1.91  \\
      \ \ CMS   7 TeV             &    54    &   1.58  & 2.03 &   1.75   &    1.92  \\
      \ \ CMS   8 TeV             &    122   &   3.87  & 3.61 &   1.48   &    1.55  \\
      \ \ \textbf{CMS   5 TeV}    &    \textbf{85}    &  \textbf{[5.87]}  & \textbf{2.51} &  \textbf{[12.04]}    &    \textbf{6.91}  \\
        \midrule
         Total                    &          &  1.37   & 1.42     &   1.24   &   1.41      \\
\bottomrule
\end{tabular}
\caption{The $\chi^2$ per datapoint for ...}
\label{tab:CMS2JET_chi2s}
\end{table}
%-------------------------------------------------------------------------------
\end{comment}

%-------------------------------------------------------------------------------
\begin{table}%[ht]
  \centering
  \begin{tabular}{lccc}  \toprule
      Dataset              & $N_{\text{dat}}$ &  NLO &  NNLO \\
      \midrule
    DIS NC                      &    2113  &   1.28  &   1.25    \\
    DIS CC                      &    81    &   1.24  &   1.15    \\
    Drell-Yan                   &    440   &   1.36  &   1.21    \\
    $Z$ $p_T$                   &    120   &   2.22  &   1.11    \\
    Top pair                    &    25    &   1.67  &   1.27    \\
    Dijets (all)                &    351   &   3.27  &   4.21    \\
    \ \ ATLAS 7 TeV             &    90    &   1.03  &   1.98    \\
    \ \ CMS   7 TeV             &    54    &   1.58  &   1.75    \\
    \ \ CMS   8 TeV             &    122   &   3.87  &   1.48    \\
      \midrule
       Total                    &          &  1.37   &   1.24    \\
\bottomrule
\end{tabular}
\caption{The $\chi^2$ per datapoint for ...}
\label{tab:CMS2JET_chi2s}
\end{table}
%-------------------------------------------------------------------------------

==> _tables/dijet_fits.tex <==
%-------------------------------------------------------------------------------
\begin{table}%[ht]
    \centering
    \begin{tabular}{lcc}  \toprule
& NLO$_{\text{QCD}}$ & NNLO$_{\text{QCD}}$\\
\midrule
baseline (NNPDF3.1 w/o jets)                   & b    &  bn    \\
\midrule
%ATLAS \& CMS jets   7~TeV                     & j7    & j7n    \\
%ATLAS \& CMS jets7~TeV($\mu=p_T^{\text{jet}}$)& j7-pt & j7n-pt \\
%ATLAS \& CMS jets   8~TeV                     & j8    & j8n    \\
ATLAS \& CMS jets   7-8~TeV                    & ja   & jan    \\
\midrule
%ATLAS \& CMS dijets 7~TeV                     & d7   & d7n     \\
%CMS          dijets 8~TeV                     & d8   & d8n     \\
ATLAS \& CMS dijets 7-8~TeV                    & da   & dan    \\
\bottomrule
\end{tabular}
\caption{The PDF determinations discussed in this thesis and their
IDs. Each row corresponds to a different choice of input jet dataset, 
and each column corresponds
to a different theory accuracy.
The ID encodes the process used (j for single-inclusive
jets and d for dijets); the data used (a for all datasets available);
%, 7 or 8 for the 7~TeV or 8~TeV datasets); 
the perturbative accuracy n for QCD NNLO. 
%and the choice of scale (pt when $\mu=p_T^{\text{jet}}$); 
In this and subsequent tables and plots
``jets'' is short for single-inclusive jets.}
\label{tab:listfits}
\end{table}
%-------------------------------------------------------------------------------

